Set-based state estimation and fault diagnosis using constrained zonotopes and applications

This doctoral thesis develops new methods for set-based state estimation and active fault diagnosis (AFD) of (i) nonlinear discrete-time systems, (ii) discrete-time nonlinear systems whose trajectories satisfy nonlinear equality constraints (called invariants), (iii) linear descriptor systems, and (iv) joint state and parameter estimation of nonlinear descriptor systems. Set-based estimation aims to compute tight enclosures of the possible system states in each time step subject to unknown-but-bounded uncertainties. To address this issue, the present doctoral thesis proposes new methods for efficiently propagating constrained zonotopes (CZs) through nonlinear mappings. Besides, this thesis improves the standard prediction-update framework for systems with invariants using new algorithms for refining CZs based on nonlinear constraints. In addition, this thesis introduces a new approach for set-based AFD of a class of nonlinear discrete-time systems. An affine parametrization of the reachable sets is obtained for the design of an optimal input for set-based AFD. In addition, this thesis presents new methods based on CZs for set-valued state estimation and AFD of linear descriptor systems. Linear static constraints on the state variables can be directly incorporated into CZs. Moreover, this thesis proposes a new representation for unbounded sets based on zonotopes, which allows to develop methods for state estimation and AFD also of unstable linear descriptor systems, without the knowledge of an enclosure of all the trajectories of the system. This thesis also develops a new method for set-based joint state and parameter estimation of nonlinear descriptor systems using CZs in a unified framework. Lastly, this manuscript applies the proposed set-based state estimation and AFD methods using CZs to unmanned aerial vehicles, water distribution networks, and a lithium-ion cell.

==> 03StateEstimation.tex <==
This chapter introduces novel state estimation methods based on constrained zonotopes. The first approach is applied to a linear case considering different sampling times and state-feedback control for trajectory tracking of a suspended load using a tilt-rotor UAV, in which a constrained minimum-variance criterion is proposed for feedback connection with point estimates. Moreover, three novel nonlinear set-valued state estimation methods are developed considering linear measurement, namely the constrained zonotope and interval bundle algorithm, and the consistent generalization of two existing zonotopic methods for nonlinear systems. These are referred to as the mean value extension and the first-order Taylor extension using constrained zonotopes. Preliminary results dealing with nonlinear measurement are also presented, and some future directions are proposed.


\section{Preliminaries} \label{sec:estimationpreliminaries}

\subsection{Set operations and constrained zonotopes}


Some common set operations are often used to compute enclosures required in set-valued state estimation \citep{Le2013,Scott2016}. Consider $Z, W \subset \realset^{n}$, $\mbf{R} \in \realset^{m \times n}$, and $Y \subset \realset^{m}$. Define the linear mapping, Minkowski sum, and generalized intersection, as
\begin{align}
\mbf{R}Z & \triangleq \{ \mbf{R} \mbf{z} : \mbf{z} \in Z\}, \label{eq:limage}\\
Z \oplus W & \triangleq \{ \mbf{z} + \mbf{w} : \mbf{z} \in Z,\, \mbf{w} \in W\}, \label{eq:msum}\\
Z \cap_{\mbf{R}} Y & \triangleq \{ \mbf{z} \in Z : \mbf{R} \mbf{z} \in Y\}, \label{eq:intersection}
\end{align}
respectively. Using ellipsoids or parallelotopes, the linear mapping \eqref{eq:limage} can be computed exactly, but \eqref{eq:msum} and \eqref{eq:intersection} must be over-approximated \citep{Chisci1996,Schweppe1968}. For intervals, the Minkowski sum \eqref{eq:msum} is exact, but \eqref{eq:limage} and \eqref{eq:intersection} are conservative due to the wrapping effect\footnote{The intersection is not conservative if $\mbf{R}$ is the identity matrix.}. This effect is associated to the inability of an interval variable to capture any existing dependency between its components. In contrast, convex polytopes are closed under \eqref{eq:limage}--\eqref{eq:intersection}. Moreover, \eqref{eq:limage} and \eqref{eq:msum} can be computed efficiently in vertex representation (V-rep), and \eqref{eq:intersection} can be computed efficiently in half-space representation (H-rep). However, conversion between H-rep and V-rep is computationally expensive. 

\emph{Zonotopes} \citep{Kuhn1998} allow \eqref{eq:limage} and \eqref{eq:msum} to be computed exactly and with low computational burden, but \eqref{eq:intersection} is not a zonotope in general and must be over-approximated \citep{Le2013,Bravo2006}.

\begin{definition} \rm \label{def:zonotopes}
	A set $Z \subset \realset^n$ is a \emph{zonotope} if there exists $(\mbf{G},\mbf{c}) \in \realsetmat{n}{n_g} \times \realset^n$ such that
	\begin{equation} \label{eq:zdefinition}
	Z = \left\{ \mbf{c} + \mbf{G} \bm{\xi} : \| \bm{\xi} \|_\infty \leq 1 \right\}.
	\end{equation}	
\end{definition}

The term \emph{constrained zonotope} was first used in \cite{Ponsini2012} to refer to a new class of sets introduced in \cite{Ghorbal2010}. This is an  extension of zonotopes defined by the logical product of a zonotope and polyhedral sets. In this doctoral thesis we are interested in the constrained zonotopes (also an extension of zonotopes) defined as in \cite{Scott2016}.


\begin{definition} \rm \label{def:czonotopes}
	A set $Z \subset \realset^n$ is a \emph{constrained zonotope} if there exists $(\mbf{G},\mbf{c},\mbf{A},\mbf{b}) \in \realsetmat{n}{n_g} \times \realset^n \times \realsetmat{n_c}{n_g} \times \realset^{n_c}$ such that
	\begin{equation} \label{eq:czdefinition}
	Z = \left\{ \mbf{c} + \mbf{G} \bm{\xi} : \| \bm{\xi} \|_\infty \leq 1, \mbf{A} \bm{\xi} = \mbf{b} \right\}.
	\end{equation}	
\end{definition}



Equation \eqref{eq:czdefinition} is called \emph{constrained generator representation} (CG-rep), in which each column of $\mbf{G}$ is a \emph{generator}, $\mbf{c}$ is the \emph{center}, and $\mbf{A} \bm{\xi} = \mbf{b}$ are \emph{constraints}. In this doctoral thesis, we refer to $\bm{\xi}$ as the \emph{generator variables}. By defining the constrained unitary hypercube $B_\infty(\mbf{A},\mbf{b}) = \{\bm{\xi} \in \realset^{n_g} : \ninf{\bm{\xi}} \leq 1,\,  \mbf{A} \bm{\xi} = \mbf{b} \}$, a constrained zonotope $Z$ can be alternatively interpreted as an affine transformation of $B_\infty(\mbf{A},\mbf{b})$, given by $Z = \mbf{c} \oplus \mbf{G} B_\infty(\mbf{A},\mbf{b})$. The linear equality constraints allow constrained zonotopes to represent any convex polytope provided that the complexity of the CG-rep \eqref{eq:czdefinition} is not limited. In fact, $Z$ is a constrained zonotope iff it is a convex polytope \citep{Scott2016}. We use the compact notation $Z = \{\mbf{G}, \mbf{c},\mbf{A},\mbf{b} \}$ for constrained zonotopes, and $Z = \{\mbf{G}, \mbf{c}\}$ for zonotopes.


In addition to \eqref{eq:limage} and \eqref{eq:msum}, the intersection \eqref{eq:intersection} can also be computed exactly with constrained zonotopes. The set operations \eqref{eq:limage}--\eqref{eq:intersection} are computed in CG-rep as
\begin{align}
\mbf{R}Z & = \left\{ \mbf{R} \mbf{G}_z, \mbf{R} \mbf{c}_z, \mbf{A}_z, \mbf{b}_z \right\}, \label{eq:czlimage}\\
Z \oplus W & =\left\{ \begin{bmatrix} \mbf{G}_z \,\; \mbf{G}_w \end{bmatrix}, \mbf{c}_z + \mbf{c}_w, \begin{bmatrix} \mbf{A}_z & \bm{0} \\ \bm{0} & \mbf{A}_w \end{bmatrix}, \begin{bmatrix} \mbf{b}_z \\ \mbf{b}_w \end{bmatrix} \right\}\!, \label{eq:czmsum}\\
Z \cap_{\mbf{R}} Y & = \left\{ \begin{bmatrix} \mbf{G}_z \,\; \bm{0} \end{bmatrix}, \mbf{c}_z, \begin{bmatrix} \mbf{A}_z & \bm{0} \\ \bm{0} & \mbf{A}_y \\ \mbf{R} \mbf{G}_z & -\mbf{G}_y \end{bmatrix}, \begin{bmatrix} \mbf{b}_z \\ \mbf{b}_y \\ \mbf{c}_y - \mbf{R} \mbf{c}_z \end{bmatrix} \right\}. \label{eq:czintersection}
\end{align}


These operations can be performed efficiently and cause only a moderate increase in the complexity of the CG-rep. Other useful operations with constrained zonotopes are presented in the following. Property \ref{prop:isemptybelongsto} provides methods to verify if a constrained zonotope is empty and if a given point belongs to it \citep{Scott2016}. Property \ref{prop:hreptocgrep} is a method to compute the corresponding CG-rep of a given convex polytope. Property \ref{prope:ihull} provides a simple method for computing the interval hull of a constrained zonotope by solving $2n$ linear programs (LPs), while Proposition \ref{propo:closest} provides a way to obtain the closest point in a constrained zonotope to another point in space (in the 1-norm sense) through the solution of a single LP. %Such computations are required in some parts of the proposed methods, and the computational cost involved is reasonable because efficient LP algorithms are available. 


\begin{property} \rm \citep{Scott2016} \label{prop:isemptybelongsto}
	For every $\standardcz \subset \realset^{n}$ and $\mbf{z} \in \realset^n$, 
	\begin{align*}
	& Z \neq \emptyset \iff \underset{\bm{\xi}}{\min} \left\{ \ninf{\bm{\xi}} : \mbf{A} \bm{\xi} = \mbf{b} \right\} \leq 1, \\
	& \mbf{z} \in Z \iff \underset{\bm{\xi}}{\min} \left\{ \ninf{\bm{\xi}} : \begin{bmatrix} \mbf{G} \\ \mbf{A} \end{bmatrix} \bm{\xi} = \begin{bmatrix} \mbf{z} - \mbf{c} \\ \mbf{b} \end{bmatrix} \right\} \leq 1.% and $\bm{z} \in \realset{n}$,
	\end{align*}
\end{property}

\begin{property} \rm \citep{Scott2016} \label{prop:hreptocgrep}
	Let $P = \{\mbf{z} : \mbf{H} \mbf{z} \leq \mbf{k}\} \subset \realset^{n}$ be a convex polytope in H-rep, and choose $Z = \{\mbf{G}, \mbf{c}\} \subset \realset^{n}$ and $\bm{\sigma} \in \realset^{n}$ such that $P \subseteq Z$ and $\mbf{H}\mbf{z} \in \left[\bm{\sigma},\,\mbf{k}\right]$, $\forall \mbf{z} \in P$. Then, the convex polytope $P$ can be written in CG-rep as
	\begin{equation} \label{eq:hreptocg}
	P = \left\{ \left[ \mbf{G} \,\; \bm{0} \right], \mbf{c}, \left[ \mbf{H}\mbf{G} \,\;\, \text{diag}\!\left( \dfrac{\bm{\sigma} - \mbf{k}}{2} \right) \right] , \dfrac{\mbf{k} + \bm{\sigma}}{2} - \mbf{H}\mbf{c} \right\}.
	\end{equation}
\end{property}

\begin{property}\rm  \citep{Scott2016,Rego2018} \label{prope:ihull}
	Let $Z = \{\mbf{G}, \mbf{c}, \mbf{A}, \mbf{b} \} \subset \realset^{n}$ and let $\mbf{G}_j$ denote the $j$-th row of $\mbf{G}$. The \emph{interval hull} $[\bm{\zeta}^\text{L},\,\bm{\zeta}^\text{U}] \supseteq Z$ is obtained by solving the following linear programs for each $j = 1,2,\dots,n$:
	\begin{align*}
	\zeta_j^\text{L} & = \underset{\bm{\xi}}{\min} \left\{c_j + \mbf{G}_j \bm{\xi} : \ninf{\bm{\xi}} \leq 1,\, \mbf{A} \bm{\xi} = \mbf{b} \right\}, \\
	\zeta_j^\text{U} & = \underset{\bm{\xi}}{\max} \left\{c_j + \mbf{G}_j \bm{\xi} : \ninf{\bm{\xi}} \leq 1,\, \mbf{A} \bm{\xi} = \mbf{b} \right\}.
	\end{align*}
\end{property}

\begin{proposition} \rm \label{propo:closest} 
	Let $Z = \{\mbf{G}, \mbf{c}, \mbf{A}, \mbf{b} \} \subset \realset^{n}$ and $\mbf{h} \in \realset^{n}$. A point $\mbf{z} \in Z$ that minimizes $\none{\mbf{z} - \mbf{h}}$ is given by $\mbf{z}^* = \mbf{c} + \mbf{G} \bm{\xi}^*$, where $\bm{\xi}^*$ is a solution of the linear program
	\begin{align*}
	& \underset{\bm{\xi}}{\min}~\| \mbf{c} - \mbf{h} + \mbf{G} \bm{\xi} \|_1 \\
	& \text{\rm s.t.} \quad \mbf{A}\bm{\xi} = \mbf{b}, \quad \ninf{\bm{\xi}} \leq 1.
	\end{align*}
\end{proposition}
\proof By definition,
\begin{align*}
\none{\mbf{z}^* - \mbf{h}} &= \none{\mbf{c} - \mbf{h} + \mbf{G} \bm{\xi}^*} \\
&\leq \none{\mbf{c} - \mbf{h} + \mbf{G} \bm{\xi}}, \quad \forall \bm{\xi}\in B_{\infty}(\mbf{A},\mbf{b}).
\end{align*}
But, for any $\mbf{z}\in Z$, there exists $\bm{\xi}\in B_{\infty}(\mbf{A},\mbf{b})$ such that $\mbf{z} = \mbf{c} + \mbf{G} \bm{\xi}$. Therefore, $\none{\mbf{z}^* - \mbf{h}} \leq \none{\mbf{z} - \mbf{h}}$, $\forall \mbf{z}\in Z$.
\qed

The presence of the equality constraints in \eqref{eq:czdefinition} may imply that $\mbf{c} \notin Z$ (i.e., when $\bm{0} \notin B_\infty(\mbf{A},\mbf{b})$). Some of the techniques proposed in this chapter require that $\mbf{c} \in Z$ (Section \ref{sec:choosehfirstorder}). To accommodate this, Proposition \ref{propo:center} provides a simple method for computing an alternative (more complex) CG-rep for $Z$ whose center is any desired point in space.


\begin{proposition}[Rescaling with desired center] \rm \label{propo:center}
	Let $Z = \{\mbf{G},\mbf{c},\mbf{A},\mbf{b}\} \subset \realset^n$ and  let $\tilde{\bm{\xi}}^\text{L}, \tilde{\bm{\xi}}^\text{U} \in \realset^{n_g}$ satisfy $\conball \subseteq [\tilde{\bm{\xi}}^\text{L},\,\tilde{\bm{\xi}}^\text{U}]$. Choose any desired center $\mbf{h} \in \realset^n$ lying in the range of $\mbf{G}$ and let $\xil, \xiu \in \realset^{n_g}$ be solutions of the linear program:
	\begin{align*}
	%& \underset{\xil,\xiu}{\min}~\| \bm{\zeta} \|_\infty, \quad \bm{\zeta} = \begin{bmatrix} \xil \\ \xiu \end{bmatrix},\\
	& \underset{\xil,\xiu}{\min}~\left\| \half (\xiu - \xil) \right\|_1 \\% \quad \bm{\zeta} = \begin{bmatrix} \xil \\ \xiu \end{bmatrix},\\
	& \text{s.t.} \quad \mbf{c} + \half \mbf{G} (\xil + \xiu) = \mbf{h} \\
	& \xil \leq \tilde{\bm{\xi}}^\text{L} \\
	& \xiu \geq \tilde{\bm{\xi}}^\text{U}
	\end{align*}
	Letting $\xim = \half (\xil + \xiu)$ and $\mbf{E}_r = \half\text{diag}(\xiu - \xil)$, an equivalent CG-rep of $Z$ with center $\mbf{h}$ is given by
	\begin{align} 
	Z = \left\{\begin{bmatrix} \mbf{G} \mbf{E}_r & \bm{0} \end{bmatrix}, \mbf{h}, \begin{bmatrix} \mbf{A} \mbf{E}_r & \bm{0} \\ \bm{0} & \mbf{A} \\ \mbf{G} \mbf{E}_r & -\mbf{G} \end{bmatrix} , \begin{bmatrix}\mbf{b} - \mbf{A} \xim  \\ \mbf{b} \\ \mbf{c} - \mbf{h} \end{bmatrix}  \right\}. \label{eq:centerchange}
	\end{align}
\end{proposition}

\proof It is first shown that $Z$ is contained in the set 
\begin{equation*}
\bar{Z} = \{ \mbf{GE}_r,\,\mbf{c} + \mbf{G} \xim,\, \mbf{AE}_r,\, \mbf{b} - \mbf{A} \xim \}.
\end{equation*}
Choose any $\mbf{z} \in Z$. There must exist $\bm{\xi} \in B_\infty (\mbf{A},\mbf{b})$ such that $\mbf{z} = \mbf{c} + \mbf{G} \bm{\xi}$. Since $\bm{\xi} \in [\xil,\,\xiu]$, there must exist $\bm{\delta} \in B_\infty$ such that $ \bm{\xi} = \xim + \mbf{E}_r\bm{\delta}$. Thus,
\begin{align*}
\mbf{z} \in Z & \implies \exists \bm{\delta} \in B_\infty : \mbf{z} = \mbf{c} + \mbf{G} (\xim + \mbf{E}_r \bm{\delta}), \\ & \qquad \qquad \qquad \quad \; \mbf{A}(\xim + \mbf{E}_r \bm{\delta})= \mbf{b},\\
& \implies \mbf{z} \in \bar{Z}.
\end{align*}
Therefore, $Z \subseteq \bar{Z}$ and it follows that $Z=\bar{Z} \cap Z$. Since $\xil$ and $\xiu$ satisfy $\mbf{c} + \half \mbf{G} (\xil + \xiu) = \mbf{h}$, the constrained zonotope $\bar{Z}$ has center $\mbf{h}$. Then, representing $\bar{Z} \cap Z$ as in \eqref{eq:czintersection} gives \eqref{eq:centerchange}. \qed


\begin{remark} \rm \label{rem:rescalingtocenter}
	The linear program in Proposition \ref{propo:center} does not require $[\xil, \xiu] \subseteq B_\infty$. Therefore, the midpoint $\half (\xil + \xiu)$ can assume any desired value, and it is always possible to satisfy $\mbf{c} + \half \mbf{G} (\xil + \xiu) = \mbf{h}$ if $\mbf{h}$ is in the range of $\mbf{G}$. Thus, the linear program is always feasible.
\end{remark}

\subsection{Interval arithmetic} \label{sec:iarithmetic}

Interval arithmetic is a traditional tool for set-valued state estimation of nonlinear systems \citep{Jaulin2009}. Let $\intvalset$ denote the set of compact intervals in $\realset$. An \emph{interval} $x \in \intvalset$ is a real compact set defined by $x = \{ a \in \realset : x^\lbound \leq a \leq x^\ubound \}$, with shorthand notation $[x^\lbound,x^\ubound]$, where $x^\lbound, x^\ubound \in \realset$ are called \emph{endpoints}. The four basic interval arithmetic operations are defined by $[x^\lbound,x^\ubound] \odot [y^\lbound,y^\ubound] = \{ a \odot b : a \in [x^\lbound,x^\ubound], b \in [y^\lbound,y^\ubound] \}$, where `$\odot$' denotes interval addition, subtraction, multiplication or division (the latter works provided that $0 \notin [y^\lbound,y^\ubound]$). The midpoint and radius are defined by $\midpoint{x} = \half(x^\ubound + x^\lbound)$ and $\rad{x} = \half(x^\ubound - x^\lbound)$. The diameter is defined by $\diam{x} = 2\rad{x}$. 

\begin{definition} \rm \label{def:intvalvector}
	A set $B \subset \realset^n$ is an \emph{interval vector} if there exists $(\betal,\betau) \in \realset^{n} \times \realset^{n}$ such that $B = \{ \bm{\beta} \in \realset^{n} : \beta_j^\text{L} \leq \beta_j \leq \beta_j^\text{U},\, j=1,2,\dots,n \}$.
\end{definition}

Similarly, interval matrices are defined by $\{ \mbf{A} \in \realset^{n \times m}: A_{ij}^\lbound \leq A_{ij} \leq A_{ij}^\ubound\}$. Interval matrix operations are performed according to the rules of real matrix algebra. The midpoint and radius are defined component-wise for interval vectors and matrices \citep{Moore2009}. An interval $[x^\lbound, x^\ubound]$ is said to be \emph{degenerate} iff $x^\text{L} = x^\text{U}$. %In this chapter, we say that an interval vector $\mbf{x} \in \intvalset^n$ is degenerate iff $x_j^\text{L} = x_j^\text{U}$ for any $j \in \{1,2,\ldots,n\}$. Otherwise, it is said to be \emph{non-degenerate}. 

\begin{definition} \rm \label{def:degenerate}
	An interval vector $[\mbf{x}^\lbound, \mbf{x}^\ubound] \in \intvalset^n$ is \emph{degenerate} iff $x_j^\text{L} = x_j^\text{U}$ for any $j \in \{1,2,\ldots,n\}$. Otherwise, it is said to be \emph{non-degenerate}. 
\end{definition}

Inclusion functions perform a central role in interval arithmetic. Let $\iextension{\mbf{f}(X)}$ denote an interval enclosure of a real valued function $\mbf{f}$ over an interval $X \subset \realset^n$, where $X$ is an interval enclosure of the domain of interest (the notation $\iextension{\mbf{f}(X)}$ is used through the chapter even when $X$ is not an interval. In this case, it is assumed that an interval hull of $X$ is employed in the operation). Then, $\mbf{f}(X) \subseteq \iextension{\mbf{f}(X)}$. Inclusion functions of elementary operations, such as $\{\sin, \cos, \ln, \exp\}$, are defined by their images over the respective interval arguments. For instance, the natural interval extension of a real function is obtained by recursively computing inclusion functions for all arithmetic and elementary operations that compose it \citep{Moore2009}.

\begin{remark} \rm  \label{rem:intervaloverestimation}
	The most common sources of conservatism in inclusion functions are the \emph{interval dependency} and the \emph{wrapping effect}. The latter is inherent to multi-variable mappings of interval variables, and results from the inability of an interval vector (matrix) to capture any existing dependency between its components. On the other hand, the interval dependency results from the multi-occurrence of the same interval variable in an algebraic expression \citep{Moore2009}.
\end{remark}

A usual method to reduce overestimation of inclusion functions is the use of refinements \citep{Moore2009}. In order to proceed we first define \emph{interval bundles} and \emph{$n_d$-partitions}.

\begin{definition} \rm \label{def:partitions}
	Given $n_b$ interval vectors $B_j \subset \realset^{n}$, with $j = 1,2,\ldots,n_b$. An \emph{interval bundle} is defined by $\mathcal{B} \triangleq \bigcup_{j=1}^{n_b} B_j$.
\end{definition}


It is clear that an interval bundle is not a interval vector in general. Thus, an interval bundle cannot be defined through endpoints. However, it can be regarded as a \emph{list of interval vectors} without computing the union explicitly. Moreover, the concept of an interval bundle is closely related to subpavings.% \citep{Jaulin2001}.

\begin{remark} \rm \label{rem:subpavings}
	A subpaving is defined as the union of non-overlapping intervals, and it is often associated with a tree structure. This class of sets is usually employed in interval branch-and-bound procedures such as set inversion \citep{Jaulin2001}.
\end{remark} 


\begin{definition} \rm
	Let $B$ be a non-degenerate interval vector in $\realset^{n}$. The \emph{$n_d$-partition} of $B$ is an interval bundle $\mathcal{B} = \cup_{j=1}^{n_b} B_j$ such that $\mathcal{B} = B$, $\text{diam}(B_j) = (1/n_d)\text{diam}(B)$, and the intersection of two intervals $B_j$ and $B_i$ produces a degenerate interval vector in $\realset^{n}$ for every $i\neq j$, with $i,j = 1,2,\dots,n_b$, and $n_d \in \naturalset\textbackslash0$.
\end{definition}

The $n_d$-partition of an interval vector can be seen as a ``multi-dimensional grid'' with $n_d$ divisions per dimension. By definition, the diameter of each interval vector composing the grid is inversely proportional to the number of divisions, and proportional to the diameter of the original interval vector. Note that $n_b = n_d$ for the unidimensional case. %

For a real valued function $f(\cdot)$ and a $n_d$-partition $\mathcal{B} = \cup_{j=1}^{n_b} B_j$ of an interval vector $B$, a \emph{refinement} of an inclusion function $\iextension{f(\cdot)}$ over $\mathcal{B}$ is defined by $\cup_{j=1}^{n_b} \iextension{f(B_j)}$. The conservatism of a refinement is substantially reduced if compared with single inclusion functions over $B$ (see Chapter 6 in \cite{Moore2009} for details), and since each $\iextension{f(B_j)}$ results in an interval vector, a refinement is also an interval bundle.

%\section{Linear state estimation} \label{sec:linearestimation}
%
%This section deals with the problem of path tracking of a suspended load using a tilt-rotor UAV. Such task requires the knowledge of the load position, which may not be provided by available sensors. Therefore, to accomplish the path tracking, a linear set-valued state estimator based on constrained zonotopes is proposed to solve the problem of estimating the load position and orientation, considering sensors with different sampling times, and unknown-but-bounded disturbances. In order to provide feedback to the controller using the estimated state set, an optimal choice of the estimated point is given according to a proposed constrained minimum-variance criterion. The path tracking is then solved by a discrete-time mixed $\mathcal{H}_2/\mathcal{H}_\infty$ controller with pole-placement constraints \citep{Rego2018c}. Results from numerical experiments, performed in a platform based on the Gazebo simulator with a Computer Aided Design (CAD) model of the system\footnote{See https://github.com/Guiraffo/ProVANT-Simulator.} \citep{Lara2017}, are presented to corroborate the performance of the linear set-valued state estimator along with the designed control strategy. The content of this section was accepted to be published in \cite{Rego2018b}.
%
%
%\subsection{Tilt-rotor UAV with suspended load modeling} \label{sec:tiltrotormodeling}
%
%\subsubsection{Equations of motion}
%
%This section describes the tilt-rotor UAV with suspended load (Fig. \ref{fig:modeling_kinematics}) as a multi-body mechanical system composed of: (i) the aircraft's main structure (including batteries, landing skids, electronics and instrumentation); (ii) the right thruster group (right thruster and revolute joint); (iii) the left thruster group (left thruster and revolute joint); and (iv) the load group (load and rope). For control purposes, the rope is assumed to be rigid and massless.
%
%%The equations of motion of the entire system are formulated considering the load as a free rigid body, with the tilt-rotor UAV rigidly attached to it. This choice of perspective allows state-feedback control strategies to directly steer the trajectory of the load \citep{Rego2018c}. Nine reference frames are defined (Fig. \ref{fig:modeling_kinematics}): (i) the inertial reference frame, $\frI$; (ii) the load center of mass frame, $\frL$; (iii) the aircraft's geometric center frame, $\frB$; (iv) the main body center of mass frame, $\frC{1}$; (v) the right thruster center of mass frame, $\frC{2}$; and (vi) the left thruster center of mass frame, $\frC{3}$; (vii) the rope's point of connection frame, $\frA{1}$; (viii) the right tilting axis frame, $\frA{2}$; and (ix) the left tilting axis frame, $\frA{3}$.
%
%The equations of motion of the entire system are formulated from the perspective of the load, by considering the load as a free rigid body with the tilt-rotor UAV rigidly attached to it. This choice of perspective allows state-feedback control strategies to directly steer the trajectory of the load \citep{Rego2018c}. Nine reference frames are defined (Fig. \ref{fig:modeling_kinematics}): (i) the inertial reference frame, $\frI$; (ii) the load center of mass frame, $\frL$; (iii) the aircraft's geometric center frame, $\frB$; (iv) the main body center of mass frame, $\frC{1}$; (v) the right thruster center of mass frame, $\frC{2}$; (vi) the left thruster center of mass frame, $\frC{3}$; (vii) the rope's point of connection frame, $\frA{1}$; (viii) the right tilting axis frame, $\frA{2}$; and (ix) the left tilting axis frame, $\frA{3}$.
%
%\begin{figure}[!ht]
%	\centering{
%		%\def\svgwidth{0.6\textwidth}
%		%\def\svgwidth{0.8\columnwidth}
%		\def\svgwidth{0.6\columnwidth}
%		%{\small\import{Figures_02Modeling/}{loadtiltrotor2_newkinematics_nopoints.pdf_tex}}%\vspace{-1mm}
%		{\vspace{-3mm}\small\import{Figures_CDC/Figures_02Modeling/}{loadtiltrotor2_newkinematics_nopoints.pdf_tex}}%\vspace{-1mm}
%		\caption{The tilt-rotor UAV with suspended load, kinematic definitions, input forces and torques.}\label{fig:modeling_kinematics}}
%	%\vspace{-3mm}
%\end{figure}
%
%The position of the load with respect to $\frI$ is denoted by $\bm{\zeta} \triangleq [ x \;\, y \;\, z ]^T$. The displacement from $\frL$ to $\frA{1}$ is defined in $\frL$ as $\dLA{1} \triangleq [ 0 \;\, 0 \;\, l ]^T$, where $l$ corresponds to the rope's length. The displacements from $\frA{1}$ to $\frB$, from $\frB$ to $\frC{1}$, from $\frB$ to $\frA{i}$, and from $\frA{i}$ to $\frC{i}$ are denoted by $\dAB{1}$, $\dBC{1}$, $\dBA{i}$, $\dAC{i}{i}$, respectively, in the respective preceding frames, with $i \in \{2,3\}$. The orientation of the load with respect to $\frI$ is parametrized by Euler angles, $\bm{\eta} \triangleq [ \phi \; \theta \; \psi ]^T$, using the $ZYX$ convention about local axes, and is described by
%\begin{equation} \label{eq:RIL}
%\RIL {\triangleq} \mbf{R}_{z,\psi} \mbf{R}_{y,\theta} \mbf{R}_{x,\phi} {=}  \begin{bmatrix}
%\text{c}_\psi \text{c}_\theta & \text{c}_\psi \text{s}_\theta \text{s}_\phi {-} \text{s}_\psi \text{c}_\phi & \text{c}_\psi \text{s}_\theta \text{c}_\phi {+} \text{s}_\psi \text{s}_\phi \\
%\text{s}_\psi \text{c}_\theta & \text{s}_\psi \text{s}_\theta \text{s}_\phi {+} \text{c}_\psi \text{c}_\phi & \text{s}_\psi \text{s}_\theta \text{c}_\phi {-} \text{c}_\psi \text{s}_\phi \\
%-\text{s}_\theta & \text{c}_\theta \text{s}_\phi & \text{c}_\theta \text{c}_\phi
%\end{bmatrix} \text{.}
%\end{equation}
%with $\text{s}_{(\cdot)} {\triangleq} \sin(\cdot)$ and $\text{c}_{(\cdot)} {\triangleq} \cos(\cdot)$. The orientation of the UAV with respect to $\frL$ is described by $\bm{\gamma} \triangleq [ \gone \; \gtwo ]^T$, with $\RLA{1} \triangleq \mbf{R}_{x,-\gone} \mbf{R}_{y,-\gtwo}$. The orientation of the thrusters' groups with respect to $\frB$ are defined by $\RBA{2} \triangleq \mbf{R}_{x,-\beta} \mbf{R}_{y,\aR}$ and $\RBA{3} \triangleq \mbf{R}_{x,\beta} \mbf{R}_{y,\aL}$, where $\aR$ and $\aL$ are the right and left tilting angles, respectively, and $\beta$ is a fixed inclination angle of the thrusters towards $\frB$ \citep{Rego2018c}. Moreover, $\frA{1}$, $\frB$, and $\frC{1}$ are parallel and attached to the same rigid body, thus $\RAB{1} = \RBC{1} = \RAC{i}{i} = \eye{3}$, $\RLB = \RLA{1}$, $\RBC{i} = \RBA{i}$, $i \in \{2,3\}$.
%
%Let $\wLIL$ denote the angular velocity of frame $\frL$ with respect to $\frI$, expressed in $\frL$. Then, $\wLIL = \Weta \deta$, $\wALA{1} = \mbf{Q} \dgamma$, $\wABA{2} = \ay \daR$, $\wABA{3} = \ay \daL$, $\wBAB{1} = \wiBi{1} = \wiAi{i} = \zeros{3}{1}$\footnote{$\eye{n}$ is an identity matrix with dimension $n$, and $\zeros{n}{m}$ denotes an $n$ by $m$ matrix of zeros.}, $\wBLB = \wALA{1}$, and $\wiBi{i} = \wABA{i}$, with
%\begin{equation*}
%\Weta \triangleq \begin{bmatrix}
%1 & 0 & -\text{s}_\theta \\
%0 & \text{c}_\phi & \text{s}_\phi \text{c}_\theta \\
%0 & -\text{s}_\phi & \text{c}_\phi \text{c}_\theta
%\end{bmatrix}\text{,} \quad \mbf{Q} \triangleq \begin{bmatrix}
%-\text{c}_\gtwo & 0 \\
%0 & -1 \\
%\text{s}_\gtwo & 0
%\end{bmatrix}\text{,} \quad \ay \triangleq \begin{bmatrix} 0 \\ 1 \\ 0 \end{bmatrix}.
%\end{equation*}
%
%The generalized coordinates are defined according to $\mbf{q} \triangleq [ \bm{\zeta}^T \,\; \bm{\eta}^T \,\; \bm{\gamma}^T \,\; \aR \,\; \aL ]^T$, 
%which include the load's position and orientation given in the inertial frame and reflect the choice of perspective. Therefore, through the Euler-Lagrange formulation \citep{Rego2018c}, the equations of motion are written as
%\begin{equation} \label{eq:eulerlagrangeCANONICAL}
%\mbf{M}(\mbf{q})\ddot{\mbf{q}} + \mbf{C}(\mbf{q},\dot{\mbf{q}})\dot{\mbf{q}} + \mbf{g}(\mbf{q}) = \gforce(\mbf{q},\dot{\mbf{q}},\mbf{u},\mbf{d}) \text{,}
%\end{equation}
%where $\mbf{M}(\mbf{q})$ is the inertia matrix, $\mbf{C}(\mbf{q},\dot{\mbf{q}})$ is the Coriolis and centripetal forces matrix, $\mbf{g}(\mbf{q})$ is the gravitational forces vector, and $\gforce(\mbf{q},\dot{\mbf{q}},\mbf{u},\mbf{d}) = \mbf{L}_\text{in}(\mbf{q}) \mbf{u} - \mbf{L}_\text{fr} \dot{\mbf{q}} + \mbf{L}_\text{db} \mbf{d}$, with $\mbf{u} = [\infR \,\; \infL \,\; \intauaR \,\; \intauaL]^T \in \setreal^4$ denoting the system inputs (thrust forces and servomotor torques, see Fig. \ref{fig:modeling_kinematics}), and $\mbf{d} \in \setreal^3$ denoting external disturbances affecting the load (see \cite{Rego2018c} for details).
%
%Finally, by defining the system states $\mbf{x} \triangleq \begin{bmatrix} \mbf{q}^T & \dot{\mbf{q}}^T \end{bmatrix}^T \in \setreal^{20}$, the equations \eqref{eq:eulerlagrangeCANONICAL} are written as $\dot{\mbf{x}} = \mbf{\varphi}(\mbf{x}, \mbf{u}, \mbf{d})$, 
%\begin{equation} \label{eq:modeling_statespacenonlinear}
%\bm{\varphi}(\mbf{x}, \mbf{u}, \mbf{d}) {=} \begin{bmatrix}
%\dot{\mbf{q}} \\
%\mbf{M}^{-1} \left[ - (\mbf{C}  + \mbf{L}_\text{fr}) \dot{\mbf{q}} - \mbf{g}(\mbf{q}) + \mbf{L}_\text{in}(\mbf{q}) \mbf{u} + \mbf{L}_\text{db}\mbf{d} \right]
%\end{bmatrix} \text{,}
%\end{equation}
%which describes the load behavior in the inertial frame explicitly, with the aircraft's position and orientation being described only with respect to the load.
%
%
%\subsubsection{Measurement equation} \label{sec:tiltrotormeasurement}
%
%
%This doctoral thesis assumes that the load position and orientation with respect to the inertial frame are not measured. Available measurements are provided by: (i) a Global Positioning System (GPS), providing the planar position of the tilt-rotor UAV with respect to $\frI$; (ii) a barometer, providing the altitude of the UAV with respect to $\frI$; (iii) an Inertial Measurement Unit (IMU), providing the orientation and angular velocities of the UAV with respect to $\frI$; (iv) a camera, providing the position of the load with respect to the $\frA{1}$; and (v) embedded sensors at the servos, providing the tilting angles and their time derivatives.
%
%The GPS, barometer, and IMU are located at $\frB$, while the camera is placed at the origin of $\frA{1}$. Let $\zetaB \triangleq [x_\frB \,\; y_\frB \,\; z_\frB]^T$ denote the position of the UAV with respect to $\frI$. Then,
%\begin{equation} \label{eq:estimation_gpsbarometerequation}
%\zetaB(\bm{\zeta},\bm{\eta}) = \bm{\zeta} + \RIL \dLA{1} + \RIL \RLB \dAB{1} \text{.} 
%\end{equation}
%
%The orientation of the UAV with respect to $\frI$ is parametrized by $\etaB \triangleq [\phiB \; \theta_\frB \; \psi_\frB]^T$, using the local roll-pitch-yaw convention. Therefore, $\RIB \triangleq \mbf{R}_{z,\psiB} \mbf{R}_{y,\thetaB} \mbf{R}_{x,\phiB} = \RIL \RLB$, hence, %
%\begin{gather}
%\phiB(\bm{\eta},\bm{\gamma}) = \arctan({{(\RIL \RLB)}_{32}}/{{(\RIL \RLB)}_{33}}) \text{,} \label{eq:estimation_IMUetaBequation01}\\
%\thetaB(\bm{\eta},\bm{\gamma}) = \arcsin(-{(\RIL \RLB)}_{31}) \text{,} \label{eq:estimation_IMUetaBequation02}\\
%\psiB(\bm{\eta},\bm{\gamma}) = \arctan({{(\RIL \RLB)}_{21}}/{{(\RIL \RLB)}_{11}}) \text{,} \label{eq:estimation_IMUetaBequation03}
%\end{gather}
%for $\thetaB \neq \pm \pi/2$, where $(\cdot)_{ij}$ denotes the element from the $i$-th row and $j$-th column. Moreover, the angular velocity provided by the IMU is given by
%\begin{equation}
%\wBIB(\bm{\eta},\bm{\gamma},\deta,\dgamma) = \bm{\omega}^\frB_{\frI \frL} + \wBLB = (\RLB)^T \Weta \deta + \mbf{Q} \dgamma. \label{eq:estimation_IMUwBIBequation}
%\end{equation}
%
%On the other hand, let $\mbf{d}^\frA{1}_{\frA{1}\frL}$ denote the displacement from $\frA{1}$ to $\frL$, expressed in $\frA{1}$, provided by the camera. Then,
%\begin{equation} \label{eq:estimation_cameraequation}
%\mbf{d}^\frA{1}_{\frA{1}\frL}(\bm{\gamma}) = - (\RLA{1})^T \mbf{d}^\frL_{\frA{1}} = - (\RLB)^T \mbf{d}^\frL_{\frA{1}}.
%\end{equation}
%
%Putting together \eqref{eq:estimation_gpsbarometerequation} through \eqref{eq:estimation_cameraequation}, and considering $\aR$, $\aL$, $\daR$, and $\daL$, provided by sensors at the servos, lead to the nonlinear measurement equation $\mbf{y}_k = \bm{\pi}(\mbf{x}_k) + \mbf{v}_k$, where $\mbf{v}_k$ denotes measurement noise, and
%\begin{equation*}
%\bm{\pi}(\mbf{x}_k) = \left[\bm{\zeta}^T_\frB \,\; \bm{\eta}_\frB^T \,\; (\wBIB)^T \,\; (\mbf{d}^\frA{1}_{\frA{1}\frL})^T \,\; \aR \;\, \aL \;\, \daR \;\, \daL  \right]^T.
%\end{equation*}
%
%Finally, let $\setI_k$ denote the set of available measurements at time instant $k$, such that $\setI_k \subseteq \{1,2,\dots,16\}$, and $\iota_k$ denote the number of elements in $\setI_k$. Then, $\mbf{y}_k, \mbf{v}_k \in \setreal^{\iota_k}$, and %we have the time-switching nonlinear mapping
%\begin{equation} \label{eq:estimation_switchedmapping}
%\bm{\pi}^{[k]}(\mbf{x}_k) \triangleq \left[ \bm{\pi}(\mbf{x}_k)(i) \right]_{i \in \setI_k} \text{,}
%\end{equation}
%where $\bm{\pi}(\mbf{x}_k)(i)$ denotes the $i$-th row of $\bm{\pi}(\mbf{x}_k)$, and the brackets denote vertical concatenation.
%
%
%
%\subsubsection{Linearized model for state estimation} \label{sec:linearizedmodel}
%Since the method proposed in this section is formulated for linear systems, the state-space equations \eqref{eq:modeling_statespacenonlinear} and measurement mapping \eqref{eq:estimation_switchedmapping} are linearized around equilibrium values\footnote{Equilibrium values are used here since online evaluation of a time-varying model around trajectory values has demonstrated to be intractable.} $\mbf{x}^\text{eq}$, $\mbf{u}^\text{eq}$, $\mbf{d} = \bm{0}$, through first-order Taylor series expansion, and discretized by the zero-order-hold method, yielding to the disturbed switching linear discrete-time system%through first-order Taylor series expansion, leading to 
%\begin{equation}
%\begin{aligned} \label{eq:linearsystem0}
%\Delta \mbf{x}_{k} & = \mbf{A} \Delta \mbf{x}_{k-1} + \mbf{B} \Delta \mbf{u}_{k-1} + \mbf{F} \mbf{d}_{k-1} + \mbf{w}_{k-1} \text{,} \\
%\mbf{y}_{k} & = \mbf{H}^{[k]} \Delta \mbf{x}_{k} + \bm{\pi}^{[k]}(\mbf{x}^\text{eq}) + \mbf{v}_k,
%\end{aligned}
%\end{equation}
%where the process noise $\mbf{w}_{k}$ corresponds to unmodeled dynamics due to linearization and discretization, and the measurement noise $\mbf{v}_{k}$ now includes the nonlinearities of \eqref{eq:estimation_switchedmapping}. Moreover, $\Delta \mbf{x}_k \triangleq \mbf{x}_k - \mbf{x}^\text{eq}$ and $\Delta \mbf{u}_k \triangleq \mbf{u}_k - \mbf{u}^\text{eq}$, where $\mbf{A} \in \setrealmat{20}{20}$, $\mbf{B} \in \setrealmat{20}{4}$, $\mbf{F} \in \setrealmat{20}{3}$, and $\mbf{H}^{[k]} \in \setrealmat{\iota_k}{20}$ are the respective Jacobian matrices evaluated at the equilibrium values followed by the discretization procedure.
%
%For robust state estimation, the state vector is augmented with the external disturbances $\mbf{d}_k$, yielding the augmented dynamics
%\begin{equation} \label{eq:linearsystem}
%\begin{aligned}
%\begin{bmatrix} \Delta \mbf{x}_k \\ \mbf{d}_k \end{bmatrix} & {=} \begin{bmatrix} \mbf{A} & \mbf{F} \\ \zeros{3}{20} & \eye{3} \end{bmatrix} \begin{bmatrix} \Delta \mbf{x}_{k-1} \\ \mbf{d}_{k-1} \end{bmatrix} \!{+}\! \begin{bmatrix} \mbf{B} \\ \zeros{3}{4} \end{bmatrix} \Delta \mbf{u}_{k-1} {+}\! \begin{bmatrix} \mbf{w}_{k-1} \\ \tilde{\mbf{d}}_{k-1} \end{bmatrix}\!\!, \\
%\mbf{y}_k & = \begin{bmatrix} \mbf{H}^{[k]} & \zeros{\iota_k}{3} \end{bmatrix} \begin{bmatrix} \Delta \mbf{x}_k \\ \mbf{d}_k \end{bmatrix} + \bm{\pi}^{[k]}(\mbf{x}^\text{eq}) + \mbf{v}_k,
%\end{aligned}
%\end{equation}
%with $\tilde{\mbf{d}}_{k-1} \triangleq \mbf{d}_{k} - \mbf{d}_{k-1}$. 
%
%Accordingly, define $\bm{\nu}_k \triangleq \begin{bmatrix} \Delta \mbf{x}_k^T & \mbf{d}_k^T \end{bmatrix}^T$, $\bar{\mbf{w}}_k \triangleq \begin{bmatrix} \mbf{w}_{k}^T & \tilde{\mbf{d}}_{k}^T \end{bmatrix}^T$, and $\bar{\mbf{v}}_k \triangleq \bm{\pi}^{[k]}(\mbf{x}^\text{eq}) + \mbf{v}_k$. %This work assumes that $\bm{\nu}_0 \in X_0$, $\bar{\mbf{w}}_k \in W$ and $\bar{\mbf{v}}_k \in V_k$, where $X_0$, $W$, and $V_k$ are compact sets that can be expressed as constrained zonotopes. 
%Thus, the linear set-valued state estimation method is formulated in the next subsection.%straightforwardly through the techniques presented in Section \ref{sec:stateestimation}. % \subset \setreal^{23}$
%
%\subsection{Problem formulation} \label{sec:linearformulation}
%
%Constrained zonotopes are effectively used in \cite{Scott2016} for set-valued state estimation of linear systems, and in \cite{Raimondo2016} for active fault diagnosis. This section adapts the estimation method in \cite{Scott2016} for discrete-time switching systems. Consider the augmented linear discrete-time switching system described by \eqref{eq:linearsystem}, and let $\Anu$, $\Bnu$ and $\Hnu^{[k]}$ denote the associated matrices. Assuming bounded uncertainties $\bar{\mbf{w}}_{k} \in W_k$ and $\bar{\mbf{v}}_k \in V_k$, and $\bm{\nu}_0 \in X_0$\footnote{Note that $X_0 \subset \realset^{23}$, since this set is associated to the augmented state variables $\bm{\nu}_k$.}, where $X_0$, $W_k$ and $V_k$ are known compact sets, linear set-valued state estimation consists in computing enclosures $\bar{X}_k$ and $\hat{X}_k$ such that% $\bar{X}_k
%\begin{align}
%\bar{X}_k & \supseteq \{ \Anu \bm{\nu} + \Bnu \Delta \mbf{u}_{k-1} {+} \bar{\mbf{w}} : \bm{\nu} \in \hat{X}_{k-1}, \, \bar{\mbf{w}} \in W_{k-1} \}, \label{eq:predictionlinear0}\\
%\hat{X}_k & \supseteq \{ \bm{\nu} \in \bar{X}_k : \Hnu^{[k]} \bm{\nu} + \bar{\mbf{v}} = \mbf{y}_k, \, \bar{\mbf{v}} \in V_k \}, \label{eq:updatelinear0}
%\end{align}
%with \eqref{eq:predictionlinear0} referred to as \emph{prediction step}, and \eqref{eq:updatelinear0} as \emph{update step}. These enclosures can be obtained exactly with constrained zonotopes through \citep{Scott2016}
%\begin{align}
%\bar{X}_k & = \Anu \hat{X}_{k-1} \oplus \Bnu \Delta\mbf{u}_{k-1} \oplus W_{k-1} , \label{eq:predictionlinear}\\
%\hat{X}_k & = \bar{X}_k \cap_{\Hnu^{[k]}} (\mbf{y}_k \oplus (- V_k)), \label{eq:updatelinear}
%\end{align}
%using \eqref{eq:czlimage}--\eqref{eq:czintersection}. 
%
%
%%To clarify the advantages of using constrained zonotopes, we first present existing results for set-valued state estimation of linear discrete-time systems \cite{Scott2016}. Consider the discrete-time system \eqref{eq:system} with a linear mapping of the form
%In the following, we discuss the advantages of using constrained zonotopes for set-valued state estimation of the linear discrete-time switching system \eqref{eq:linearsystem}. The right-hand side of \eqref{eq:predictionlinear} cannot be computed using interval arithmetic without over-approximation due to wrapping (see Remark \ref{rem:intervaloverestimation}), either using a single or multiple intervals \citep{Kuhn1998} (in this discussion, we always assume that $\hat{X}_0$, $W_k$ and $V_k$ can be expressed using the class of sets being discussed). On the other hand, the equality in \eqref{eq:predictionlinear} can be achieved using zonotopes, constrained zonotopes, or general convex polytopes. However, this involves substantial computational cost for convex polytopes, while the operations for zonotopes and constrained zonotopes are very efficient and result in only a linear increase in the complexity of the set representation \citep{Combastel2003,Scott2016}.
%
%On the other side, the intersection in \eqref{eq:updatelinear} can not be computed exactly using zonotopes, and must be over-approximated \citep{Alamo2005a,Le2013}. As a consequence, the enclosures of the system states obtained after many iterations of prediction and update may be quite conservative using zonotopes. Zonotope bundles \citep{Althoff2011} can be used to compute \eqref{eq:updatelinear} exactly and inexpensively, but the prediction step \eqref{eq:predictionlinear} is done conservatively. However, with constrained zonotopes both \eqref{eq:predictionlinear} and \eqref{eq:updatelinear} are easily computed using \eqref{eq:czlimage}--\eqref{eq:czintersection}. Moreover, iterated computations of \eqref{eq:predictionlinear} and \eqref{eq:updatelinear} result in only a linear increase in the complexity of the CG-rep \eqref{eq:czdefinition}. As with zonotopes, this can be effectively addressed using \emph{order reduction} algorithms \citep{Kopetzki2017,Scott2018} that over-approximate a constrained zonotope by another with lower complexity. Efficient methods for reducing the number of generators and constraints of the CG-rep \eqref{eq:czdefinition} with reasonable conservativeness were proposed in \cite{Scott2016}, which we refer to in this doctoral thesis as \emph{generator reduction} and \emph{constraint elimination} algorithms.
%
%\subsection{Minimum-variance feedback} \label{sec:minimumvariance}
%
%
%Despite the accuracy and low computational burden of the method described by \eqref{eq:predictionlinear}--\eqref{eq:updatelinear}, to perform state-feedback control with estimated states one must choose a point satisfying $\hat{\bm{\nu}}_k \in \hat{X}_k$. Therefore, we propose an optimal choice according to a \emph{minimum-variance criterion}, which is one of the central contributions of this doctoral thesis, and can be straightforwardly adapted to more general classes of linear discrete-time switching dynamical systems.
%
%The proposed criterion is based on the well-known Kalman filter algorithm \citep{Simon2006}. Let $\mbf{P}^{\nu}_k$, $\mbf{P}^{w}_k$, and $\mbf{P}^{v}_k$, denote the covariance matrices of the estimation error $\bm{\nu}_k - \hat{\bm{\nu}}_k$, process noise $\bar{\mbf{w}}_k$, and measurement noise $\bar{\mbf{v}}_k$, respectively. Consider the constrained optimization problem
%\begin{gather}
%\underset{\mbf{N}_k}{\min} ~ \text{trace}\{\mbf{P}^{\nu}_k\} \quad \text{s.t.} \quad \hat{\bm{\nu}}_k \in \hat{X}_k, \label{eq:minCKF}
%\end{gather}
%where $\mbf{N}_k$ is the Kalman gain, and $\hat{\bm{\nu}}_k$ is given according to the correction step% of Kalman filter,
%\begin{equation} \label{eq:CKF_correction}
%\hat{\bm{\nu}}_{k} = \bar{\bm{\nu}}_{k} + \mbf{N}_k (\mbf{y}_k - (\Hnu^{[k]} \bar{\bm{\nu}}_{k} + \bm{\pi}^{[k]}(\mbf{x}^\text{eq}))),
%\end{equation}
%with $\bar{\bm{\nu}}_{k} = \mbf{A}_{\bm{\nu}} \hat{\bm{\nu}}_{k-1} + \mbf{B}_{\bm{\nu}} \Delta \mbf{u}_{k-1}$. Moreover,
%\begin{equation} \label{eq:CKF_covariance}
%%\begin{aligned}
%\mbf{P}^{\bm{\nu}}_{k} = (\eye{23} - \mbf{N}_k \mbf{H}^{[k]}_{\bm{\nu}}) \bar{\mbf{P}}^{\bm{\nu}}_{k} (\eye{23} - \mbf{N}_k \mbf{H}^{[k]}_{\bm{\nu}})^T 
%+ \mbf{N}_k \mbf{P}^{{\mbf{v}}}_k \mbf{N}_k^T,
%%\end{aligned}
%\end{equation}
%where $\bar{\mbf{P}}^{\bm{\nu}}_{k} = \mbf{A}_{\bm{\nu}} \mbf{P}^{\bm{\nu}}_{k-1} \mbf{A}_{\bm{\nu}}^T + \mbf{P}^{\mbf{w}}_k$. Considering Property \ref{prop:isemptybelongsto} and $\hat{X}_k = \{\mbf{G}_x, \mbf{c}_x, \mbf{A}_x, \mbf{b}_x \}$, the optimization problem \eqref{eq:minCKF} is rewritten as a quadratic program with linear constraints,
%\begin{align}
%\underset{\mbf{N}_k, \bm{\xi}}{\min} & ~ \text{trace}\{\mbf{P}^{\nu}_k\} \label{eq:CKFQP}\\
%\text{s.t.} & ~ \bar{\bm{\nu}}_{k} + \mbf{N}_k (\mbf{y}_k - (\Hnu^{[k]} \bar{\bm{\nu}}_{k} + \bm{\pi}^{[k]}(\mbf{x}^\text{eq}))) = \mbf{c}_x + \mbf{G}_x \bm{\xi}, \nonumber\\
%& \ninf{\bm{\xi}} \leq 1, \quad \mbf{A}_x \bm{\xi} = \mbf{b}_x,\nonumber
%\end{align}
%with $\mbf{P}^{\nu}_k$ given by \eqref{eq:CKF_covariance}. The minimum-variance choice $\hat{\bm{\nu}}_k$ is then obtained by solving \eqref{eq:CKFQP}, and computing \eqref{eq:CKF_correction} afterwards. The optimization problem \eqref{eq:CKFQP} can be regarded as \emph{constrained Kalman filtering}, in which divergence issues are not present since $\hat{\bm{\nu}}_k \in \hat{X}_k$ is guaranteed by construction.
%
%
%\subsection{Path tracking control}
%
%
%\subsubsection{Linearized parameter-varying error dynamics} \label{sec:lpvmodel}
%
%The tilt-rotor UAV with suspended load is an underactuated mechanical system with four control inputs. For path tracking of the suspended load, the position $\bm{\zeta} = [x \; y \; z]^T$ and yaw angle $\psi$ of the load are chosen to be regulated. Let $\mbf{q}^\text{tr} = [\bm{\zeta}^\text{tr} \,\; \bm{\eta}^\text{tr} \,\; \bm{\gamma}^\text{eq} \,\; \alpha^\text{eq}_\text{R} \,\; \alpha^\text{eq}_\text{L}]$, with $\bm{\eta}^\text{tr} = [\phi^\text{eq} \,\; \theta^\text{eq} \,\; \psi^\text{tr}]$, where `tr' denotes trajectory values. Assuming $\psi^\text{tr}$ constant, the linearized error dynamics of \eqref{eq:modeling_statespacenonlinear} are given by $\delta \dot{\mbf{x}} = \mbf{A}_\text{c}(t) \delta \mbf{x} + \mbf{B}_\text{c} \delta \mbf{u} + \mbf{F}_\text{c} \mbf{d}$, where $\delta \mbf{x} \triangleq \mbf{x} - \mbf{x}^\text{tr}$, $\delta \mbf{u} \triangleq \mbf{u} - \mbf{u}^\text{tr}$, $\mbf{x}^\text{tr} \triangleq [(\mbf{q}^\text{tr})^T \;\, (\dot{\mbf{q}}^\text{tr})^T]^T$, and $\mbf{A}_\text{c}(t)$ is a function of $\mbf{u}^\text{tr}$ \citep{Rego2016c}.
%
%Considering a feasible reference trajectory, the desired input can be obtained from \eqref{eq:modeling_statespacenonlinear} as follows:
%\begin{equation} \label{eq:feedforward}
%\mbf{u}^\text{tr} = \mbf{L}_\text{in}(\mbf{q}^\text{tr})^+ \! \left[ \mbf{M}(\mbf{q}^\text{tr}) \ddot{\mbf{q}}^\text{tr} {+} (\mbf{C}(\mbf{q}^\text{tr}, \dot{\mbf{q}}^\text{tr}) {+} \mbf{L}_\text{fr}) \dot{\mbf{q}}^\text{tr} {+} \mbf{g}(\mbf{q}^\text{tr}) \right],
%\end{equation}
%where $\mbf{L}_\text{in}(\mbf{q}^\text{tr})^+$ denotes the pseudo-inverse of $\mbf{L}_\text{in}(\mbf{q}^\text{tr})$. It can be shown that \eqref{eq:feedforward} is a function only of the accelerations $\ddot{\bm{\zeta}}^\text{tr}$ \citep{Rego2016c}. By defining the vector of parameters $\bm{\sigma} \triangleq \ddot{\bm{\zeta}}^\text{tr}$, we have that $\mbf{u}^\text{tr}(t) \triangleq \mbf{u}(\bm{\sigma})$, which is affine in $\bm{\sigma}$. Then, substituting \eqref{eq:feedforward} in $\mbf{A}_\text{c}(t)$ yields the parameter-varying matrix $\mbf{A}_\text{c}(\bm{\sigma})$, which is affine in $\bm{\sigma}$ since \eqref{eq:modeling_statespacenonlinear} is affine in $\mbf{u}$.
%
%For an improved trajectory tracking and rejection of constant disturbances, the state vector $\delta\mbf{x}$ is augmented with integral actions over the regulated variables, as $\bm{\chi} \triangleq [\delta \mbf{x}^T \,\; \smallint (\bm{\zeta}-\bm{\zeta}^\text{tr})^T \,\; \smallint (\psi - \psi^\text{tr})]^T$. The resulting augmented dynamics are then discretized through Euler approximation\footnote{The Euler approximation is used here in order to obtain a discrete-time LPV system. On the other hand, the zero-order-hold method is used in \eqref{eq:linearsystem0} for reduced discretization error. }, yielding the discrete-time, augmented LPV error dynamics
%\begin{equation} \label{eq:LPVsystem}
%\bm{\chi}_{k+1} = \Achi (\bm{\sigma}) \bm{\chi}_{k} + \Bchi \delta \mbf{u}_{k} + \Fchi \mbf{d}_{k} \text{,}
%\end{equation}
%with $\Achi(\bm{\sigma}) \in \setrealmat{24}{24}$, $\Bchi \in \setrealmat{24}{4}$ and $\Fchi \in \setrealmat{24}{3}$. Finally, assuming bounded trajectory accelerations, the LPV system \eqref{eq:LPVsystem} can be rewritten in a convex polytopic representation, by defining $\Achi(\bm{\sigma}) \triangleq \Achi(\tilde{\bm{\sigma}}) = \sum_{i=1}^{8} \tilde{\sigma}_i\Achi^i$, with $\Achi^i$ denoting the $i$-th vertex of $\Achi(\tilde{\bm{\sigma}})$, and $\sum_{i=1}^{8} \tilde{\sigma}_i = 1$. Resulting errors from linearization and discretization are taken into account in this section as unmodeled dynamics. Note that the LPV dynamics \eqref{eq:LPVsystem} describe the behavior of the tracking error $\delta \mbf{x}$ augmented with integral actions, while the time-invariant linear dynamics \eqref{eq:linearsystem} describe the evolution of the system states $\mbf{x}$ around equilibrium values augmented with the external disturbances.
%
%\subsubsection{Discrete-time mixed $\mathcal{H}_2/\mathcal{H}_\infty$ control with pole placement constraints}
%
%The aim of the proposed controller is to perform robust trajectory tracking of the load with stabilization of the tilt-rotor UAV, with estimation provided by the novel method presented in Section \ref{sec:minimumvariance}. The desired accelerations for the load are required to be smooth and bounded. The present method extends the approach in \cite{Gahinet1996} for discrete-time linear systems. Let
%\begin{equation*}
%\begin{aligned}
%\mbf{z}_k^{(2)} & = \mbf{H}_{\mbf{z}} \bm{\chi}_k + \mbf{D}_{\mbf{zu}} \delta\mbf{u}_k \text{,} \\
%\mbf{z}_k^{(\infty)} & = \mbf{H}_{\mbf{z}} \bm{\chi}_k + \mbf{D}_{\mbf{zu}} \delta\mbf{u}_k + \mbf{D}_{\mbf{zd}} \mbf{d}_k \text{,}
%\end{aligned}
%\end{equation*}
%where $\mbf{H}_{\mbf{z}} \in \setrealmat{n_z}{24}$, $\mbf{D}_{\mbf{zu}} \in \setrealmat{n_z}{4}$, $\mbf{D}_{\mbf{zd}} \in \setrealmat{n_z}{3}$. %
%%
%Let $\bm{\Psi}^{(2)}_{\mbf{d}{\mbf{z}}}(\zdomain)$ and $\bm{\Psi}^{(\infty)}_{\mbf{d}{\mbf{z}}}(\zdomain)$ denote the discrete-time transfer matrices from $\mbf{d}_k$ to $\mbf{z}_k^{(2)}$ and $\mbf{d}_k$ to $\mbf{z}_k^{(\infty)}$, and $\| \bm{\Psi}^{(2)}_{{\mbf{d}}\mbf{z}} (\zdomain) \|_2$ and $\| \bm{\Psi}^{(\infty)}_{{\mbf{d}}{\mbf{z}}} (\zdomain) \|_\infty$ be the corresponding $\mathcal{H}_2$ and $\mathcal{H}_\infty$ norms, respectively. Given the state-feedback control law $\mbf{u}_k = - \mbf{K} \bm{\chi}$, the gain matrix $\mbf{K}$ that minimizes $\text{trace}({\bm{\Omega}}) > \| \bm{\Psi}^{(2)}_{{\mbf{d}}\mbf{z}} \|_2^2$ while guaranteeing an upper-bound $\tilde{\gamma} > \| \bm{\Psi}^{(\infty)}_{{\mbf{d}}{\mbf{z}}} \|_\infty^2$, is given by $\mbf{K} = -\mbf{Y}\mbf{X}^{-1}$, where $\mbf{Y}$ and $\mbf{X}$ are the solution of the optimization problem %\cite{Oliveira2002}
%\begin{gather}
%\underset{\mbf{P},\mbf{X},\mbf{Y},\bm{\Omega}}{\min} ~ \text{trace}\{\bm{\Omega}\} \quad \text{s.t.} \label{eq:h2hinf}\\
%\begin{bmatrix}
%\bm{\Omega} & \mbf{H}_{\mbf{z}} \mbf{X} + \mbf{D}_{\mbf{zu}} \mbf{Y} \\
%* & \mbf{X} + \mbf{X}^T - \mbf{P}
%\end{bmatrix} > 0, \nonumber\\
%\begin{bmatrix}
%\mbf{P} & \Achi^i \mbf{X} + \mbf{B}_{\bm{\chi}} \mbf{Y} & \mbf{F}_{\bm{\chi}} & \zeros{24}{n_z} \\
%* & \mbf{X} + \mbf{X}^T - \mbf{P} & \zeros{24}{3} & \mbf{X}^T \mbf{H}_{\mbf{z}}^T + \mbf{Y}^T \mbf{D}_{\mbf{zu}}^T \\
%* & * & \eye{3} & \mbf{D}_{\mbf{zd}}^T \\
%* & * & * & \tilde{\gamma} \eye{n_z} 
%\end{bmatrix} > 0, \nonumber
%\end{gather}
%with $i = 1,2,\dots,8$, $\mbf{P} = \mbf{P}^T > 0$, $\mbf{X} > 0$ and $\bm{\Omega} = \bm{\Omega}^T$.
%
%To ensure transient properties for the closed-loop system, additional constraints are imposed to pole placement. Seeking minimum and maximum settling times, maximum percentage overshoot, and also to avoid ringing, three regions are of interest: $\mathbb{D}_1 \triangleq \{ \zdomain \in \mathbb{C} : \real{\zdomain} > \deps \geq 0\}$, $\mathbb{D}_2 \triangleq \{ \zdomain \in \mathbb{C} : 0 \leq |\zdomain| < \varpi \}$ and $\mathbb{D}_3 \triangleq \{ \zdomain \in \mathbb{C} : 0 \leq |\imag{\zdomain}| < \tau \}$. The eigenvalues of $\Achi(\bm{\sigma}) - \Bchi \mbf{K}$ belong to $\bigcap_{j=1}^{3} \mathbb{D}_j$ iff \citep{Rego2018c}
%\begin{gather*}
%\mbf{X} (\Achi^i)^T + \Achi^i \mbf{X} + \mbf{Y}^T\mbf{B}_{\bm{\chi}}^T + \mbf{B}_{\bm{\chi}}\mbf{Y} - 2\varepsilon \mbf{X} > 0, \nonumber \\
%\begin{bmatrix}
%-\varpi \mbf{X} & \Achi^i \mbf{X} + \mbf{B}_{\bm{\chi}} \mbf{Y} \\
%* & -\varpi \mbf{X}
%\end{bmatrix} < 0, \nonumber \\
%\begin{bmatrix} -2 \tau \mbf{X} ~& ~\mbf{X} (\Achi^i)^T \!{-} \Achi^i \mbf{X} + \mbf{Y}^T \Bchi^T {-} \Bchi \mbf{Y} \\ * & - 2 \tau \mbf{X} \end{bmatrix} < 0. \nonumber
%\end{gather*}
%
%Finally, the control signals applied to \eqref{eq:modeling_statespacenonlinear} are obtained from $\mbf{u}_k = \delta \mbf{u}_k + \mbf{u}_k^\text{tr} {=} -\mbf{K}\hat{\bm{\chi}}_k + \mbf{u}_k^\text{tr}$, with $\mbf{u}_k^\text{tr}$ given by \eqref{eq:feedforward}, where the estimated states $\hat{\bm{\chi}}_k$ are retrieved from $\hat{\bm{\nu}}_k$ according to the definitions of the state vectors $\bm{\nu}_k$ and $\bm{\chi}_k$.
%
%\subsection{Numerical experiments} \label{sec:estimationexamples}
%
%This section evaluates the performance of the proposed method through numerical experiments.
%
%The experiment is performed in the ProVANT simulator platform, using a Computer Aided Design (CAD) model of the system. The model parameters are shown in Table\footnote{Parameter uncertainties can be considered immediately through $\bar{\mbf{w}}_k$, $\bar{\mbf{v}}_k$.} \ref{tab:results_modelparameters}, where $m_j$ is the mass of each rigid body, $j \in \{ \mathcal{L}, 1,2,3\}$, $\Ii{j}$ is the inertia tensor, $\hat{\mbf{g}}$ is the gravity acceleration vector in $\frI$, $k_\tau$ and $b$ are drag torque parameters obtained experimentally, $\lambdaR,\lambdaL \in \{-1,1\}$ are given according to the direction of rotation of the propellers, $\mu_\gamma$ and $\mu_\alpha$ are constant parameters associated with viscous friction \citep{Rego2018c}. These model parameters yield the equilibrium point
%\begin{equation*}% \label{eq:results_equilibriumpoint}
%\begin{aligned}
%\mbf{q}^{\text{eq}} = &~
%[ \zeros{1}{6} \;\, 0.000132 \;\, 0.01396 \;\, 0.01401 \;\, 0.01381]^T \text{,} \\
%\mbf{u}^{\text{eq}} = &~
%[ 11.7323 \;\, 11.7676 \;\, 4.1389{\cdot}10^{-7} \;\, 1.0121{\cdot}10^{-5}]^T \text{.}
%\end{aligned}
%\end{equation*}
%
%\begin{table}[!ht]
%	\centering
%	%\scriptsize
%	\caption{Model parameters of the system.} \vspace{-3mm}
%	\begin{tabular}{c c}
%		Parameter & Value \\ \hline
%		$(\mL,m_1,m_2,m_3)$ & $(0.5,1.7068,0.08978,0.08978)$ Kg \\
%		%$m_1$ & 1.70682 Kg \\
%		%$m_2$, $m_3$ & $0.0897833$ Kg \\
%		$(\dLA{1},\dAB{1})$ & $([ 0 \; 0 \; 0.5 ]^T,[ 0 \; 0 \; 0.119 ]^T)$ m\\
%		%$\dAB{1}$ & $[ 0 \; 0 \; 0.119 ]^T$ m\\
%		$\dBC{1}$ & $[ \text{-}0.004321 \; 0.000601 \; \text{-}0.045113]^T$ m\\
%		$\dBA{2}$ & $[  0 \; \text{-}0.275433 \; 0.056262 ]^T$ m\\
%		$\dBA{3}$ & $[  0 \; 0.275433 \; 0.056261 ]^T$ m\\
%		$(\dAC{2}{2},\dAC{3}{3})$ & $([  0 \; 0 \; 0.05647 ]^T, [  0 \; 0 \; 0.05648 ]^T)$ m\\
%		%$\dAC{3}{3}$ & $[  0 \; 0 \; 0.05648 ]^T$ m\\		
%		%		$\IL$ & $0.000002645 \cdot \eye{3}$ Kg$\cdot$m$^2$ \\
%		$\IL$ & $8.333 {\cdot} 10^{-6} {\cdot} \eye{3} $ Kg$\cdot$m$^2$ \\
%		$\Ii{1}$ & $\begin{bmatrix} 4047.04 & 0.8606 & 9.6577 \\ * &  881.62 & \text{-}0.8731 \\ * & * & 4173.18 \end{bmatrix} {\cdot} 10^{-6}$ Kg${\cdot}$m$^2$ \\
%		$\Ii{2},\Ii{3}$ & $\text{diag} (335.74, 335.74, 641.59) {\cdot} 10^{-6}$Kg${\cdot}$m$^2$ \\
%		%$\Ii{3}$ & $\begin{bmatrix} 335.74 & 0 & 0 \\ * & 335.74 & 0 \\ * & * & 641.59 \end{bmatrix} {\cdot} 10^{-6}$Kg${\cdot}$m$^2$ \\		
%		$\hat{\mbf{g}}$ & $[ 0\;\, 0 \;\, \text{-}9.81]^T$ m/s$^2$ \\
%		$(k_\tau, b)$ &  $(1.7 {\cdot} 10^{-7}$ N$\cdot$m$\cdot$s$^2, 9.5 {\cdot} 10^{-6}$ N$\cdot$s$^2)$\\
%		%$b$ & $9.5 \cdot 10^{-6}$ N$\cdot$s$^2$\\
%		$(\lambdaR, \lambdaL, \beta)$ & $(1, \text{-}1, 5^\text{o})$\\
%		%$\beta$ & $5^\text{o}$ \\
%		$\mu_\gamma$, $\mu_\alpha$ & $0.005$ N${\cdot}$m/(rad/s) \\
%		\hline
%	\end{tabular}
%	\normalsize
%	\label{tab:results_modelparameters}
%\end{table}
%
%The desired trajectory is composed of several paths, with $\psi^\text{tr}$ = 0 rad. The sensor parameters are shown in Table \ref{tab:sensorparameters}.
%
%\begin{table}[!ht]
%	\footnotesize
%	\centering
%	%\caption{Parameters of the sensors used in the experiment.}
%	\caption{Parameters of the sensors.} \vspace{-3mm}
%	%\caption{Measurement parameters.}
%	%\caption{}
%	\begin{tabular}{c c c c c}% \hline
%		Sensor & $\mathbb{I}$ & Noise bound & Sampling & PDF \\ \hline
%		GPS & $\{1,2\}$ & $\pm\!\!$ $0.15\!$ m & $120\!$ ms & Gauss.\\ %\hline
%		Barometer & $\{3\}$ & $\pm\!\!$ $0.51\!$ m & $12\!$ ms & Gauss.\\ %\hline
%		\multirow{2}{*}{IMU} & $\{4,5,6\}$ & $\pm\!\!$ $2.618 {\cdot} 10^{-3}\!$ rad & \multirow{2}{*}{$12\!$ ms} & \multirow{2}{*}{Gauss.} \\
%		& $\{7,8,9\}$ & $\pm\!\!$ $16.558 {\cdot} 10^{-3}\!$ rad/s & \\ %\hline
%		\multirow{2}{*}{Camera} & $\{10,11\}$ & $\pm\!\!$ $0.005\!$ m & \multirow{2}{*}{$24\!$ ms} & \multirow{2}{*}{Unif.} \\
%		& $\{12\}$ & $\pm\!\!$ $0.02\!$ m & \\		                           	                           
%		\multirow{2}{*}{Servos} & $\{13,14\}$ & $\pm\!\!$ $5.67 {\cdot} 10^{-3}\!$ rad & \multirow{2}{*}{$12\!$ ms} & \multirow{2}{*}{Unif.} \\
%		& $\{15,16\}$ & $\pm\!\!$ $0.50772\!$ rad/s & \\		                           
%		\hline
%	\end{tabular} \normalsize
%	\label{tab:sensorparameters}
%\end{table}
%
%The optimization problem \eqref{eq:h2hinf} was solved using SDPT3, with $\varepsilon = 0.55$, $\varpi = 0.994$, $\tau = 0.3$, $\tilde{\gamma} = 81$, $\ddot{x}^\text{tr}(t) \in [-0.5,\; 0.5]$, $\ddot{y}^\text{tr}(t) \in [-0.5,\; 0.5]$, $\ddot{z}^\text{tr}(t) \in [-0.3,\; 0.3]$,
%\begin{align*}% \label{eq:Cz}
%\mbf{H}_{\mbf{z}} & = \text{diag} \Big(\tfrac{\sqrt{10}}{2} \ones{3}{1},\tfrac{\sqrt{0.5}}{\pi/2}\ones{2}{1},\tfrac{\sqrt{5}}{\pi},\tfrac{2}{\pi}\ones{2}{1},\tfrac{0.2}{\pi}\ones{2}{1},\\
%& \quad \tfrac{1}{2}\ones{3}{1},\tfrac{3}{\pi}\ones{2}{1},\tfrac{4}{\pi},\tfrac{\sqrt{5}}{3\pi}\ones{2}{1},\tfrac{0.1}{3\pi}\ones{2}{1},\sqrt{5}{\cdot}\ones{3}{1},\sqrt{0.1}\Big) \text{,} \\
%\mbf{D}_{\mbf{zu}} & = \begin{bmatrix} \text{diag}\left(
%\frac{\sqrt{750}}{30-\infR^\text{eq}},\frac{\sqrt{750}}{30-\infL^\text{eq}},  \frac{\sqrt{5000}}{2-\intauaR^\text{eq}} \right)& \zeros{3}{1} \\
%\zeros{2}{3} & \zeros{2}{1} \\
%\zeros{1}{3} & \frac{\sqrt{5000}}{2-\intauaL^\text{eq}} \\
%\zeros{18}{3} & \zeros{18}{1}
%\end{bmatrix},\\
%\mbf{D}_{\mbf{zd}} & = [
%\zeros{3}{10} \;\,
%\eye{3} \;\,
%\mbf{V}^T \;\,
%0.5{\cdot}\ones{3}{1}\;\,
%\mbf{V}^T \;\,
%\zeros{3}{2} \;\,
%\eye{3} \;\,
%0.5{\cdot}\ones{3}{1}
%]^T,
%\end{align*}
%%$\mbf{V} \triangleq \begin{bmatrix} 0 & 1 & 0 \\ 1 & 0 & 0 \end{bmatrix}$\footnote{$\ones{n}{m}$ is an $n$ by $m$ matrix of ones.}. These matrices were adjusted empirically using the Bryson's method \citep{Johnson1987} as starting point. The constrained zonotopes $X_0$, $W_k$, and $V_k$, were chosen as $X_0 = \{\mbf{G}_{x_0}, [(\bm{\zeta}^\text{tr}_0)^T \; \zeros{1}{20}]^T\}$, $W_k = \{\mbf{G}_{w}, \zeros{23}{1}\}$ and $V_k = \{\mbf{G}_{v},\bm{\pi}(\mbf{x}^\text{eq})\}$, with $\mbf{G}_{x_0} = \text{diag} ( 0.5 {\cdot} \ones{3}{1},$ $ 0.02, $ $ 0.02, $ $\pi/180, $ $1.5 {\cdot} |\gamma_1^\text{eq}|, $ $1.5 {\cdot} |\gamma_2^\text{eq}|, $ $1.5 {\cdot} |\aR^\text{eq}|, $ $1.5 {\cdot} |\aL^\text{eq}|, $ $0.02 {\cdot} \ones{13}{1})$, $\mbf{G}_w = $ $\text{diag} (10^{-4} {\cdot} \ones{13}{1}, $ $0.01 {\cdot} \ones{3}{1}, $ $0.05 {\cdot} \ones{2}{1}, $ $10^{-4} {\cdot} \ones{2}{1}, $ $0.01 {\cdot} \ones{3}{1})$, $\mbf{G}_v = $ $\text{diag} (0.18 {\cdot} \ones{2}{1}, $ $0.612, $ $3.1416\ten{-3}{\cdot}\ones{2}{1}, $ $0.03, $ $19.872 {\cdot} 10^{-3} {\cdot} \ones{2}{1}, $ $0.24, $ $0.006 {\cdot} \ones{2}{1}, $ $0.06 , $  $6.8067 {\cdot} 10^{-3} {\cdot} \ones{2}{1}, $ $0.6093 {\cdot} \ones{2}{1})$. These were adjusted empirically to accommodate linearization errors. The number of generators and constraints of $\hat{X}_k$ were limited to 50 and 10, respectively, using the complexity reduction methods in \cite{Scott2016}. The optimal estimate $\hat{\bm{\nu}}_k \in \hat{X}_k$ was obtained considering $\mbf{P}^\nu_0 = \eye{23}$, with $\hat{\bm{\nu}}_0$ as the center of the interval hull\footnote{The interval hull is computed as in Proposition \ref{prope:ihull}.} of $\hat{X}_0 = X_0 \cap_{\Hnu^{[0]}}(\mbf{y}_0 \oplus (- V_0))$, $\mbf{P}^w_k = \frac{1}{3} \mbf{G}_w^2$, and $\mbf{P}^v_k = \frac{1}{3} \mbf{G}_v^2$. The quadratic program \eqref{eq:CKFQP} was solved using CPLEX \citep{cplex}. For comparison, estimation results using the zonotope-based algorithm of \cite{Rego2018c} are also presented, with same $X_0$, $W_k$, and $V_k$, and number of generators limited to 1725. The initial state is $\mbf{x}_0 = [0\,\; 0\,\; 1 \,\; \zeros{1}{13}]^T$.
%$\mbf{V} \triangleq \begin{bmatrix} 0 & 1 & 0 \\ 1 & 0 & 0 \end{bmatrix}$\footnote{$\ones{n}{m}$ is an $n$ by $m$ matrix of ones.}. These matrices were adjusted empirically using the Bryson's method \citep{Johnson1987} as starting point. For comparison with results obtained using the zonotope-based algorithm of \cite{Rego2018c}, the constrained zonotopes $X_0$, $W_k$, and $V_k$, were chosen as the zonotopes $X_0 = \{\mbf{G}_{x_0}, [(\bm{\zeta}^\text{tr}_0)^T \; \zeros{1}{20}]^T\}$, $W_k = \{\mbf{G}_{w}, \zeros{23}{1}\}$ and $V_k = \{\mbf{G}_{v},\bm{\pi}(\mbf{x}^\text{eq})\}$, with $\mbf{G}_{x_0} = \text{diag} ( 0.5 {\cdot} \ones{3}{1},$ $ 0.02, $ $ 0.02, $ $\pi/180, $ $1.5 {\cdot} |\gamma_1^\text{eq}|, $ $1.5 {\cdot} |\gamma_2^\text{eq}|, $ $1.5 {\cdot} |\aR^\text{eq}|, $ $1.5 {\cdot} |\aL^\text{eq}|, $ $0.02 {\cdot} \ones{13}{1})$, $\mbf{G}_w = $ $\text{diag} (10^{-4} {\cdot} \ones{13}{1}, $ $0.01 {\cdot} \ones{3}{1}, $ $0.05 {\cdot} \ones{2}{1}, $ $10^{-4} {\cdot} \ones{2}{1}, $ $0.01 {\cdot} \ones{3}{1})$, $\mbf{G}_v = $ $\text{diag} (0.18 {\cdot} \ones{2}{1}, $ $0.612, $ $3.1416\ten{-3}{\cdot}\ones{2}{1}, $ $0.03, $ $19.872 {\cdot} 10^{-3} {\cdot} \ones{2}{1}, $ $0.24, $ $0.006 {\cdot} \ones{2}{1}, $ $0.06 , $  $6.8067 {\cdot} 10^{-3} {\cdot} \ones{2}{1}, $ $0.6093 {\cdot} \ones{2}{1})$. These were adjusted empirically to accommodate linearization errors. The number of generators and constraints of $\hat{X}_k$ were limited to 50 and 10, respectively, using Methods \ref{meth:czgenred} and \ref{meth:czconelim} in the Appendix, while the number of generators of the zonotopes was limited to 1725 using Method \ref{meth:genredA}. The optimal estimate $\hat{\bm{\nu}}_k \in \hat{X}_k$ was obtained considering $\mbf{P}^\nu_0 = \eye{23}$, with $\hat{\bm{\nu}}_0$ as the center of the interval hull\footnote{The interval hull is computed as in Proposition \ref{prope:ihull}.} of $\hat{X}_0 = X_0 \cap_{\Hnu^{[0]}}(\mbf{y}_0 \oplus (- V_0))$, $\mbf{P}^w_k = \frac{1}{3} \mbf{G}_w^2$, and $\mbf{P}^v_k = \frac{1}{3} \mbf{G}_v^2$. The quadratic program \eqref{eq:CKFQP} was solved using CPLEX \citep{cplex}. The initial state is $\mbf{x}_0 = [0\,\; 0\,\; 1 \,\; \zeros{1}{13}]^T$.
%
%The trajectories performed by the load and the UAV are shown in Fig. \ref{fig:trajectory}, and the tracking error is shown in Fig. \ref{fig:error}. External forces were added and removed from the load, as filtered steps with magnitude 0.5 N. The estimation error of the regulated variables is shown in Fig. \ref{fig:estimation}, along with confidence limits (interval hull), and results using the strategy of \cite{Rego2018c}. Sharper bounds are observed for the proposed method, which demonstrate the reduced conservatism of constrained zonotopes. This is a direct result of the exact intersection \eqref{eq:updatelinear}, which was severely over-estimated by zonotopic enclosures even with a much higher number of generators. Note that the confidence limits are not symmetric, since the optimal choice $\bm{\nu}_k$ is not the geometric center of $\hat{X}_k$ in general. Moreover, since outliers can happen due to unmodeled dynamics, if $\hat{X}_k = \emptyset$ (verified through Property \ref{prop:isemptybelongsto}), $\bar{X}_k$ was used instead. The path tracking was performed successfully, as shown by the tracking error of the regulated variables, which remained bounded during the experiment\footnote{A video of the performed experiment is available in https://youtu.be/x-oJNQqdavs .}. The control signals applied to the aircraft are shown in Fig. \ref{fig:inputs}. To conclude, experiments were conducted with an alternative feedback $\hat{\bm{\nu}}_k \in \hat{X}_k$, as the center of the interval hull of $\hat{X}_k$. Although less computationally demanding \citep{Scott2016}, such choice demonstrated to be substantially noisy, destabilizing the closed-loop system.
%
%\begin{figure}[!ht]
%	\centering{
%		%\def\svgwidth{0.9\columnwidth}
%		\def\svgwidth{0.6\columnwidth}
%		{\scriptsize\import{Figures_CDC/Figures/}{fig_trajectory.pdf_tex}}%\vspace{-1mm}
%		\caption{Trajectories performed by the UAV and the load.}\label{fig:trajectory}}
%	%\vspace{-3mm}
%\end{figure}
%
%\begin{figure}[!ht]
%	\centering{
%		%\def\svgwidth{0.6\textwidth}
%		%\def\svgwidth{\columnwidth}
%		\def\svgwidth{0.7\columnwidth}
%		{\scriptsize\import{Figures_CDC/Figures/}{fig_error.pdf_tex}}%\vspace{-1mm}
%		\caption{Tracking error of the regulated variables.}\label{fig:error}}
%	%\vspace{-3mm}
%\end{figure}
%
%\begin{figure}[!ht]
%	\centering{
%		%\def\svgwidth{0.6\textwidth}
%		%\def\svgwidth{\columnwidth}
%		\def\svgwidth{0.7\columnwidth}
%		{\scriptsize\import{Figures_CDC/Figures/}{fig_estimation_v3.pdf_tex}}%\vspace{-1mm}
%		\caption{Estimation error of the regulated variables, along with confidence limits (outer lines). Dotted lines denote results from the algorithm of \cite{Rego2018c}.}\label{fig:estimation}}
%	%\vspace{-3mm}
%\end{figure}
%
%\begin{figure}[!ht]
%	\centering{
%		%\def\svgwidth{0.6\textwidth}
%		\def\svgwidth{0.7\columnwidth}
%		{\scriptsize\import{Figures_CDC/Figures/}{fig_inputs.pdf_tex}}%\vspace{-1mm}
%		\caption{Control signals applied to the UAV.}\label{fig:inputs}}
%	%\vspace{-3mm}
%\end{figure}
%
%
%%\subsection{Conclusion}
%%
%%This paper addressed path tracking of a suspended load by a tilt-rotor UAV, based on set-valued state estimation by constrained zonotopes, to accurately estimate the load position and orientation, considering sensors with different sampling times, and unknown-but-bounded disturbances. Aiming to feedback the controller with a state that belongs to the estimated set, an optimal state choice was proposed based on a constrained minimum-variance criteria, which is the main contribution of this work. Path tracking control was solved by discrete-time mixed $\mathcal{H}_2/\mathcal{H}_\infty$ control with pole-placement constraints. The proposed method was validated through numerical experiments, demonstrating the reduced conservativeness of the set-valued state estimator based on constrained zonotopes, the performance of the optimal selection of estimated states, and robustness of the designed controller. 



\section{Nonlinear state estimation} \label{sec:nonlinearestimation}

%This section presents three new methods for set-valued state estimation of a class of nonlinear discrete-time systems. The first method (Section \ref{sec:czib}) combines properties of interval arithmetic and constrained zonotopes, and yields a highly tunable and accurate state estimation algorithm. The other methods (Sections \ref{sec:meanvalue} and \ref{sec:firstorder}) are developed by extending, in a consistent way, two existing approaches for propagating zonotopes through nonlinear mappings. The key advantage of these new extensions is that they allow the entire state estimation procedure to be done using constrained zonotopes in CG-rep. Therefore, the update step can be done by exact intersection (with linear measurements), which is known to generate highly asymmetrical sets that cannot be accurately enclosed by ellipsoids, intervals, parallelotopes, and zonotopes. Using the methods developed in this section, such sets can be directly propagated to the next time step without prior simplification to a symmetric set. This overcomes a major source of conservatism in existing methods based on the aforementioned enclosures, while largely retaining the efficiency of computations with zonotopes. The content regarding the first method (Section \ref{sec:czib}) was published in \cite{Rego2018}. The content concerning the two new extensions (Sections \ref{sec:meanvalue} and \ref{sec:firstorder}) was submitted in \cite{Rego2018d}.

This section presents three new methods for set-valued state estimation of a class of nonlinear discrete-time systems. The first method (Section \ref{sec:czib}) combines properties of interval arithmetic and constrained zonotopes, and yields a highly tunable and accurate state estimation algorithm. The other methods (Sections \ref{sec:meanvalue} and \ref{sec:firstorder}) expand the linear state estimation algorithm in \cite{Scott2016} for a class of nonlinear discrete-time systems. These methods extend, in a consistent way, two existing approaches for propagating zonotopes through nonlinear mappings. The key advantage of these new extensions is that they allow the entire state estimation procedure to be done using constrained zonotopes in CG-rep. Therefore, the update step can be done by exact intersection (with linear measurements), which is known to generate highly asymmetrical sets that cannot be accurately enclosed by ellipsoids, intervals, parallelotopes, and zonotopes. Using the methods developed in this section, such sets can be directly propagated to the next time step without prior simplification to a symmetric set. This overcomes a major source of conservatism in existing methods based on the aforementioned enclosures, while largely retaining the efficiency of computations with zonotopes. The content regarding the first method (Section \ref{sec:czib}) was published in \cite{Rego2018}. The content concerning the two new extensions (Sections \ref{sec:meanvalue} and \ref{sec:firstorder}) was submitted in \cite{Rego2018d}.


\subsection{Problem formulation} \label{sec:nonlinearformulation}


Consider a class of discrete-time systems with nonlinear dynamics and linear measurements, described by
\begin{equation}
\begin{aligned} \label{eq:system}
\mbf{x}_k & = \mbf{f}(\mbf{x}_{k-1}, \mbf{u}_{k-1}, \mbf{w}_{k-1}), \\
\mbf{y}_k & = \mbf{C} \mbf{x}_k + \mbf{D}_u \mbf{u}_k +\mbf{D}_v \mbf{v}_k,	
\end{aligned}
\end{equation}
for $k \geq 1$, with $\mbf{y}_0 = \mbf{C} \mbf{x}_0 + \mbf{D}_u \mbf{u}_0 +\mbf{D}_v \mbf{v}_0$, where $\mbf{x}_k \in \realset^{n_x}$ denotes the system state, $\mbf{u}_{k} \in \realset^{n_u}$ is a known input, $\mbf{w}_k \in \realset^{n_w}$ is the process disturbance, $\mbf{y}_k \in \realset^{n_y}$ is the measured output, and $\mbf{v}_k \in \realset^{n_v}$ is the measurement uncertainty. The nonlinear mapping $\mbf{f}$ is assumed to be of class $\mathcal{C}^2$, and the uncertainties are assumed to be bounded, i.e., $\mbf{w}_{k} \in W_k$ and $\mbf{v}_k \in V_k$, where $W_k$ and $V_k$ are known compact sets.

This section proposes new methods to perform set-valued state estimation for nonlinear systems as in \eqref{eq:system}. The exact characterization of sets $X_k$ containing the evolution of the system states is very difficult in the nonlinear case, if not intractable \citep{Alamo2005a,Kieffer1998,Kuhn1998}. Therefore, in the set-membership framework the objective is to over-approximate such sets by guaranteed outer bounds $\hat{X}_k$ on the possible trajectories of the system states $\mbf{x}_k$. Such outer bounds must be consistent with the previous estimate $\hat{X}_{k-1}$ and known inputs $\mbf{u}_{k-1}$, and also with the current measurement $\mbf{y}_k$, and the bounds on the disturbances and uncertainties $W_{k-1}$, $V_k$. Given an initial set $\mbf{x}_0 \in \hat{X}_0$, a common approach is to proceed through the well-known prediction-update algorithm, which consists in computing real compact sets $\bar{X}_k$ and $\hat{X}_k$ such that
\begin{align}
\bar{X}_k & \supseteq \{ \mbf{f}(\mbf{x}, \mbf{u}_{k-1}, \mbf{w}) : \mbf{x} \in \hat{X}_{k-1}, \, \mbf{w} \in W_{k-1} \}, \label{eq:prediction0}\\
\hat{X}_k & \supseteq \{ \mbf{x} \in \bar{X}_k : \mbf{C} \mbf{x} + \mbf{D}_u \mbf{u}_k + \mbf{D}_v \mbf{v} = \mbf{y}_k, \, \mbf{v} \in V_k \}, \label{eq:update0}
\end{align}
in which \eqref{eq:prediction0} is referred to as the \emph{prediction step}, and \eqref{eq:update0} as the \emph{update step}. 

Our goal is to obtain accurate outer bounds $\bar{X}_k$ and $\hat{X}_k$ according to \eqref{eq:prediction0} and \eqref{eq:update0}, respectively. Following these definitions, and considering the initial condition $\mbf{x}_0 \in \hat{X}_0$, the property $\mbf{x}_k \in \hat{X}_k$ is guaranteed by construction for all $k \geq 0$ \citep{Chisci1996,Le2013,Alamo2008}.


%\subsection{Constrained zonotope and interval bundle algorithm}
\subsection{CZIB algorithm} \label{sec:czib}

This section presents the first proposed approach for set-valued state estimation of the class of nonlinear systems described in Section \ref{sec:nonlinearformulation}. The method is referred to as the constrained zonotope and interval bundle (CZIB) algorithm, and combines important properties from interval arithmetic and constrained zonotopes. A highly tunable and accurate nonlinear state estimation algorithm is developed, capable of providing tight enclosures for the set-valued state estimation problem described by \eqref{eq:prediction0}--\eqref{eq:update0}.


\subsubsection{Main ideas and assumptions} \label{sec:czibideas}

We first present the underlying ideas of the proposed algorithm. Some assumptions are made with respect to the set-valued state estimation problem described in Section \ref{sec:nonlinearformulation}:
\begin{itemize}
	\item[\textit{\textbf{A1)}}] \emph{The bounds on the process and measurement uncertainties can be described by constrained zonotopes (Definition \ref{def:czonotopes});}
	\item[\textit{\textbf{A2)}}] \emph{An initial guess $\bar{X}_0$ satisfying $\mbf{x}_0 \in \bar{X}_0$ is available, in which $\bar{X}_0$ is described by a constrained zonotope;}
	\item[\textit{\textbf{A3)}}] \emph{The nonlinear mapping $\mbf{f}$ is affine in $\mbf{w}$, namely $\mbf{f}(\mbf{x},\mbf{u},\mbf{w}) = \bar{\mbf{f}}(\mbf{x},\mbf{u}) + \mbf{D}_w \mbf{w}$.}
\end{itemize}

%Since constrained zonotopes can represent arbitrary convex polytopes, assumptions \emph{A1} and \emph{A2} impose very little restrictions to the problem. Moreover, interval vectors, parallelotopes, and zonotopes are particular constrained zonotopes \cite{Scott2016}, thus these classes of sets are covered by such assumptions.% by \emph{A1} and \emph{A2}.%  On the other hand, we will require that the process disturbances must be bounded by an interval vector (assumption A1), which may seem to be restrictive at a first glance. However, in practical situations, known bounds for disturbances can be often described component-wise.
Since constrained zonotopes can represent arbitrary convex polytopes, assumptions \emph{A1} and \emph{A2} impose very little restrictions to the problem. Besides, intervals, parallelotopes, and zonotopes are special cases of constrained zonotopes \citep{Scott2016}. Thus, these classes of sets are covered by these assumptions. On the other hand, \emph{A3} is restrictive and leads a particular reformulation of the prediction step \eqref{eq:prediction0}, given by
\begin{equation} \label{eq:predictionczib}
	\bar{X}_k \supseteq \{ \bar{\mbf{f}}(\mbf{x}, \mbf{u}_{k-1}) + \mbf{D}_w \mbf{w} : \mbf{x} \in \hat{X}_{k-1}, \, \mbf{w} \in W_{k-1} \}.
\end{equation}


For simplicity, we first present a straightforward solution to the update step. The problem of computing an enclosure $\hat{X}_k$ satisfying \eqref{eq:update0} is similar to the linear case \eqref{eq:updatelinear0}, and can be restated in terms of the generalized intersection \eqref{eq:intersection}. Let $Y_k \subset \realset^{n_y}$ be a constrained zonotope such that $Y_k = (\mbf{y}_k - \mbf{D}_u \mbf{u}_k) \oplus (-\mbf{D}_v V_k)$. Then, \eqref{eq:update0} is restated as  
\begin{equation} \label{eq:updateczib}
\hat{X}_k \supseteq \{ \mbf{x} \in \bar{X}_k : \mbf{C} \mbf{x} \in Y_k \} = \bar{X}_k \ginter{C} Y_k.	
\end{equation}

Since $Y_k$ is a constrained zonotope, if $\bar{X}_k$ is also a constrained zonotope then an exact bound for \eqref{eq:updateczib} can be obtained through \eqref{eq:czintersection}. However, even if $\bar{X}_0$ and $W_k$ are constrained zonotopes, the reachable sets of the nonlinear system \eqref{eq:system} computed over the domains $\hat{X}_{k-1}$ and $W_{k-1}$ are not even convex in general \citep{Althoff2013}. Thus, the main challenge is to solve the prediction step \eqref{eq:predictionczib} such that the obtained bound $\bar{X}_k$ is a constrained zonotope, which is the main contribution of the CZIB algorithm as the first proposed solution to this problem.

%An early attempt to obtain bounds $\bar{X}_k$ as zonotopes can be found in \cite{Alamo2005a}. However, since zonotopes are centrally symmetric, severe conservativeness can occur in over-approximating a non-convex set by a zonotope. Since constrained zonotopes can describe at least any convex polytope, the associated conservativeness is substantially reduced. However, for the knowledge of the authors, no methods for approximating the reachable sets of nonlinear systems using interval bundles and exploiting constrained zonotopes have been proposed so far.%However, for the knowledge of the authors, no methods for approximating the reachable sets of nonlinear systems by constrained zonotopes have been proposed so far.

In order to bound the possible trajectories of the nonlinear system \eqref{eq:system} using constrained zonotopes, we subdivide the prediction step into three main problems:%sub-steps:% problems:


%\smallskip
\begin{enumerate}%{enumerate}
	\item[\textit{\textbf{P1)}}]\emph{Compute an interval bundle $\standardib$ satisfying $\hat{X}_{k-1} \subseteq \mathcal{B}$;}
	\item[\textit{\textbf{P2)}}]\emph{Compute a refinement $\particularref$, where $\square(\bar{\mbf{f}}(\cdot))$ is an inclusion function of $\bar{\mbf{f}}(\cdot)$;}
	\item[\textit{\textbf{P3)}}]\emph{Compute a constrained zonotope $\bar{X}_{k}$ satisfying $\standardref \oplus \mbf{D}_w W_{k-1} \subseteq \bar{X}_k$}.
\end{enumerate}
%\smallskip


Problem \emph{P2} can be solved straightforwardly through interval arithmetic. Therefore, we focus on obtaining solutions to problems \emph{P1} and \emph{P3}, which are the presented in the next subsection along with the complete CZIB state estimation algorithm.



%\subsubsection{The algorithm} \label{sec:thealgorithm}
\subsubsection{Proposed solutions} \label{sec:thealgorithm}


In order to obtain tight enclosures on \emph{P1}, we require the ability to compute the interval hull of a constrained zonotope (Proposition \ref{prope:ihull}). Our goal is to obtain the \emph{least interval bundle} containing $\hat{X}_{k-1}$. The following proposition shows how to generate the least interval bundle containing $\hat{X}_{k-1}$ from a given $n_d$-partition of the interval hull of $\hat{X}_{k-1}$ (recall Definition \ref{def:partitions}).


\begin{proposition} \rm \label{prop:leastibundle}
	Let $Z = \{\mbf{G}, \mbf{c}, \mbf{A}, \mbf{b} \} \subset \realset^{n}$. For a given $n_d \in \naturalset\backslash 0$, the \emph{least interval bundle} $\mathcal{B} = \cup_{j=1}^{n_b} B_j$ containing $Z$ is obtained by the union of all intervals $B_j$ composing the $n_d$-partition of the interval hull of $Z$, such that
	\small
	\begin{equation} \label{eq:leastibundle}
	Z \cap_{\eyenoarg} B_j \neq \emptyset,
	\end{equation}
	\normalsize
	where $\eyenoarg$ denotes the identity matrix. 
\end{proposition}
\proof Let $H(Z)$ denote the interval hull of $Z$. Clearly, for a given $n_d$ the $n_d$-partition $\bar{\mathcal{B}} = \cup_{j=1}^{\bar{n}_b} B_j$ of $H(Z)$ is the least interval bundle containing $H(Z)$. By definition, for every $B_j$ in $\bar{\mathcal{B}}$ satisfying $Z \cap_{\eyenoarg} B_j = \emptyset$, $\nexists \mbf{z} \in Z : \mbf{z} \in B_j$. Therefore, by removing all such $B_j$ from $\bar{\mathcal{B}}$, yields $\mathcal{B} = \cup_{j=1}^{n_b} B_j \supseteq Z$, with $n_b \leq \bar{n}_b$. Then, by definition for every $B_j$ in $\mathcal{B}$, $\exists \mbf{z} \in Z : \mbf{z} \in B_j$. By removing any such $B_j$ from $\mathcal{B}$ yields $\tilde{\mathcal{B}} \nsupseteq Z$. \qed 

\begin{remark} \rm
	Since every interval vector is a constrained zonotope, the condition \eqref{eq:leastibundle} can be easily verified through \eqref{eq:czintersection} and Property \ref{prop:isemptybelongsto} for each $B_j$, from which the least interval bundle containing $\hat{X}_{k-1}$ can be effectively obtained. Further reductions in overestimation can be achieved by increasing the number of divisions when computing the least interval bundle.
\end{remark}


\begin{figure}[!tb]
	%\vspace{1.5mm}
	\begin{scriptsize}
		\centering{
			\def\svgwidth{0.7\columnwidth}
			\import{Figures_ECC/}{fig_intervalhull_leastintervalbundle_v2.pdf_tex}
			\caption{Solid lines (blue) depicts a constrained zonotope $Z = \{\mbf{G},\mbf{c},\mbf{A},\mbf{b}\}$ defined by $\mbf{G} = \protect\begin{bmatrix} 1 & 0 & 1 \protect\\ 1 & 2 & -1 \protect\end{bmatrix}$, $\mbf{c} = \protect\begin{bmatrix} 0 \protect\\ 0 \protect\end{bmatrix}$, $\mbf{A} = \protect\begin{bmatrix} -2 & 1 & -1 \protect\end{bmatrix}$, and $\mbf{b} = 2$. Dashed lines denote the interval hull of $Z$ (left), and the least interval bundle containing $Z$ for a 10-partition (right).}\label{fig:ihull_libundle}}
		%\caption{Solid lines depicts the constrained zonotope $Z = \left\{ \right\}$ }\label{fig:ihull_libundle}}
		%\vspace{-5mm}
	\end{scriptsize}
\end{figure}

Fig. \ref{fig:ihull_libundle} illustrates the underlying ideas regarding Proposition \ref{prop:leastibundle}. We are then able to state Algorithm \ref{alg:o1}, which solves problem \emph{P1}.

\begin{algorithm}[!htb]
	%\renewcommand{\addcontentsline}[3]{}
	\caption{Solver for \emph{P1}}
	\label{alg:o1}
	\small
	\begin{algorithmic}[1]
		\State Compute the interval hull of $\hat{X}_{k-1}$ by means of Property \ref{prope:ihull}
		\State Compute the $n_d$-partition of the interval hull according to Definition \ref{def:partitions}
		\State Compute the least interval bundle $\standardib$ containing $\hat{X}_{k-1}$ through Proposition \ref{prop:leastibundle}
	\end{algorithmic}
	\normalsize
\end{algorithm}


Problem \emph{P2} can be solved straightforwardly using interval arithmetic. The associated algorithm is presented in Algorithm \ref{alg:o2}, which essentially generates a refinement of $\bar{\mbf{f}}(\mbf{x}, \mbf{u}_{k-1})$ over $\standardib$. This algorithm allows different inclusion functions to be used\footnote{E.g., natural interval extension, mean value extension, and others \citep{Moore2009}.}, which may be tested offline for choosing which one leads to less conservatism, according to the nonlinear mapping $\bar{\mbf{f}}(\mbf{x}, \mbf{u}_{k-1})$. Furthermore, as in the case of algorithms involving zonotope bundles \citep{Althoff2011}, Algorithm \ref{alg:o2} can be parallelized in order to improve computational performance.

\begin{algorithm}[!htb]
	%\renewcommand{\addcontentsline}[3]{}
	\caption{Solver for \emph{P2}}
	\label{alg:o2}
	\small
	\begin{algorithmic}[1]
		\For {$j = 1,...,n_b$}
		\State Compute an inclusion function of $\bar{\mbf{f}}(\mbf{x}, \mbf{u}_{k-1})$ for $B_j$, from $\standardib$ obtained through Algorithm \ref{alg:o1}
		\EndFor
	\end{algorithmic}
	\normalsize
\end{algorithm}



In order to develop a solution to problem \emph{P3}, we first propose a method to compute the interval hull of an interval bundle, and then we define the concept of \emph{interval vertices}.

\begin{proposition} \rm \label{prop:ihullibundle}
	Let $\mathcal{B} = \cup_{j=1}^{n_b} B_j$ be an interval bundle in $\realset^{n}$. The \emph{interval hull} of $\mathcal{B}$ is obtained component-wise by searching for $\zeta_i^\text{L} = {\min}\{ \beta_{j,i}^\text{L} \}$, $\zeta_i^\text{U} = {\max}\{ \beta_{j,i}^\text{U} \}$
	for each $i = 1,2,\dots,n$, and $\mathcal{B} \subseteq [\bm{\zeta}^\text{L},\,\bm{\zeta}^\text{U}]$.
\end{proposition}
\proof The proof follows from Definition \ref{def:intvalvector}. \qed 

\begin{definition} \rm \label{def:ivertex}
	Let $\mathcal{B} = \cup_{j=1}^{n_b} B_j$ be an interval bundle in $\realset^{n}$. The $j$-th interval vector $B_j$ is an \emph{interval vertex} of $\mathcal{B}$ iff at least one component of any of its endpoints coincide with one component of any endpoint of the interval hull of $\mathcal{B}$.
\end{definition}



Ideally, the convex hull of $\particularref$ must be obtained to solve problem \emph{P3} with reduced conservatism. However, due to the complexity of this operation, our solution consists in the following:
\begin{itemize}
	\item[\emph{P3.1})] \emph{Build an auxiliary convex polytope using the midpoints of the interval vertices of $\particularref$ as its vertices, and denote it as $\tilde{X}_k$;}
	\item[\emph{P3.2})] \emph{Move the hyperplanes of $\tilde{X}_k$ to obtain a constrained zonotope bounding $\particularref$.}	
\end{itemize}

 
Algorithm \ref{alg:firstconvexpoly} clarifies how to perform \emph{P3.1}.


\begin{algorithm}[!htb]
	%\renewcommand{\addcontentsline}[3]{}
	\caption{Auxiliary convex polytope}
	\label{alg:firstconvexpoly}
	\small
	\begin{algorithmic}[1]
		\State Compute the interval vertices of $\particularref$ according to Definition \ref{def:ivertex}
		\State Build a convex polytope in V-rep using the midpoints of the interval vertices
		\State Convert the result from V-rep to H-rep
	\end{algorithmic}
	\normalsize
\end{algorithm}

Fig. \ref{fig:ivertices_auxcz} demonstrates the essential stages to obtain the auxiliary convex polytope. Algorithm \ref{alg:firstconvexpoly} requires the conversion from V-rep to H-rep, which can be expensive. However, in the proposed state estimation algorithm such conversion is performed only once per iteration. In addition, \emph{P3.2} is solved by means of Algorithm \ref{alg:minksum}, which requires the computation of $n_h$ LPs.%, in

\begin{figure}[!htb]
	%\vspace{1.5mm}
	\begin{scriptsize}
		\centering{
			\def\svgwidth{0.7\columnwidth}
			%\import{images/}{fig_intervalhull_leastintervalbundle.pdf_tex}
			\import{Figures_ECC/}{fig_intervalvertices_auxcz.pdf_tex}
			\caption{Solid lines depicts an interval bundle $\mathcal{B}$. Left: the interval hull (dashed) and the interval vertices (red) of $\mathcal{B}$. Right: the auxiliary convex polytope, formed by the midpoints of the interval vertices (red, dashed).}\label{fig:ivertices_auxcz}}
		%\vspace{-5mm}
	\end{scriptsize}
\end{figure}


In some cases, the refinement $\particularref$ may not yield enough interval vertices to form a simplex in $\realset^{n_x}$. In this situation, a Minkowski sum can be performed over the associated vertices (midpoints) in V-rep using a ``very small'' zero-centered interval vector, to generate additional vertices before performing the conversion to H-rep.


\begin{algorithm}[!htb]
	%\renewcommand{\addcontentsline}[3]{}
	\caption{Moving hyperplanes}
	\label{alg:minksum}
	\small
	\begin{algorithmic}[1]
		\Statex Given $\tilde{X}_k$ in the H-rep $\{\mbf{x} \in \realset^n : \mbf{H}\mbf{x} \leq\mbf{k}\}, \mbf{k} \in \realset^{n_h}$
		\For{$i = 1,2,\dots n_h$}
		\State ${k}'_i = \underset{k_i}{\min} \{k_i : \mbf{H}_i \mbf{x}^{\{j,l\}} \leq k_i ,\, \forall j,l \}$,
		\Statex $\quad \,\,\,$where $\mbf{x}^{\{j,l\}}$ denotes the $l$-th vertex of the $j$-th interval vector in $\particularref$
		\EndFor
		\State Convert the resulting $\{\mbf{H},\mbf{k}'\}$ to CG-rep using \eqref{eq:hreptocg}% to obtain $\tilde{X}_k$ 
	\end{algorithmic}
	\normalsize
\end{algorithm}


We now conclude our solution to \emph{P3}. Given the constrained zonotope $\tilde{X}_k \supset \particularref$ obtained using Algorithms \ref{alg:firstconvexpoly} and \ref{alg:minksum}, a constrained zonotope $\bar{X}_k$ bounding the trajectories of the system can be obtained through
\begin{equation} \label{eq:problem3}
\bar{X}_k = (\tilde{X}_k \ginter{\eyenoarg} H) \oplus \mbf{D}_w W_{k-1},
\end{equation}
where $H$ denotes the interval hull of $\particularref$. The intersection with the interval hull $H$ is introduced to obtain tighter bounds, since the vertices of the constrained zonotope $\tilde{X}_k$ may extrapolate $H$. This intersection is computed using \eqref{eq:intersection}. The linear image and the Minkowski sum in \eqref{eq:problem3} are computed exactly using \eqref{eq:czlimage} and \eqref{eq:czmsum}, respectively.

By solving problems \emph{P1}, \emph{P2} and \emph{P3}, a constrained zonotope enclosing \eqref{eq:predictionczib} is obtained. Therefore, the correction step \eqref{eq:updateczib} can be performed exactly using \eqref{eq:czintersection}. The CZIB state estimation algorithm can be finally stated.%, which we call as \emph{constrained zonotope and interval bundle} (CZIB) algorithm.


\begin{algorithm}
	%\renewcommand{\addcontentsline}[3]{}
	\caption{CZIB algorithm}
	\label{alg:czib}
	\small
	\begin{algorithmic}[1]
		%\Procedure{order\_reduction}{$\hat{\mathbb{X}}_{k}, r_\text{max}$}
		%\Statex \emph{Parameters:} $\bar{X}_0$, $W_k$, $V_k$, $n_d$, $\varepsilon$
		\Statex \emph{Prediction step}% \nonumber
		\State $\quad$ Compute $\standardib \supset \hat{X}_{k-1}$ using Algorithm \ref{alg:o1}%, for a given $n_d$
		\State $\quad$ Compute $\particularref$ using Algorithm \ref{alg:o2}%, for a given $n_d$
		\State $\quad$ Compute $\bar{X}_k$ through Algorithms \ref{alg:firstconvexpoly}, \ref{alg:minksum} and \eqref{eq:problem3}
		\Statex \emph{Update step}
		\State $\quad$ Compute $\hat{X}_{k}$ using \eqref{eq:updateczib}
	\end{algorithmic}
	\normalsize
\end{algorithm}

Algorithm \ref{alg:czib} is highly tunable. The compromise between conservatism and complexity is given by the number of divisions in Algorithm \ref{alg:o1} and the inclusion function chosen to be used in Algorithm \ref{alg:o2}. Moreover, due to the proposed transformations performed in the prediction step (from CG-rep to interval bundle and vice-versa), the complexity of the constrained zonotope $\hat{X}_{k}$ \emph{is not associated with time}, but with the number of interval vertices instead (see Figure \ref{fig:ivertices_auxcz}). The set complexity can be limited by choosing a given collection of interval vertices taken from the existing ones according to any desired criteria. 

\subsubsection{State estimation using interval bundles}

It is possible to perform the prediction step \eqref{eq:predictionczib} and the correction step \eqref{eq:updateczib}, using only interval bundles, i.e., without performing transformations involving constrained zonotopes. However, assumptions \emph{A1} and \emph{A2} (see Section \ref{sec:czibideas}) should be restricted to interval variables, or interval bundles containing the associated constrained zonotopes must be available. If intervals are used as bounds for disturbances instead, the wrapping effect arises in the linear mappings in \eqref{eq:predictionczib} and \eqref{eq:updateczib}.%, which is avoided by the use of constrained zonotopes. 

Moreover, in order to perform \eqref{eq:updateczib} using interval bundles, a set of consistent states must be obtained beforehand \citep{Alamo2005a}. If the latter is also an interval bundle, the intersection must be computed \emph{interval by interval}, yielding a worst-case factorial increase in the number of intervals composing the bundle.% On the other hand, the intersection \eqref{eq:czcorrection} is performed directly and exactly using constrained zonotopes.% through \eqref{eq:czintersection}.




\subsection{Mean value extension} \label{sec:meanvalue}



This section presents the first of the two new extensions for enclosing the range of a nonlinear function over a set of inputs described by constrained zonotopes. This method is referred to as the \emph{mean value extension} (because it relies on the Mean Value Theorem), and is a direct generalization of the method for zonotopes in \cite{Alamo2005a}. The method in \cite{Alamo2005a} relies on a \emph{zonotope inclusion} operator that computes a zonotopic enclosure of the product of an interval matrix with a unitary box. We first generalize this operator to constrained zonotopes.

\begin{theorem} \rm \label{the:gzielim}   
	Let $X = \mbf{p} \oplus \mbf{M} B_\infty (\mbf{A},\mbf{b}) \subset \realset^n$ be a constrained zonotope, let $\mbf{J} \in \intvalsetmat{n}{n}$ be an interval matrix, and consider the set 
	\begin{equation*}
	Z = \mbf{J} X \triangleq \{\hat{\mbf{J}} \mbf{x} : \hat{\mbf{J}} \in \mbf{J}, \mbf{x} \in X\}.
	\end{equation*}	
	Let $\bar{X} = \bar{\mbf{p}} \oplus \bar{\mbf{M}} B_\infty^{\bar{n}_g}$ be a zonotope satisfying $X \subseteq \bar{X}$, let $\mbf{m}$ be an interval vector such that $\mbf{m} \supseteq (\mbf{J} - \midpoint{\mbf{J}}) \bar{\mbf{p}}$ and $\midpoint{\mbf{m}} = \bm{0}$, and let $\mbf{G} \in \realsetmat{n}{n}$ be a diagonal matrix defined by
	\begin{equation*}
	G_{ii} = \half \diam{m_i} +  \half \sum_{j=1}^{\bar{n}_g} \sum_{k=1}^n \diam{J_{ik}} |\bar{M}_{kj}|,
	\end{equation*}
	for all $i=1,2,\dots,n$. Then $Z$ is contained in the \emph{CZ-inclusion}
	\begin{equation} \label{eq:czinclusion}
	Z \subseteq \gzinclusion(\mbf{J},X) \triangleq \midpoint{\mbf{J}}X \oplus \mbf{G}B_\infty^n,
	\end{equation}
	where $B_\infty^n$ denotes the $n$-dimensional unitary hypercube.
\end{theorem}

\proof 
Choose any $\mbf{z} \in Z$. It will be shown that $\mbf{z} \in \gzinclusion(\mbf{J},X)$. By the definition of $Z$, there must exist $\mbf{x} \in X$ and $\hat{\mbf{J}} \in \mbf{J}$ such that $\mbf{z} = \hat{\mbf{J}} \mbf{x}$. Adding and subtracting $\midpoint{\mbf{J}} \mbf{x}$,
\begin{equation*}
\mbf{z} = \midpoint{\mbf{J}} \mbf{x} + (\hat{\mbf{J}} - \midpoint{\mbf{J}}) \mbf{x}.	
\end{equation*}
Since $\mbf{x}\in X\subset \bar{X}$, there exists $\bm{\gamma} \in B_\infty^{\bar{n}_g}$ such that $\mbf{x} = \bar{\mbf{p}} + \bar{\mbf{M}} \bm{\gamma}$. Therefore,
\begin{align*}
\mbf{z} &= \midpoint{\mbf{J}}\mbf{x} + (\hat{\mbf{J}} - \midpoint{\mbf{J}}) (\bar{\mbf{p}} + \bar{\mbf{M}} \bm{\gamma}).
\end{align*}
By the choice of $\mbf{m}$, there must exist $\hat{\mbf{m}}\in\mbf{m}$ such that
\begin{align}
\label{Eq: CZ Inc Proof - z equality}
\mbf{z} &= \midpoint{\mbf{J}}\mbf{x} + \hat{\mbf{m}} + (\hat{\mbf{J}} - \midpoint{\mbf{J}}) \bar{\mbf{M}} \bm{\gamma}.
\end{align}
Let $\bm{\eta}= \hat{\mbf{m}}+(\hat{\mbf{J}} - \midpoint{\mbf{J}}) \bar{\mbf{M}} \bm{\gamma}$. Then 
\begin{align*}
\eta_{i} &= \hat{m}_i+\sum_{j=1}^{\bar{n}_g} ((\hat{\mbf{J}} - \midpoint{\mbf{J}}) \bar{\mbf{M}})_{ij} \gamma_j, \\
&= \hat{m}_i+\sum_{j=1}^{\bar{n}_g} (\sum_{k=1}^{n} (\hat{J}_{ik}-\midpoint{J_{ik}}) \bar{M}_{kj}) \gamma_j.
\end{align*}
By the triangle inequality and the fact that $|\gamma_j|\leq 1$,
\begin{align*}
|\eta_{i}| &\leq |\hat{m}_i|+\sum_{j=1}^{\bar{n}_g} (\sum_{k=1}^{n} |(\hat{J}_{ik}-\midpoint{J_{ik}})|| \bar{M}_{kj}|)|\gamma_j|, \\
&\leq \half \diam{m_i} +  \half \sum_{j=1}^{\bar{n}_g} \sum_{k=1}^n \diam{J_{ik}} |\bar{M}_{kj}|.
\end{align*}
Therefore, $\bm{\eta}\in \mbf{G}B_\infty^n$. From \eqref{Eq: CZ Inc Proof - z equality}, this implies that
\begin{align*}
\mbf{z} = \midpoint{\mbf{J}}\mbf{x} + \bm{\eta} \in \midpoint{\mbf{J}} X \oplus \mbf{G} B_\infty^n = \gzinclusion(\mbf{J},X).
\end{align*}
Thus $Z \subseteq \gzinclusion(\mbf{J},X)$.
\qed

\begin{remark} \rm  \label{rem:contrelim}
	In Theorem \ref{the:gzielim}, a zonotope satisfying $X \subseteq \bar{X}$ can be easily obtained by performing $n_c$ iterated constraint eliminations on $X$ using Method \ref{meth:czconelim} in the Appendix. Moreover, $\mbf{m}$ can be obtained by simply evaluating $(\mbf{J} - \midpoint{\mbf{J}}) \bar{\mbf{p}}$ with interval arithmetic. These methods are used in this doctoral thesis.
\end{remark}

The following theorem provides the mean value extension for constrained zonotopes. In the remainder of this section, functions with set-valued arguments are consistently used to denote exact image of the set under the function; e.g., $\bm{\mu}(X,W)\triangleq\{\bm{\mu}(\mbf{x},\mbf{w}): \mbf{x}\in X, \ \mbf{w}\in W\}$.


\begin{theorem} \rm \label{the:pred2}
	Let $\bm{\mu} : \realset^n \times \realset^{n_w} \to \realset^n$ be continuously differentiable and let $\nabla_x \bm{\mu}$ denote the gradient of $\bm{\mu}$ with respect to its first argument. Let $X\subset \realset^n$ and $W \subset \realset^{n_w}$ be constrained zonotopes and choose any $\mbf{h} \in X$. If $Z$ is a constrained zonotope such that $\bm{\mu}(\mbf{h},W) \subseteq Z$ and $\mbf{J} \in \intvalsetmat{n}{n}$ is an interval matrix satisfying $\nabla^T_x \bm{\mu}(X, W)\subseteq \mbf{J}$, then $\bm{\mu}(X,W) \subseteq Z \oplus \gzinclusion\left(\mbf{J},  X - \mbf{h} \right)$.
\end{theorem}

\proof Choose any $(\mbf{x},\mbf{w})\in X\times W$. It will be shown that $\bm{\mu}(\mbf{x},\mbf{w}) \in Z \oplus \gzinclusion\left(\mbf{J},  X - \mbf{h} \right)$. For any $i=1,2,\ldots,n$, the Mean Value Theorem ensures that $\exists \bm{\delta}^i\in X$ such that
\begin{align*}
\mu_i(\mbf{x},\mbf{w}) &= \mu_i(\mbf{h},\mbf{w}) + \nabla^T_x \mu_i(\bm{\delta}^i,\mbf{w}) (\mbf{x} - \mbf{h}).
\end{align*}
But the vector $\nabla^T_x \mu_i(\bm{\delta}^i,\mbf{w})$ is contained in the $i$-th row of $\mbf{J}$ by hypothesis, and since this is true for all $i=1,2,\ldots,n$, there exists a real matrix $\hat{\mbf{J}}\in \mbf{J}$ such that
\begin{align*}
\bm{\mu}(\mbf{x},\mbf{w}) &= \bm{\mu}(\mbf{h},\mbf{w}) + \hat{\mbf{J}} (\mbf{x} - \mbf{h}).
\end{align*}
By Theorem \ref{the:gzielim} and the choice of $Z$, it follows that $\bm{\mu}(\mbf{x},\mbf{w}) \in Z \oplus \gzinclusion\left(\mbf{J}, X - \mbf{h}\right)$, as desired. \qed

\begin{remark} \rm \label{rem:affine}
	The interval matrix $\mbf{J}$ required by Theorem \ref{the:pred2} can be obtained by computing the interval hulls of $X$ and $W$ as in Property \ref{prope:ihull} and then bounding $\nabla^T_x \bm{\mu}(X, W)$ using interval arithmetic. Similarly, the constrained zonotope $Z \supseteq \bm{\mu}(\mbf{h},W)$ can be obtained by bounding $\bm{\mu}(\mbf{h},W)$ with interval arithmetic. Alternatively, another mean value extension can be applied around some $\mbf{h}_w \in W$ to obtain $\bm{\mu}(\mbf{h},W) \subseteq Z\triangleq \bm{\mu}(\mbf{h},\mbf{h}_w) \oplus \gzinclusion\left(\mbf{J}_w,W - \mbf{h}_w\right)$, where $\mbf{J}_w$ is an interval enclosure of $\nabla^T_w\bm{\mu}(\mbf{h}, W)$. Finally, if $\bm{\mu}$ is affine in $\mbf{w}$, i.e, $\bm{\mu}(\mbf{x},\mbf{w}) \triangleq \mbf{g}_x(\mbf{x}) + \mbf{G}_w(\mbf{x}) \mbf{w}$, then an exact enclosure of $\bm{\mu}(\mbf{h},W)$ is $Z = \mbf{g}_x(\mbf{h}) \oplus \mbf{G}_w(\mbf{h}) W$.
\end{remark}


\subsubsection{Selection of h} \label{sec:choosehmeanvalue}


In the mean value extension for intervals and zonotopes, a usual choice of $\mbf{h} \in X$ is the center of $X$ \citep{Alamo2005a,Moore2009}. However, with constrained zonotopes, since the center of the CG-rep \eqref{eq:czdefinition} is not the geometric center of $X$ in the general case, and may not even belong to $X$ \citep{Scott2016}, a different point $\mbf{h} \in X$ must be chosen in Theorem \ref{the:pred2}.


A simple and inexpensive choice of $\mbf{h}$ is the center of the interval hull of $X$. This point lies in $X$ in all of our computational experiments, although a proof ensuring membership in $X$ is not yet known. Nevertheless, this choice can be applied rigorously in Theorem \ref{the:pred2} by simply checking $\mbf{h} \in X$ beforehand by solving an LP \citep{Scott2016}, and using another choice if this fails.

However, as shown by experiment at the end of this subsection, different choices of $\mbf{h}$ can lead to significantly different results from Theorem \ref{the:pred2}. By investigating the CZ-inclusion defined in Theorem \ref{the:gzielim}, an appropriate approach consists in choosing $\mbf{h}$ such that $\bar{\mbf{p}} = \bm{0}$, which results in  $\diam{\mbf{m}} = \bm{0}$, regardless of $\mbf{J}$. This corresponds to make the center of $\bar{X}$ equal to zero, where $\bar{X}$ denotes the zonotope obtained after all of the constraints in the CG-rep of $X - \mbf{h}$ have been eliminated (see Theorem \ref{the:gzielim} and Remark \ref{rem:contrelim}, where $X \triangleq X - \mbf{h}$).


Let $X - \mbf{h} = X^{(n_c)} = \{\mbf{G}^{(n_c)}, \mbf{c}^{(n_c)}, \mbf{A}^{(n_c)}, \mbf{b}^{(n_c)}\}$, where $(\cdot)^{(\ell)}$ denotes variables associated with the constrained zonotope with $\ell$ remaining constraints, and $X = \{\mbf{G}_x, \mbf{c}_x, \mbf{A}_x, \mbf{b}_x\}$. Following the constraint elimination algorithm in \cite{Scott2016}, for each $\ell=n_c,n_c-1,\dots,1$, the remaining constraints $\mbf{A}^{(\ell)} \bm{\xi} = \mbf{b}^{(\ell)}$ are first preconditioned through Gauss-Jordan elimination with full pivoting and then subject to a rescaling procedure before the next constraint is eliminated. The entire procedure can be represented by the following recursive equations (see Methods \ref{meth:rescaling} and \ref{meth:czconelim} in the Appendix for details), where $\bar{(\cdot)}$ denotes variables after preconditioning, $\tilde{(\cdot)}$ denotes variables after rescaling, and $\bm{\Lambda}_\text{G}$, $\bm{\Lambda}_\text{A}$, $\bm{\xi}_\text{m}$, and $\bm{\xi}_\text{r}$ are defined as in Method \ref{meth:czconelim} in the Appendix:
\begin{equation} \label{eq:rescaling}
\begin{aligned}
\tilde{\mbf{c}}^{(\ell)} & = \mbf{c}^{(\ell)} + \bar{\mbf{G}}^{(\ell)} \bm{\xi}_\text{m}^{(\ell)}, \\		
\tilde{\mbf{G}}^{(\ell)} & = \bar{\mbf{G}}^{(\ell)} \text{diag}(\bm{\xi}_\text{r}^{(\ell)}),\\
\tilde{\mbf{A}}^{(\ell)} & = \bar{\mbf{A}}^{(\ell)} \text{diag}(\bm{\xi}_\text{r}^{(\ell)}),\\
\tilde{\mbf{b}}^{(\ell)} & = \bar{\mbf{b}}^{(\ell)} - \bar{\mbf{A}}^{(\ell)} \bm{\xi}_\text{m}^{(\ell)},
\end{aligned}
\end{equation}
\begin{equation} \label{eq:constrelim}
\begin{aligned}
\mbf{c}^{(\ell-1)} & = \tilde{\mbf{c}}^{(\ell)} + \bm{\Lambda}_\text{G}^{(\ell)} \tilde{\mbf{b}}^{(\ell)}, \\
\mbf{G}^{(\ell-1)} & = \tilde{\mbf{G}}^{(\ell)} - \bm{\Lambda}_\text{G}^{(\ell)} \tilde{\mbf{A}}^{(\ell)}, \\
\mbf{A}^{(\ell-1)} & = \tilde{\mbf{A}}^{(\ell)} - \bm{\Lambda}_\text{A}^{(\ell)} \tilde{\mbf{A}}^{(\ell)}, \\
\mbf{b}^{(\ell-1)} & = \tilde{\mbf{b}}^{(\ell)} - \bm{\Lambda}_\text{A}^{(\ell)} \tilde{\mbf{b}}^{(\ell)}.
\end{aligned}
\end{equation}
Note that if rescaling is not performed, then $\bm{\xi}_\text{m}^{(\ell)} = \bm{0}$ and $\bm{\xi}_\text{r}^{(\ell)} = \bm{1}$. Recursive computation of \eqref{eq:rescaling} and \eqref{eq:constrelim} leads to
\begin{equation} \label{eq:pbar}
\mbf{c}^{(0)} = \mbf{c}^{(n_c)} + \sum_{\ell=1}^{n_c} \left( \bar{\mbf{G}}^{(\ell)} \bm{\xi}_\text{m}^{(\ell)} + \bm{\Lambda}_\text{G}^{(\ell)} \tilde{\mbf{b}}^{(\ell)} \right).
\end{equation}

Careful examination of this algorithm reveals that the actions taken during preconditioning, rescaling, and constraint elimination are all independent of the center of the original constrained zonotope, which in this case is $\mbf{c}^{(n_c)} = \mbf{c}_x - \mbf{h}$. Thus, \eqref{eq:pbar} implies that the center of the final zonotope, $\mbf{c}^{(0)}$, can be made zero as desired if $\mbf{h}$ is chosen as 
\begin{equation} \label{eq:choice3}
\mbf{h} = \mbf{c}_x + \sum_{\ell=1}^{n_c} \left(\bar{\mbf{G}}^{(\ell)} \bm{\xi}_\text{m}^{(\ell)} + \bm{\Lambda}_\text{G}^{(\ell)} \tilde{\mbf{b}}^{(\ell)}\right).
\end{equation}


Unfortunately, this $\mbf{h}$ may not belong to $X$, so it is not always possible to achieve $\diam{\mbf{m}}=\bm{0}$. Thus, an alternative is to minimize $\diam{\mbf{m}}$ by solving
\begin{equation} \label{eq:choice3optimal}
\underset{\mbf{h}}{\min}~\{\|\diam{\mbf{m}}\|_1 : \mbf{h} \in X\}.
\end{equation}
By minimizing $\|\diam{\mbf{m}}\|_1$, the size of the box $\mbf{G} B_\infty^n$ in \eqref{eq:czinclusion} is reduced, leading to less conservative bounds. Recall that $\mbf{m} \supseteq (\mbf{J} - \midpoint{\mbf{J}}) \bar{\mbf{p}}$, with $\bar{\mbf{p}} \triangleq \mbf{c}^{(0)}$. In this section, we assume that $\mbf{m}$ is obtained using interval arithmetic, as is done in all of our numerical experiments. Since each element of $(\mbf{J} - \midpoint{\mbf{J}})\in \intvalsetmat{n}{n}$ is a symmetric interval satisfying $(J_{ij} - \midpoint{J_{ij}}) = (1/2) \diam{J_{ij}}[-1,1]$, and for a given $a \in \realset$, $a [-1,1] = |a| [-1,1]$, we have that
\begin{equation*}
\mbf{m} = \begin{bmatrix} \sum_{j=1}^{n} (1/2) \diam{J_{1j}} |\bar{p}_j| [-1,1] \\ \sum_{j=1}^{n} (1/2) \diam{J_{2j}} |\bar{p}_j| [-1,1] \\ \vdots \\ \sum_{j=1}^{n} (1/2) \diam{J_{nj}} |\bar{p}_j| [-1,1] \end{bmatrix}.
\end{equation*}
Therefore, $\diam{m_i} = \sum_{j=1}^n \diam{J_{ij}} |\bar{p}_j|$, and
\begin{align*}
\|\diam{\mbf{m}}\|_1 & = \sum_{i=1}^n \sum_{j=1}^n \diam{J_{ij}} |\bar{p}_j|\\
& = \sum_{j=1}^n \left( \sum_{i=1}^n \diam{J_{ij}} \right) |\bar{p}_j| = \sum_{j=1}^n \Theta_{jj} |\bar{p}_j|,
\end{align*}
with $\Theta_{jj} = \sum_{i=1}^n \diam{J_{ij}}$, and $\Theta_{ij} = 0$ for $i\neq j$. Then, considering \eqref{eq:pbar}, the optimization problem \eqref{eq:choice3optimal} is equivalent to
\begin{align}
\underset{\bm{\xi}}{\min}~& \|\bm{\Theta} \bar{\mbf{p}}\|_1 \label{eq:choosehmindiam}\\
\text{s.t.} \quad & \bar{\mbf{p}} = \mbf{c}_x - \mbf{h} + \sum_{\ell=1}^{n_c} \left( \bar{\mbf{G}}^{(\ell)} \bm{\xi}_\text{m}^{(\ell)} + \bm{\Lambda}_\text{G}^{(\ell)} \tilde{\mbf{b}}^{(\ell)} \right),\nonumber\\
& \mbf{h} = \mbf{c}_x + \mbf{G}_x \bm{\xi}, \nonumber\\
& \mbf{A}_x \bm{\xi} = \mbf{b}_x, \nonumber\\
& \ninf{\bm{\xi}} \leq 1, \nonumber
\end{align}
where the last three equalities ensure that $\mbf{h} \in X$.

The solution of \eqref{eq:choosehmindiam} yields an optimal choice of $\mbf{h} \in X$ that can be used in Theorem \ref{the:pred2} to reduce conservatism in the CZ-inclusion, and requires only the solution of one LP. Note that formulating \eqref{eq:choosehmindiam} requires the knowledge of $\mbf{G}^{(\ell)}$, $\bm{\xi}_\text{m}^{(\ell)}$, $\bm{\Lambda}_\text{G}^{(\ell)}$, and $\tilde{\mbf{b}}^{(\ell)}$, which are obtained from the iterated constraint elimination process. In turn, the constraint elimination process requires a choice of $\mbf{h} \in \realset^n$ to be made \emph{a priori}. However, since $\mbf{G}^{(\ell)}$, $\bm{\xi}_\text{m}^{(\ell)}$, $\bm{\Lambda}_\text{G}^{(\ell)}$, and $\tilde{\mbf{b}}^{(\ell)}$ are not affected by the center of the original constrained zonotope, constraint elimination can be performed with $\mbf{h} = \bm{0}$ to obtain the required data prior to the solution of \eqref{eq:choosehmindiam}. Once the optimal $\mbf{h}$ is obtained, constraint elimination can be repeated, or equivalently, the zonotope obtained using $\mbf{h} = \bm{0}$ can simply be translated by $-\mbf{h}$.


We summarize the proposed choices of $\mbf{h} \in X$ for use in Theorem \ref{the:pred2} as follows:
\begin{itemize}
	\item[\textbf{\textit{C1)}}] $\mbf{h}$ is given by the center of the interval hull of $X$, if it satisfies $\mbf{h} \in X$;
	\item[\textbf{\textit{C2)}}] $\mbf{h}$ is given by the closest point in $X$ to the center of $X$, computed through Proposition \ref{propo:closest};
	\item[\textbf{\textit{C3)}}] $\mbf{h}$ is obtained by solving \eqref{eq:choosehmindiam}.
\end{itemize}


To demonstrate the effect of the different choices of $\mbf{h}$, we consider the problem of one-step reachability analysis for the nonlinear system \citep{Raimondo2012}
\begin{equation} \label{eq:model2}
\begin{aligned}
x_{1,k} & = x_{1,k-1} + 0.4 x_{2,k-1} \\
x_{2,k} & = -0.132 e^{-x_{1,k-1}}x_{1,k-1} - 0.213 x_{1,k-1} + 0.274 x_{2,k-1},
\end{aligned}
\end{equation}
with
\begin{equation} \label{eq:reachX0}
X_0 = \left\{ \begin{bmatrix} 1 & 0 & 1 \\ 1 & 3 & -1 \end{bmatrix}, \begin{bmatrix} 0 \\ 0 \end{bmatrix}, \begin{bmatrix} -2 & 1 & -1  \end{bmatrix}, 2 \right\}.
\end{equation}

Figure \ref{fig:reachable} shows the constrained zonotope $X_0$ and the enclosures of the one-step reachable set obtained by Theorem \ref{the:pred2} using \emph{C1}--\emph{C3}. Clearly, the choice of $\mbf{h}$ has a significant impact, with \emph{C3} providing the least conservative result, as expected. Therefore, \emph{C3} is employed in Theorem \ref{the:pred2} henceforth.

\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_reachable_model2.pdf_tex}}
		\caption{Left: The constrained zonotope $X_0$ with `$\times$' denoting its center. Right: Enclosures obtained by applying Theorem \ref{the:pred2} to \eqref{eq:model2} with $\mbf{h}$ determined by \emph{C1} (green), \emph{C2} (yellow), and \emph{C3} (red).}\label{fig:reachable}}
\end{figure}


Since the CG-rep \eqref{eq:czdefinition} is an alternative representation for convex polytopes \citep{Scott2016}, the mean value extension developed in Theorem \ref{the:pred2} provides a new method for propagating convex polytopes implicitly through nonlinear mappings. A related approach can be found in \cite{Wan2018}, where convex polytopes are represented by intersections of zonotopes (i.e., zonotope bundles \citep{Althoff2011}). However, while effective complexity reduction algorithms are available for constrained zonotopes \citep{Scott2016}, efficient methods for complexity control of zonotope bundles have not yet been proposed.

\subsubsection{Update step} \label{sec:meanvalueupdate}

Similarly to the CZIB algorithm (Section \ref{sec:czib}), an exact bound for the update step \eqref{eq:update0} can be easily obtained by computing the generalized intersection of two constrained zonotopes as follows. Given the prediction set $\bar{X}_k$ obtained using the mean value extension (Theorem \ref{the:pred2}) which is described by a constrained zonotope, the bounds on measurement disturbances $V_k$, the current input $\mbf{u}_k$ and measurement $\mbf{y}_k$, the update step \eqref{eq:update0} is computed by
\begin{equation} \label{eq:updatemeanvalue}
	\hat{X}_k = \bar{X}_k \ginter{\mbf{C}} ((\mbf{y}_k - \mbf{D}_u \mbf{u}_k) \oplus (-\mbf{D}_v V_k)).
\end{equation}

Lastly, despite the exactness of this operation, similarly to zonotope-based methods iterated computations of the mean value extension and \eqref{eq:updatemeanvalue} result in complexity increase of the CG-rep \eqref{eq:czdefinition}. As discussed in Section \ref{sec:linearformulation}, this can be effectively addressed using order reduction algorithms that over-approximate a constrained zonotope by another with lower complexity \citep{Kopetzki2017,Scott2018}. Efficient methods for reducing the number of generators and constraints of the CG-rep \eqref{eq:czdefinition} with inevitable but reasonable conservativeness were proposed in \cite{Scott2016}. These are used in the numerical experiments conducted in this doctoral thesis. 

\subsection{First-order Taylor extension} \label{sec:firstorder}

This section presents the second new extension for enclosing the range of a nonlinear function over a set of inputs described by constrained zonotopes. This method is referred to as the \emph{first-order Taylor extension} (because it relies on a first-order Taylor expansion with a rigorous remainder bound), and is a direct generalization of the method for zonotopes in \cite{Combastel2005}. In the main result below, $(\cdot)_{i,:}$ denotes the $i$-th row of a matrix, and $(\cdot)_{ij}$ denotes the element from its $i$-th row and $j$-th column.  


\begin{theorem} \label{thm:firstorder} \rm
	Let $\bm{\eta}: \realset^n \to \realset^m$ be of class $\mathcal{C}^2$ and let $\mbf{z} \in \realset^n$ denote its argument. Let $\eta_q$ denote the $q$-th component of $\bm{\eta}$ and let $\mbf{H} \eta_q$ denote an upper triangular matrix describing half of the Hessian of $\eta_q$. Specifically, let $H_{ii} \eta_q = (1/2) \partial^2 \eta_q/\partial z_i^2$, $H_{ij} \eta_q = \partial^2 \eta_q/\partial z_i \partial z_j$ for $i<j$, and $H_{ij} \eta_q = 0$ for $i>j$. Let $Z = \{\mbf{G}, \mbf{c}, \mbf{A}, \mbf{b}\} \subset \realset^n$ be a constrained zonotope with $n_g$ generators and $n_c$ constraints. For each $q = 1,2,\dots,m$, let $\mbf{Q}^{[q]}\in\mathbb{IR}^{n\times n}$ and $\tilde{\mbf{Q}}^{[q]}\in\mathbb{IR}^{n_g\times n_g}$ be interval matrices satisfying $\mbf{Q}^{[q]} \supseteq \mbf{H} \eta_q (Z)$ and $\tilde{\mbf{Q}}^{[q]} \supseteq \mbf{G}^T \mbf{Q}^{[q]} \mbf{G}$. Moreover, define    
	\begin{align*}
	& \tilde{c}_q = \trace{\midpoint{\tilde{\mbf{Q}}^{[q]}}}/2, \\
	& \tilde{\mbf{G}}_{q,:} = \big[ \cdots \,\; \underbrace{\midpoint{\tilde{Q}^{[q]}_{ii}}/2}_{\forall i} \,\; \cdots  \,\; \underbrace{\left(\midpoint{\tilde{Q}^{[q]}_{ij}} + \midpoint{\tilde{Q}^{[q]}_{ji}}\right)}_{\forall i<j} \,\; \cdots \big], \\
	& \tilde{\mbf{G}}_{\mbf{v}} = \text{diag}(\mbf{v}), \quad v_q = \sum_{i,j} \left| \rad{\tilde{Q}^{[q]}_{ij}} \right|, \\
	& \tilde{\mbf{A}} = \left[ \tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \bm{0} \right],\\
	& \tilde{\mbf{A}}_{\bm{\zeta}} = \arrowmatrix{\begin{matrix} & \vdots & \\ \cdots & \half A_{ri} A_{si} & \cdots \\ & \vdots & \end{matrix}}{\forall i}{\forall r \leq s}, \quad \tilde{\mbf{A}}_{\bm{\xi}} = 
	\arrowmatrix{\begin{matrix} & \vdots & \\ \cdots & A_{ri} A_{sj} + A_{rj} A_{si} & \cdots \\ & \vdots & \end{matrix}}{\forall i < j}{\forall r \leq s}, \\
	& \tilde{\mbf{b}} = \downarrowmatrix{\begin{matrix} \vdots \\ b_{r} b_{s} - \half \sum_i A_{ri} A_{si} \\ \vdots\end{matrix}}{\forall r \leq s},
	\end{align*}
	with indices $i,j = 1,2,\dots,n_g$ and $r,s = 1,2,\dots,n_c$. Finally, choose any $\mbf{h} \in Z$ and let $\mbf{L}\in\mathbb{IR}^{m\times n}$ be an interval matrix satisfying $\mbf{L}_{q,:} \supseteq (\mbf{c} - \mbf{h})^T \mbf{Q}^{[q]}$ for all $q = 1,\dots,m$. Then,
	\begin{equation} \label{eq:firstorderextension}
	\bm{\eta}(Z) \subseteq \bm{\eta}(\mbf{h}) \oplus \nabla^T \bm{\eta}(\mbf{h})(Z - \mbf{h}) \oplus R,
	\end{equation}
	where
	\begin{align}
	R = \tilde{\mbf{c}} &\oplus [ \tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}} ] B_\infty(\tilde{\mbf{A}}, \tilde{\mbf{b}}) \oplus \gzinclusion (\mbf{L}, (\mbf{c} - \mbf{h}) \oplus 2\mbf{G} B_\infty(\mbf{A},\mbf{b}) ). \nonumber
	\end{align}
\end{theorem}

\proof
Choose any $\mbf{z}\in Z$ and $q\in\{1,\ldots,m\}$. By Taylor's theorem applied to $\eta_q$ with reference point $\mbf{h}$, there must exist $\bm{\Gamma}^{[q]} \in \mbf{H} \eta_q (Z) \subseteq \mbf{Q}^{[q]}$ such that \citep{Combastel2005}
\begin{align*}
\eta_q(\mbf{z}) & = \eta_q (\mbf{h}) + \nabla^T \eta_q (\mbf{h})(\mbf{z} - \mbf{h}) + (\mbf{z} - \mbf{h})^T \bm{\Gamma}^{[q]} (\mbf{z} - \mbf{h}). \nonumber
\end{align*}
Since $\mbf{z}\in Z$, there must exist $\bm{\xi} \in B_\infty(\mbf{A},\mbf{b})$ such that $\mbf{z}=\mbf{c} + \mbf{G}\bm{\xi}$. Thus, defining $\mbf{p} = \mbf{c} - \mbf{h}$ for brevity,
\begin{align*}
\eta_q(\mbf{z}) & = \eta_q (\mbf{h}) + \nabla^T \eta_q (\mbf{h})(\mbf{p} + \mbf{G}\bm{\xi}) + (\mbf{p} + \mbf{G}\bm{\xi})^T \bm{\Gamma}^{[q]}  (\mbf{p} + \mbf{G}\bm{\xi}).
\end{align*}
Expanding the product $(\mbf{p} + \mbf{G}\bm{\xi})^T \bm{\Gamma}^{[q]}  (\mbf{p} + \mbf{G}\bm{\xi})$ yields $\mbf{p}^T \bm{\Gamma}^{[q]} (\mbf{p} + 2 \mbf{G} \bm{\xi}) + \bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi}$, 
with $\tilde{\bm{\Gamma}}^{[q]} = \mbf{G}^T \bm{\Gamma}^{[q]} \mbf{G} \in \tilde{\mbf{Q}}^{[q]}$.
Since $\tilde{\bm{\Gamma}}^{[q]} \in \tilde{\mbf{Q}}^{[q]}$, it follows that $\tilde{\Gamma}^{[q]}_{ij} = \midpoint{\tilde{Q}^{[q]}_{ij}} + \rad{\tilde{Q}^{[q]}_{ij}} \Lambda^{[q]}_{ij}$ for some $\Lambda^{[q]}_{ij} \in B_\infty^1$. Additionally, $\xi_i \in [-1,1]$ implies that $\xi_i^2 \in [0, 1]$, and hence $\xi_i^2 = \half + \half \zeta_i$ for some $\zeta_i \in [-1,1]$. Considering these two facts,
\begin{align*}
\bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi} & = \half \sum_i \midpoint{\tilde{Q}^{[q]}_{ii}} + \half \sum_i \midpoint{\tilde{Q}^{[q]}_{ii}} \zeta_i \\
& \quad + \sum_{i<j}(\midpoint{\tilde{Q}^{[q]}_{ij}} + \midpoint{\tilde{Q}^{[q]}_{ji}}) \xi_i \xi_j + \sum_{i,j} \rad{\tilde{Q}^{[q]}_{ij}} \xi_i \xi_j \Lambda^{[q]}_{ij},
\end{align*}
where the third summation results from the fact that $\xi_i \xi_j = \xi_j \xi_i$. Thus, by defining the new generator variables% vector
\begin{equation*} %\label{eq:firstordernewgen}
\bar{\bm{\xi}} = \big[ \,\; \cdots \,\; \underbrace{\zeta_i}_{\forall i} \,\; \cdots \,\; \underbrace{\xi_i \xi_j}_{\forall i<j} \,\; \cdots \,\; \underbrace{\xi_i \xi_j \Lambda^{[q]}_{ij}}_{\forall i,j,q} \,\; \cdots \,\; \big]^T,
\end{equation*}
we have that $\bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi} = \tilde{c}_q + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}]_{q,:} \bar{\bm{\xi}}$, where
$\bar{\mbf{G}}_{\mbf{v}} = \text{blkdiag}(\mbf{N}^{[1]}, \mbf{N}^{[2]}, \dots, \mbf{N}^{[m]})$\footnote{In this doctoral thesis, $\text{blkdiag}(\mbf{A},\mbf{B},\dots)$ denotes a block diagonal matrix with blocks $\mbf{A},\mbf{B},\dots$.}, 
\begin{equation*}
\mbf{N}^{[q]} = \big[ \,\; \cdots \,\; \underbrace{\rad{\tilde{Q}^{[q]}_{ij}}}_{\forall i,j} \,\; \cdots \,\; \big] \in \realsetmat{1}{n_g^2}.
\end{equation*} 

Therefore, we have established that
\begin{align*}
\eta_q(\mbf{z}) = \eta_q (\mbf{h}) &+ \nabla^T \eta_q (\mbf{h})(\mbf{z} - \mbf{h}) + \mbf{p}^T \bm{\Gamma}^{[q]} (\mbf{p} + 2 \mbf{G} \bm{\xi}) + \tilde{c}_q + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}]_{q,:} \bar{\bm{\xi}}.
\end{align*}
This holds for every $q = 1,2,\dots,m$. Moreover, since $\mbf{L}$ is an interval matrix satisfying $\mbf{L}_{q,:} \supseteq \mbf{p}^T \mbf{Q}^{[q]}$ for all $q = 1,2,\dots,m$, there must exist $\hat{\mbf{L}}\in\mbf{L}$ such that $\hat{\mbf{L}}_{q,:}=\mbf{p}^T \bm{\Gamma}^{[q]}$ for all $q = 1,2,\dots,m$. Therefore,
\begin{align}
\label{Eq: eta vector expansion}
\bm{\eta}(\mbf{z}) = \bm{\eta}(\mbf{h}) &+ \nabla^T \bm{\eta} (\mbf{h})(\mbf{z} - \mbf{h})+ \hat{\mbf{L}}(\mbf{p} + 2 \mbf{G} \bm{\xi}) + \tilde{\mbf{c}} + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] \bar{\bm{\xi}}.
\end{align}

Furthermore, the equality constraints $\mbf{A} \bm{\xi} = \mbf{b}$ imply that $\mbf{A} \bm{\xi} \bm{\xi}^T \mbf{A}^T = \mbf{b} \mbf{b}^T$. %Thus, for $r,s = 1,2,\dots,n_c$,
Thus, considering $\xi_i^2 = \half + \half \zeta_i$, the $r$-th row and $s$-th column of this matrix equality yields
\begin{align*}
\half \sum_i A_{ri} A_{si} \zeta_i & + \sum_{i<j} (A_{ri} A_{sj} + A_{rj} A_{si}) \xi_i \xi_j = b_r b_s - \half \sum_i A_{ri} A_{si},
\end{align*}
with $r,s = 1,2,\dots,n_c$.
Such constraints are linear in $\bar{\bm{\xi}}$, and non-repeating for $r \leq s$, therefore $\bar{\mbf{A}} \bar{\bm{\xi}} = \tilde{\mbf{b}}$ holds, where $\bar{\mbf{A}} = [\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \bm{0}_{\tilde{n}_c \times n n_g^2}]$, with $\tilde{n}_c = \frac{n_c}{2}(1+n_c)$. Hence $\bm{\xi} \in B_\infty(\mbf{A},\mbf{b}) \implies \bar{\bm{\xi}} \in B_\infty(\bar{\mbf{A}},\tilde{\mbf{b}})$.

Combining this with \eqref{Eq: eta vector expansion}, we have proven the enclosure
\begin{align*}
\bm{\eta}(Z) \subseteq \bm{\eta} (\mbf{h}) & \oplus \nabla^T \bm{\eta} (\mbf{h})(Z - \mbf{h}) \\ & \oplus \mbf{L} (\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b})) \oplus \tilde{\mbf{c}} \oplus [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}).
\end{align*} 
In fact, this enclosure can be greatly simplified by noting that the columns of $\bar{\mbf{A}}$ corresponding to the variables $[\,\; \cdots \,\; \xi_i \xi_j \Lambda^{[q]}_{ij}\,\; \cdots \,\;]$ are all zero, and hence
\begin{equation*}
[\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}) = \tilde{\mbf{G}} B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}}], \tilde{\mbf{b}}) \oplus \bar{\mbf{G}}_{\mbf{v}} B_\infty^{nn_g^2}.
\end{equation*}
Since $\bar{\mbf{G}}_{\mbf{v}}$ is block diagonal and each $\mbf{N}^{[q]}$ is a row vector, $\bar{\mbf{G}}_{\mbf{v}} B_\infty^{nn_g^2}$ is an interval, and is equivalent to $\tilde{\mbf{G}}_{\mbf{v}} B_\infty^{n}$, with $\tilde{\mbf{G}}_{\mbf{v}}$ defined as in the statement of the theorem. Thus,
\begin{align*}
[\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}) &= \tilde{\mbf{G}} B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}}], \tilde{\mbf{b}}) \oplus \tilde{\mbf{G}}_{\mbf{v}} B_\infty^{n}, \\
&= [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \mbf{0}_{\tilde{n}_c\times n}], \tilde{\mbf{b}}), \\
&= [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty (\tilde{\mbf{A}}, \tilde{\mbf{b}}).
\end{align*}
Therefore,
\begin{align*}
\bm{\eta}(Z) \subseteq \bm{\eta} (\mbf{h}) &\oplus \nabla^T \bm{\eta} (\mbf{h})(Z - \mbf{h}) \\
&\oplus \mbf{L} (\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b})) \oplus \tilde{\mbf{c}} \oplus [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty (\tilde{\mbf{A}}, \tilde{\mbf{b}}),
\end{align*}
and \eqref{eq:firstorderextension} follows immediately from the definition of $R$. \qed


\begin{remark} \rm
	Regarding the definitions of $\tilde{\mbf{G}}$, $\tilde{\mbf{A}}_{\bm{\zeta}}$, $\tilde{\mbf{A}}_{\bm{\xi}}$, and $\tilde{\mbf{b}}$ in Theorem \ref{thm:firstorder}, the ordering of the indices $i<j$ and $r\leq s$ is irrelevant, as long as it is the same for all variables.
\end{remark}

\begin{remark} \rm
	The interval matrices $\mbf{Q}^{[q]}$ required by Theorem \ref{thm:firstorder} can be obtained by computing the interval hull of $Z$ (Property \ref{prope:ihull}) and then bounding $\mbf{H} \eta_q (Z)$ using interval arithmetic. Moreover, $\tilde{\mbf{Q}}^{[q]}$ and $\mbf{L}$ can be obtained by evaluating $\mbf{G}^T \mbf{Q}^{[q]} \mbf{G}$ and $(\mbf{c} - \mbf{h})^T \mbf{Q}^{[q]}$ using interval arithmetic.
\end{remark}


As in \cite{Combastel2005}, process disturbances can be taken into account in \eqref{eq:firstorderextension} by considering the augmented vector $\mbf{z} = (\mbf{x},\mbf{w})$ with $Z = X \times W \subset \realset^{n+n_w}$ and $\mbf{h} = (\mbf{h}_x,\mbf{h}_w) \in Z$. With $X = \{\mbf{G}_x, \mbf{c}_x, \mbf{A}_x, \mbf{b}_x\}$ and $W = \{\mbf{G}_w, \mbf{c}_w, \mbf{A}_w, \mbf{b}_w\}$, the Cartesian product $Z$ is easily computed by
\begin{equation*}
X \times W = \left\{ \begin{bmatrix} \mbf{G}_x & \bm{0} \\ \bm{0} & \mbf{G}_w \end{bmatrix}, \begin{bmatrix} \mbf{c}_x \\ \mbf{c}_w \end{bmatrix}, \begin{bmatrix} \mbf{A}_x & \bm{0} \\ \bm{0} & \mbf{A}_w \end{bmatrix}, \begin{bmatrix} \mbf{b}_x \\ \mbf{b}_w \end{bmatrix} \right\}.
\end{equation*}

\subsubsection{Selection of h} \label{sec:choosehfirstorder}


As with the mean value extension, the usual choice of $\mbf{h} \in Z$ in first-order Taylor extensions for intervals and zonotopes is the center of $Z$ \citep{Moore2009,Combastel2005}. However, since the center of a constrained zonotope $Z$ may not belong to $Z$, different choices of $\mbf{h}$ must be proposed.

As discussed in Section \ref{sec:choosehmeanvalue}, a simple choice is the center of the interval hull of $Z$. However, other choices may provide reduced conservatism in Theorem \ref{thm:firstorder}. By inspecting \eqref{eq:firstorderextension}, it is clear that if $\mbf{h}$ can be chosen as the center of $Z$, then $\mbf{L} = \bm{0}$, and the CZ-inclusion in $R$ vanishes, yielding less conservative results. However, since this point may not belong to $Z$, a good alternative may be to consider the closest point in $Z$ to its center, obtained by means of Proposition \ref{propo:closest}. A third option is to apply Proposition \ref{propo:center} to obtain an alternative CG-rep of $Z$ with any desired center. In this case, the new center is chosen as some point in $Z$, $\bar{\mbf{h}} \in Z$, and then $\mbf{h}$ is chosen as $\mbf{h} = \bar{\mbf{h}}$. A simple choice of new center $\bar{\mbf{h}} \in Z$ for such a procedure is the center of the interval hull of $Z$. The proposed alternatives are summarized as follows:
\begin{itemize}
	\item[\textbf{\textit{C4)}}] $\mbf{h}$ is given by the center of the interval hull of $Z$, if it satisfies $\mbf{h} \in Z$;
	\item[\textbf{\textit{C5)}}] $\mbf{h}$ is given by the closest point in $Z$ to the center of $Z$, by means of Proposition \ref{propo:closest};
	\item[\textbf{\textit{C6)}}] $\bar{\mbf{h}} \in Z$ is chosen as the center of the interval hull of $Z$. The center of $Z$ is moved to $\bar{\mbf{h}}$ using Proposition \ref{propo:center} and $\mbf{h}$ is given by $\mbf{h}=\bar{\mbf{h}}$.\footnote{If the center of the interval hull is not in $Z$, $\bar{\mbf{h}}$ can be chosen as the point obtained from Proposition \ref{propo:closest} instead.}
\end{itemize}

To evaluate the effect of different choices of $\mbf{h}$, we again consider one-step reachability analysis of the nonlinear system \eqref{eq:model2} with $X_0$ given by \eqref{eq:reachX0}. Figure \ref{fig:reachable_firstorder} shows the constrained zonotope $X_0$ and the enclosures of the one-step reachable set obtained by Theorem \ref{thm:firstorder} with \emph{C3}--\emph{C6}. Since the complexity of the enclosure for \emph{C6} is higher than for the other methods (see Proposition \ref{propo:center}), the reduction Methods \ref{meth:czgenred} and \ref{meth:czconelim} in the Appendix were used to reduce the number of generators and constraints in this enclosure to match the other methods before comparison. Clearly, the enclosures produced by Theorem \ref{thm:firstorder} are strongly affected by the choice of $\mbf{h}$, with \emph{C6} providing the least conservative result. In addition, note that the enclosures provided by the first-order Taylor extension are more conservative than those obtained by the mean value extension (see Figure \ref{fig:reachable_firstorder}). However, experience with zonotopes and intervals \citep{Raimondo2012} suggests that the relative merits of these two methods will depend on the dynamics of the system, as well as the shape and size of the set $X_0$. Therefore, one cannot affirm that one extension will provide tighter results than the other in general.

\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}
			{fig_reach_X1_model2_firstorder_withC5_andMV_newobjfun.pdf_tex}}
		\caption{Left: Constrained zonotope $X_0$ with `$\times$' denoting its center. Right: Enclosures obtained by applying Theorem \ref{thm:firstorder} to \eqref{eq:model2} with $\mbf{h}$ determined by \emph{C3} (yellow), \emph{C4} (green), \emph{C5} (blue), and \emph{C6} (red). Dashed lines denote the set obtained using Theorem \ref{the:pred2} with \emph{C3}.}\label{fig:reachable_firstorder}}
\end{figure}

\begin{remark} \rm
	Similarly to the mean value extension (Section \ref{sec:meanvalue}), given the prediction set $\bar{X}_k$ obtained using the first-order Taylor extension (Theorem \ref{thm:firstorder}) described by a constrained zonotope, the update step \eqref{eq:updatelinear0} is computed by the generalized intersection of two constrained zonotopes. This operation is given by \eqref{eq:updatemeanvalue}. Complexity reduction issues are addressed as discussed in Section \ref{sec:meanvalueupdate}.
\end{remark}

\subsection{Numerical examples}

\subsubsection{Example 1}

This section presents a numerical experiment to demonstrate the performance of the CZIB algorithm. 

We address the second example presented in \cite{Alamo2005a}. Consider a isothermal gas-phase reactor, charged with an initial amount of $A$ and $B$, in which the species are allowed to react according to the reversible reaction $2A \rightleftharpoons B$. Define the system states as the partial pressure of each species in the reactor. The objective is to estimate all the system states while measuring the total pressure of the vessel as the reaction proceeds. The dynamic equations of the system are given by (discretized through Euler)
\begin{align*}
x_{1,k} & = x_{1,k-1} + T_s \left( -2k_1 x_{1,k-1}^2  + 2k_2 x_{2,k-1}\right) + k_3 w_{1,k-1}, \\
x_{2,k} & = x_{2,k-1} + T_s \left( k_1 x_{1,k-1}^2  - k_2 x_{2,k-1}\right) + k_3 w_{2,k-1},
\end{align*}
%where $k_1 = 0.16/60$ s$^{-1}$ atm$^{-1}$, $k_2 = 0.0064/60$ s$^{-1}$ and $T_s = 6$ s. The measured output is given by $y_k = \begin{bmatrix} 1 & 1 \end{bmatrix} \bm{x}_k + v_k$, %
where $k_1 = 0.16/60$ s$^{-1}$ atm$^{-1}$, $k_2 = 0.0064/60$ s$^{-1}$, $k_3 = 0.0001$ and $T_s = 6$ s \citep{Alamo2005a}. The measured output is given by $y_k = \begin{bmatrix} 1 & 1 \end{bmatrix} \bm{x}_k + v_k$. Existing disturbances are bounded by $\ninf{\bm{w}_k} \leq 1$, 
and $\ninf{v_k} \leq 0.3$. The initial states are assumed to belong to the constrained zonotope
\begin{equation*}
\bar{X}_0 \triangleq \left\{ \begin{bmatrix} 2.5 & 0 & 1.0 \\ 0 & 0.5 & 1.0 \end{bmatrix}, \begin{bmatrix} 2.5 \\ 1.0 \end{bmatrix}, \begin{bmatrix} 1 & 0 & 1 \end{bmatrix}, 1 \right\}.
\end{equation*}

In the experiment, we use 12-partitions for Algorithm \ref{alg:o1} and the natural interval extension \citep{Moore2009} for Algorithm \ref{alg:o2}. An experiment using 3-partitions is also conducted to evaluate the resulting conservatism. The inclusion functions were computed using the INTLAB toolbox \citep{Rump1999}. The conversion from V-rep to H-rep in Algorithm \ref{alg:firstconvexpoly} was performed using the MPT toolbox \citep{Herceg2013}. Moreover, we perform an initial correction step $\hat{X}_0 = \bar{X}_0 \ginter{C} Y_0$ to obtain tighter initial bounds, where $Y_0 = \bm{y}_0 \oplus (- \bm{D}_v V_0)$. For comparison, a third experiment is conducted using the algorithm proposed in \cite{Combastel2005}, based on first-order Taylor approximation by zonotopes, with complexity limited to 20 generators using the reduction algorithm described in Method \ref{meth:genredA} in the Appendix. The real initial states are $\bm{x}_0 = \begin{bmatrix} 4.9 \,\; 1.5 \end{bmatrix}^T$.

Fig. \ref{fig:results} shows the time evolution of the system states, and the estimated bounds provided by the CZIB algorithm\footnote{The plotted curves are the bounds of the interval hull of $\hat{X}_k$.}, and the algorithm in \cite{Combastel2005}. Although reasonable for $x_1$, the bounds obtained using the latter are substantially conservative for $x_2$. Besides, the bounds obtained using the 12-partition CZIB are significantly less conservative in all cases, demonstrating the attained reduction in overestimation using the proposed method. In order to bypass the ``simplex problem'' (Section \ref{sec:thealgorithm}), a Minkowski sum was performed using a zero-centered interval vector, with $10\%$ of the total diameter, at every time it occurred. To conclude, the description of the constrained zonotope $\hat{X}_{40}$ in the 12-partition experiment was given by modest 13 generators and 9 constraints, without using any complexity reduction algorithm. The average execution times for the 3-partition and 12-partition experiments were $0.0855$ and $0.6013$ seconds per iteration, respectively, in MATLAB and CPLEX, with 8GB RAM and Intel Core i7 4510U 3.1 GHz processor, using only sequential computation.


\begin{figure}[!tb]
	%\vspace{1.5mm}
	\begin{footnotesize}
		\centering{
			\def\svgwidth{0.7\columnwidth}			
			\import{Figures_ECC/}{fig_results_3_12_Combastel.pdf_tex}\vspace{-2mm}
			\caption{Time evolution of the estimated bounds and the real states.}\label{fig:results}}
		%\vspace{-5mm}
	\end{footnotesize}
\end{figure}


\subsubsection{Example 2}

This section presents numerical results for the two new set-valued state estimation methods enabled by the new extensions proposed in Sections \ref{sec:meanvalue} and \ref{sec:firstorder}. Specifically, we use the mean value extension (Theorem \ref{the:pred2}) and the first-order Taylor extension (Theorem \ref{thm:firstorder}) for the prediction steps, while the update steps are both given by the exact intersection \eqref{eq:updatelinear}. These methods are denoted by CZMV and CZFO, respectively. The results are compared against two zonotopic methods denoted analogously by ZMV and ZFO, which use the mean value approach in \cite{Alamo2005a} and the first-order Taylor approach in \cite{Combastel2005}, respectively, for the prediction step. The update algorithm proposed in \cite{Bravo2006} is used for both ZMV and ZFO because it provided the best trade-off between accuracy and efficiency in our numerical experiments with zonotopes. Complexity reduction is applied after the update step in all four methods using Methods \ref{meth:czgenred} and \ref{meth:czconelim} for constrained zonotopes and Method \ref{meth:genredB} for zonotopes. The imposed complexity limits are described separately for each example below.



%\subsection{Example 1}
We first consider an uncertain nonlinear discrete-time system described by \citep{Raimondo2012}:
\begin{equation} \label{eq:model1}
\begin{aligned}
x_{1,k} & = 3 x_{1,k-1} - \frac{x_{1,k-1}^2}{7} - \frac{4 x_{1,k-1} x_{2,k-1}}{4 + x_{1,k-1}} + w_{1,k-1}, \\
x_{2,k} & = -2 x_{2,k-1} + \frac{3 x_{1,k-1} x_{2,k-1}}{4 + x_{1,k-1}} + w_{2,k-1},
\end{aligned}% \right.
\end{equation}
with linear measurement equation
\begin{equation} \label{eq:model1meas}
\begin{bmatrix} y_{1,k} \\ y_{2,k} \end{bmatrix} = \begin{bmatrix} 1 & 0 \\ -1 & 1 \end{bmatrix} \begin{bmatrix} x_{1,k} \\ x_{2,k} \end{bmatrix} + \begin{bmatrix} v_{1,k} \\ v_{2,k} \end{bmatrix},% \bm{v}_k.
\end{equation}
where $\mbf{w}_k, \mbf{v}_k \in \realset^2$ denote process and measurement uncertainties, respectively, bounded by $\ninf{\mbf{w}_k} \leq 0.4$ and $\ninf{\mbf{v}_k} \leq 0.4$. The initial states $\mbf{x}_0$ are bounded by the zonotope\footnote{Equality constraints are not present in $X_0$ for the purpose of comparison with zonotope-based methods.}
\begin{equation} \label{eq:model1X0}
X_0 = \left\{ \begin{bmatrix} 0.1 & 0.2 & -0.1 \\ 0.1 & 0.1 & 0 \end{bmatrix}, \begin{bmatrix} 0.5 \\ 0.5 \end{bmatrix}\right\}.
\end{equation}


To generate process measurements, \eqref{eq:model1} was simulated with $\mbf{x}_0 = (0.8,0.65) \in X_0$ and process and measurement uncertainties drawn from uniform random distributions. The number of generators and constraints of the constrained zonotopes was limited to 20 and 5, respectively, while the number of generators of the zonotopes was limited to 20. Figure \ref{fig:model1_update} shows the results of the initial update step using the intersection algorithm in \cite{Bravo2006} and the generalized intersection \eqref{eq:updatemeanvalue} computed using \eqref{eq:czintersection}, which yields a constrained zonotope. Clearly, since the exact intersection is not a symmetric set, it cannot be described by a zonotope. In contrast, the resulting constrained zonotope corresponds to the exact intersection, providing far less conservative bounds in the first update step.


\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.6\columnwidth}
		{\footnotesize\import{Figures_Automatica/}{fig_model1_initialupdate_v2.pdf_tex}}
		\caption{The initial set $X_0$ (gray), the initial bounded uncertain measurements (dashed lines), the intersection computed as in \cite{Bravo2006} (yellow), and the constrained zonotope (green) computed by \eqref{eq:updatemeanvalue}.}\label{fig:model1_update}}
\end{figure}


 
Figure \ref{fig:model1_meanvalue_4iter} shows the first four time steps of CZMV with $\mbf{h}$ given by \emph{C3} in a scenario without process uncertainties ($\mbf{w}_k = \bm{0}$). For comparison, the zonotopes computed using ZMV are also depicted. CZMV provides much less conservative enclosures than {\alamobravo} for this example, demonstrating the effectiveness of the proposed nonlinear state estimation strategy. 

\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.6\columnwidth}
		{\footnotesize\import{Figures_Automatica/}{fig_model1_meanvalue_4iter_v2.pdf_tex}}
		\caption{Results from the first four time steps of set-valued state estimation (after update) using the constrained zonotopic method CZMV (green) and the zonotopic method {\alamobravo} (yellow).}\label{fig:model1_meanvalue_4iter}}
\end{figure}


Figure \ref{fig:model1_meanvalue_radius} shows the radii (half the length of the longest edge of the interval hull) of the sets provided by CZMV and {\alamobravo} over 100 time steps. CZMV provides less conservative bounds than {\alamobravo}, with the average CZMV-to-ZMV radius ratio (i.e., the ratio of the radius of the CZMV set at $k$ over the ZMV set at $k$ averaged over all time steps $k$) being only $29.8\%$.


\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_model1_meanvalue_radius.pdf_tex}}
		\caption{Radii of the update sets obtained by applying CZMV ($\triangle$) and {\alamobravo} ($\circ$) to \eqref{eq:model1} without process disturbances ($\mbf{w}_k = \bm{0}$).}\label{fig:model1_meanvalue_radius}}
\end{figure}

\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}%{fig_model1_firstorder_radius.pdf_tex}}
			{fig_model1_firstorder_radius_newobjfun.pdf_tex}}
		\caption{Radii of the update sets obtained by applying CZFO ($\triangle$) and {\combastelbravo} ($\circ$) to \eqref{eq:model1} without process disturbances ($\mbf{w}_k = \bm{0}$).}\label{fig:model1_firstorder_radius}}
\end{figure}


Figure \ref{fig:model1_firstorder_radius} compares the radii of the update sets computed by {\combastelbravo} and CZFO with $\mbf{h}$ given by \emph{C6}. As in the previous case, CZFO provides less conservative bounds than {\combastelbravo}, with the CZFO-to-ZFO average radius ratio (ARR) being only $37.69\%$. The size of the sets provided by CZMV and CZFO were quite similar, with CZFO being less conservative (the CZFO-to-CZMV ARR was $72.55\%$).


\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_model1_meanvalue_radius_w.pdf_tex}}
		\caption{Radii of the update sets obtained by applying CZMV ($\triangle$) and {\alamobravo} ($\circ$) to \eqref{eq:model1} with process disturbances.}\label{fig:model1_meanvalue_radiusw}}
\end{figure}


Figure \ref{fig:model1_meanvalue_radiusw} shows the radii of the sets provided by CZMV and {\alamobravo} considering process disturbances. Since \eqref{eq:model1} is affine in $\mbf{w}_k$, the enclosure $Z \supseteq \bm{\mu}(\mbf{h},W)$ in Theorem \ref{the:pred2} was computed as described at the end of Remark \ref{rem:affine}. Once again, CZMV provided less conservative bounds than the zonotopes computed by {\alamobravo}, with a CZMV-to-{\alamobravo} ARR of $51.4\%$. Figure \ref{fig:model1_firstorder_radiusw} shows that the radii of the sets provided by CZFO are similarly smaller than those from {\combastelbravo}, with a CZFO-to-{\combastelbravo} ARR of $53.65\%$. Lastly, CZFO provided slightly less conservative bounds than CZMV (the CZFO-to-CZMV ARR was $98.72\%$).


The use of constrained zonotopes in CZMV and CZFO results in sets that are slightly more complex than those generated by ZMV and ZFO (specifically, the set description involves five equality constraints that are not present in the zonotopes from ZMV and ZFO). However, this example shows that this increase in complexity is compensated by greatly improved accuracy.


\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}%{fig_model1_firstorder_radius_w.pdf_tex}}
			{fig_model1_firstorder_radius_w_newobjfun.pdf_tex}}
		\caption{Radii of the update sets obtained by applying CZFO ($\triangle$) and {\combastelbravo} ($\circ$) to \eqref{eq:model1} with process disturbances.}\label{fig:model1_firstorder_radiusw}}
\end{figure}



\subsubsection{Example 3} \label{sec:nonlinearestimationex2}
This section evaluates the numerical results provided by the extensions proposed in Sections \ref{sec:meanvalue} and \ref{sec:firstorder} when applied to  nonlinear set-valued state estimation of a UAV.% to  when applied to a high-dimensional system.

Consider the quadrotor UAV described in \cite{Mistler2001} with state vector $\bm{\zeta} = [x\,\;y\,\;z\,\;u_0\,\;v_0\,\;w_0\,\;\phi\,\;\theta\,\;\psi\,\;p\,\;q\,\;r]^T$, where $[x\,\;y\,\;z]^T$ is the position of the UAV with respect to the inertial frame, $[u_0\,\;v_0\,\;w_0]^T$ is the velocity vector expressed in the inertial frame, $[\phi\,\;\theta\,\;\psi]^T$ are Euler angles describing the orientation of the UAV, and $[p\,\;q\,\;r]^T$ is the angular velocity vector expressed in the body frame. The equations of motion are \citep{Mistler2001}:
\begin{equation} \label{eq:quadrotor}
\dot{\bm{\zeta}} = 
\left\{ \begin{aligned}
\dot{x} & = u_0, \\
\dot{y} & = v_0, \\
\dot{z} & = w_0, \\
\dot{u}_0 & = \frac{1}{m} (\cos\psi \sin\theta \cos\phi + \sin\psi \sin\phi)U_1 + \frac{1}{m}D_x, \\
\dot{v}_0 & = \frac{1}{m} (\sin\psi \sin\theta \cos\phi - \cos\psi \sin\phi)U_1 + \frac{1}{m}D_y, \\
\dot{w}_0 & = -g + \frac{1}{m} (\cos\theta \cos\phi)U_1 + \frac{1}{m}D_z, \\
\dot{\phi} & = p + q \sin\phi \tan\theta + r \cos\phi \tan\theta, \\
\dot{\theta} & = q \cos\phi- r \sin\phi, \\
\dot{\psi} & = q \sin\phi \sec\theta + r \cos\phi \sec\theta, \\
\dot{p} & = \frac{I_{yy} - I_{zz}}{I_{xx}} qr + \frac{l}{I_{xx}} U_2, \\
\dot{q} & = \frac{I_{zz} - I_{xx}}{I_{yy}} pr + \frac{l}{I_{yy}} U_3, \\
\dot{r} & = \frac{I_{xx} - I_{yy}}{I_{zz}} pq + \frac{1}{I_{zz}} U_4,
\end{aligned} \right.
\end{equation}
where $m$, $I_{xx}$, $I_{yy}$, $I_{zz}$, and $l$ are physical parameters, $g$ is the gravitational acceleration, $U_1$ is the total thrust generated by the propellers, $U_2$ is the difference of thrusts between the left and right propellers, $U_3$ is the difference of thrusts between the front and back propellers, $U_4$ is the difference of torques between clockwise and counter-clockwise turning propellers, and $\mbf{d} = [D_x \,\; D_y \,\; D_z]^T$ are disturbance forces applied to the UAV with $\ninf{\mbf{d}} \leq 1$. The experiment consists in obtaining guaranteed bounds on the system states $\bm{\zeta}$ while the quadrotor UAV tracks a vertical helix trajectory defined by the reference values
\begin{gather*}
x^\text{ref}(t) = \frac{1}{2} \cos\left(\frac{t}{2}\right), \; y^\text{ref}(t) = \frac{1}{2} \cos\left(\frac{t}{2}\right), \\
z^\text{ref}(t) = 1 + \frac{t}{10}, \quad \psi^\text{ref} = \frac{\pi}{3},
\end{gather*}
subject to the disturbance forces described in Table \ref{tab:disturbances}.

\begin{table}[!htb]
	\footnotesize
	\centering
	\caption{Disturbance forces applied to the UAV in Newtons (N).}
	\begin{tabular}{c c c c} \hline
		Time (s) & $D_x$ \text{(N)} & $D_y$ \text{(N)} & $D_z$ \text{(N)} \\ \hline
		$0 \leq t < 5$ & $0$ & $0$ & $0$ \\
		$5 \leq t < 8$ & $1$ & $0$ & $0$ \\
		$8 \leq t < 10$ & $1$ & $1$ & $0$ \\		
		$10 \leq t < 15$ & $1$ & $1$ & $1$ \\				
		\hline
	\end{tabular} \normalsize
	\label{tab:disturbances} 	
\end{table}


%The dynamic feedback controller in \cite{Mistler2001} is used to track the reference trajectory above\footnote{In this experiment, the control action is computed using the real states $\bm{\zeta}_k$. The approach in \cite{Rego2018b} can be used for feedback connection using a point that belongs to $\hat{X}_k$.}. The simulation parameters are shown in Table \ref{tab:results_UAVparameters}. We consider a realistic scenario in which the available measurements are provided by sensors located at the quadrotor UAV, which include: (i) a Global Positioning System (GPS); (ii) a barometer; and (iii) an Inertial Measurement Unit (IMU). The measurements are affected by bounded uncertainties as described in Table \ref{tab:results_sensorparameters}. The velocity vector $[u_0\,\;v_0\,\;w_0]^T$ is not measured.

The dynamic feedback controller in \cite{Mistler2001} is used to track the reference trajectory above\footnote{Since the objective of this experiment is to evaluate the accuracy of the state estimation, the control action is computed using the real states $\bm{\zeta}_k$. The minimum variance criterion proposed in Section \ref{sec:minimumvariance} could be used for feedback connection using a point that belongs to $\hat{X}_k$.}. The simulation parameters are shown in Table \ref{tab:results_UAVparameters}. We consider a realistic scenario in which the available measurements are provided by sensors located at the quadrotor UAV, which include: (i) a Global Positioning System (GPS); (ii) a barometer; and (iii) an Inertial Measurement Unit (IMU). The measurements are affected by bounded uncertainties as described in Table \ref{tab:results_sensorparameters}. The velocity vector $[u_0\,\;v_0\,\;w_0]^T$ is not measured.

\begin{table}[!htb]
	\footnotesize
	\centering
	\caption{Parameters considered in the experiment.}
	\begin{tabular}{c c c c c} \hline
		Parameter & $m$ & $l$ & $I_{xx},I_{yy},I_{zz}$ & $g$ \\ \hline
		Value & $0.7$ Kg & $0.3$ m & $1.2416$ & $9.81$ m/s$^2$ \\ %\hline
		\hline
	\end{tabular} \normalsize
	\label{tab:results_UAVparameters}
\end{table}

\begin{table}[!htb]
	\footnotesize
	%\small
	\centering
	\caption{Measured variables with error bounds.}
	\begin{tabular}{c c c} \hline
		Sensor & Variables & Noise bounds \\ \hline
		GPS & $\{x,y\}$ & $\pm\!\!$ $0.15\!$ m \\ %\hline
		Barometer & $\{z\}$ & $\pm\!\!$ $0.51\!$ m \\ %\hline
		\multirow{2}{*}{IMU} & $\{\phi,\theta,\psi\}$ & $\pm\!\!$ $2.618 {\cdot} 10^{-3}\!$ rad \\
		& $\{p,q,r\}$ & $\pm\!\!$ $16.558 {\cdot} 10^{-3}\!$ rad/s \\%\hline      
		\hline
	\end{tabular} \normalsize
	\label{tab:results_sensorparameters}
\end{table}


The nonlinear equations \eqref{eq:quadrotor} were discretized by Euler approximation with sampling time $0.01$ s. The initial states $\bm{\zeta}_0$ are bounded by $X_0 = \{\mbf{G}_0,\bm{0}\}$, where
\begin{align*}
\mbf{G}_0 = \text{diag}\left(2, 2, 2, 1, 1, 1, \frac{\pi}{6}, \frac{\pi}{6}, \frac{\pi}{2}, \frac{\pi}{12}, \frac{\pi}{12}, \frac{\pi}{12}\right).
\end{align*}


To generate process measurements, the discrete-time dynamics were simulated with $\bm{\zeta}_0  = [0.5\,\;0\,\;1\,\; \zeros{1}{5} \,\; \pi/3\,\; \zeros{1}{3} ]^T \in X_0$ and process and measurement noises drawn from uniform distributions. Figure \ref{fig:quadrotor_trajectory_boxes} shows the trajectory performed by the quadrotor UAV along with the interval hulls\footnote{The conversion from CG-rep to H-rep (see \cite{Scott2016}) for the purposes of exact drawing is intractable for the constrained zonotopes in this example.} of the enclosures computed by the methods CZMV and {\alamobravo}, projected onto $(x,y,z)$-axes. CZMV was implemented with $\mbf{h}$ given by \emph{C3}, and since \eqref{eq:quadrotor} is also affine in $\mbf{w}_k \triangleq \mbf{d}_k$, Theorem \ref{thm:firstorder} was implemented with $Z \supseteq \bm{\mu}(\mbf{h},W)$ computed as described at the end of Remark \ref{rem:affine}. The number of constraints and generators of the computed constrained zonotopes was limited to 60 and 18, respectively, while the number of generators of the computed zonotopes was limited to 60. 

The interval hulls of the constrained zonotopes obtained by CZMV were smaller than those from {\alamobravo}, demonstrating the accuracy of the proposed method. Figure \ref{fig:quadrotor_meanvalue_radius} shows the radii of the constrained zonotopes and zonotopes computed by CZMV and {\alamobravo}, respectively. Both algorithms were capable of providing tight bounds on the system states $\bm{\zeta}_k \in \realset^{12}$. Nevertheless, CZMV provided less conservative bounds than {\alamobravo}, even for a high-order nonlinear dynamical system such as \eqref{eq:quadrotor} (the CZMV-to-{\alamobravo} ARR was $71.2\%$).



\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_quadrotor_trajectory_boxes_distfinal.pdf_tex}}
		\caption{The trajectory performed by the quadrotor UAV (solid line) and the interval hulls of the constrained zonotopes (red boxes) and zonotopes (green boxes) estimated by CZMV and ZMV, respectively, projected onto $(x, y, z)$.}\label{fig:quadrotor_trajectory_boxes}}
\end{figure}

Finally, Figure \ref{fig:quadrotor_firstorder_radius} compares the radii of the update sets computed by {\combastelbravo} and CZFO with $\mbf{h}$ given by \emph{C5}\footnote{The increased complexity of the constrained zonotopes provided by \emph{C6} proved to be intractable for this example.}. Once again, CZFO provided less conservative bounds than {\combastelbravo} (the CZFO-to-{\combastelbravo} ARR was $72.6\%$). The results from CZMV and CZFO were again very similar, with CZMV providing marginally better results (the CZMV-to-CZFO ARR was $97.9\%$). 


\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_quadrotor_meanvalue_dist_radius.pdf_tex}}
		\caption{Radii of the update sets computed by CZMV ($\triangle$) and {\alamobravo} ($\circ$) for the quadrotor UAV experiment.}\label{fig:quadrotor_meanvalue_radius}}
\end{figure}

\begin{figure}[!tb]
	\centering{
		\def\svgwidth{0.7\columnwidth}
		{\scriptsize\import{Figures_Automatica/}{fig_quadrotor_firstorder_dist_radius.pdf_tex}}
		\caption{Radii of the update sets computed by CZFO ($\triangle$) and {\combastelbravo} ($\circ$) for the quadrotor UAV experiment.}\label{fig:quadrotor_firstorder_radius}}
\end{figure}

\section{Nonlinear measurement} \label{sec:nonlinearmeasurement}

In this section we describe a new method based on constrained zonotopes to perform set-valued state estimation of nonlinear systems considering nonlinear measurement.% using constrained zonotopes.

\subsection{Problem formulation}

Consider a class of nonlinear discrete-time systems described by
\begin{equation}
\begin{aligned} \label{eq:nonlinearmeasurement}
\mbf{x}_k & = \mbf{f}(\mbf{x}_{k-1}, \mbf{u}_{k-1}, \mbf{w}_{k-1}), \\
\mbf{y}_k & = \mbf{g}(\mbf{x}_k, \mbf{u}_{k}, \mbf{v}_{k}),	
\end{aligned}
\end{equation}
for $k \geq 1$, with $\mbf{y}_0 = \mbf{g}(\mbf{x}_0, \mbf{u}_0, \mbf{v}_0)$, where $\mbf{x}_k \in \realset^{n_x}$ denotes the system state, $\mbf{u}_{k} \in \realset^{n_u}$ is a known input, $\mbf{w}_k \in \realset^{n_w}$ is the process uncertainty, $\mbf{y}_k \in \realset^{n_y}$ is the measured output, and $\mbf{v}_k \in \realset^{n_v}$ is the measurement uncertainty. The nonlinear mappings $\mbf{f}$ and $\mbf{g}$ are assumed to be of class $\mathcal{C}^2$, and the uncertainties are assumed to be bounded, i.e., $\mbf{w}_{k} \in W_k$ and $\mbf{v}_k \in V_k$, where $W_k$ and $V_k$ are known compact sets.


The set-valued state estimation approach for the discrete-time system with nonlinear dynamics and measurement \eqref{eq:nonlinearmeasurement} is stated as follows. Given an initial set $\mbf{x}_0 \in \hat{X}_0$, the previous estimate bounds $\hat{X}_{k-1}$, the known inputs $\mbf{u}_{k-1}$, $ \mbf{u}_k$, the current measurement $\mbf{y}_k$, and the bounds on the uncertainties $W_{k-1}$, $V_k$, the prediction-update algorithm consists in computing real compact sets $\bar{X}_k$ and $\hat{X}_k$ satisfying
\begin{align}
\bar{X}_k & \supseteq \{ \mbf{f}(\mbf{x}, \mbf{u}_{k-1}, \mbf{w}) : \mbf{x} \in \hat{X}_{k-1}, \, \mbf{w} \in W_{k-1} \}, \label{eq:predictionnonlinearmeas}\\
\hat{X}_k & \supseteq \{ \mbf{x} \in \bar{X}_k : \mbf{g}(\mbf{x}, \mbf{u}_k, \mbf{v}) = \mbf{y}_k, \, \mbf{v} \in V_k \}, \label{eq:updatenonlinear}
\end{align}
in which \eqref{eq:predictionnonlinearmeas} is referred to as the prediction step, and \eqref{eq:updatenonlinear} as the update step. The goal is to obtain accurate outer bounds $\bar{X}_k$ and $\hat{X}_k$ according to \eqref{eq:predictionnonlinearmeas} and \eqref{eq:updatenonlinear}, respectively. As in Section \ref{sec:nonlinearformulation}, following these definitions and considering the initial condition $\mbf{x}_0 \in \hat{X}_0$, the property $\mbf{x}_k \in \hat{X}_k$ is guaranteed by construction for all $k \geq 0$ \citep{Chisci1996,Le2013,Alamo2008}.

\subsection{Proposed method}

This section sketches a new method to perform set-valued state estimation for nonlinear systems as in \eqref{eq:system}. In contrast to the problem stated in Section \ref{sec:nonlinearformulation}, the update step \eqref{eq:updatenonlinear} can not be directly formulated using the generalized intersection as in \eqref{eq:updateczib}.

Clearly, enclosures satisfying the prediction step \eqref{eq:predictionnonlinearmeas} can be straightforwardly obtained using the mean value extension and first-order Taylor extension proposed in the previous sections, since this is the same as \eqref{eq:prediction0}. Therefore, the associated procedure is omitted. On the other hand, tight enclosures satisfying \eqref{eq:updatenonlinear} are hard to obtain, being addressed in the literature by methods based on set inversion \citep{Jaulin2009}, whose complexity scale exponentially with the system dimension, and methods based on strips and zonotopes \citep{Alamo2005a,Alamo2008}, which demonstrated to be substantially conservative in several numerical experiments performed during the elaboration of this doctoral thesis. We propose a method based on constrained zonotopes and the first-order Taylor extension developed in Theorem \ref{thm:firstorder}, from which we are able to reformulate the update step \eqref{eq:updatenonlinear} as the generalized intersection of two constrained zonotopes.

\begin{theorem} \rm \label{thm:nonlinearmeasurement}
	Let $\bm{\kappa}: \realset^n \times \realset^m \to \realset^p$ be of class $\mathcal{C}^2$ and let $\mbf{x} \in \realset^n$ and $\mbf{v} \in \realset^m$ denote its arguments. Let $\kappa_q$ denote the $q$-th component of $\bm{\kappa}$, and let $\mbf{H} \kappa_q$ denote an upper triangular matrix describing half of the Hessian of $\kappa_q$. Specifically, let $H_{ii} \kappa_q = (1/2) \partial^2 \kappa_q/\partial z_i^2$, $H_{ij} \eta_q = \partial^2 \eta_q/\partial z_i \partial z_j$ for $i<j$, and $H_{ij} \eta_q = 0$ for $i>j$, where $\mbf{z} = (\mbf{x},\mbf{v})$. Let $X = \{\mbf{G}_x, \mbf{c}_x, \mbf{A}_x, \mbf{b}_x\}$ and  $V = \{\mbf{G}_v, \mbf{c}_v, \mbf{A}_v, \mbf{b}_v\}$ be constrained zonotopes with $n_g$ generators and $n_c$ constraints, and with $m_g$ generators and $m_c$ constraints, respectively, and let $\bm{y} \in \realset^p$ such that $\exists \mbf{x} \in X$, $\mbf{v} \in V : \bm{\kappa}(\mbf{x},\mbf{v}) = \mbf{y}$. Let $Z = X \times V = \{\mbf{G}, \mbf{c}, \mbf{A}, \mbf{b}\} \subset \realset^{n+m}$. For each $q = 1,2,\dots,p$, let $\mbf{Q}^{[q]}\in\mathbb{IR}^{(n+m)\times (n+m)}$ and $\tilde{\mbf{Q}}^{[q]}\in\mathbb{IR}^{(n_g+m_g)\times (n_g+m_g)}$ be interval matrices satisfying $\mbf{Q}^{[q]} \supseteq \mbf{H} \kappa_q (Z)$ and $\tilde{\mbf{Q}}^{[q]} \supseteq \mbf{G}^T \mbf{Q}^{[q]} \mbf{G}$. Moreover, define    
	\begin{align*}
	& \tilde{c}_q = \trace{\midpoint{\tilde{\mbf{Q}}^{[q]}}}/2, \\
	& \tilde{\mbf{G}}_{q,:} = \big[ \cdots \,\; \underbrace{\midpoint{\tilde{Q}^{[q]}_{ii}}/2}_{\forall i} \,\; \cdots \,\; \underbrace{\left(\midpoint{\tilde{Q}^{[q]}_{ij}} + \midpoint{\tilde{Q}^{[q]}_{ji}}\right)}_{\forall i<j} \,\; \cdots \big], \\
	& \tilde{\mbf{G}}_{\mbf{v}} = \text{diag}(\mbf{v}), \quad v_q = \sum_{i,j} \left| \rad{\tilde{Q}^{[q]}_{ij}} \right|, \\
	& \tilde{\mbf{A}} = \left[ \tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \bm{0} \right],\\
	& \tilde{\mbf{A}}_{\bm{\zeta}} = \arrowmatrix{\begin{matrix} & \vdots & \\ \cdots & \half A_{ri} A_{si} & \cdots \\ & \vdots & \end{matrix}}{\forall i}{\forall r \leq s}, \quad \tilde{\mbf{A}}_{\bm{\xi}} = 
	\arrowmatrix{\begin{matrix} & \vdots & \\ \cdots & A_{ri} A_{sj} + A_{rj} A_{si} & \cdots \\ & \vdots & \end{matrix}}{\forall i < j}{\forall r \leq s}, \\
	& \tilde{\mbf{b}} = \downarrowmatrix{\begin{matrix} \vdots \\ b_{r} b_{s} - \half \sum_i A_{ri} A_{si} \\ \vdots\end{matrix}}{\forall r \leq s},
	\end{align*}
	with indices $i,j = 1,2,\dots,(n_g+m_g)$ and $r,s = 1,2,\dots,(n_c+m_c)$. Finally, choose any $\mbf{h} = (\mbf{h}_x, \mbf{h}_v) \in Z$ and let $\mbf{L}\in\mathbb{IR}^{p\times (n+m)}$ be an interval matrix satisfying $\mbf{L}_{q,:} \supseteq (\mbf{c} - \mbf{h})^T \mbf{Q}^{[q]}$ for all $q = 1,\dots,p$. Then, $\{ \mbf{x} \in X : \bm{\kappa}(\mbf{x}, \mbf{v}) = \mbf{y}, \, \mbf{v} \in V \} \subseteq X \ginter{\mbf{C}} Y$, where $\mbf{C} = \nabla^T_x \bm{\kappa}(\mbf{h})$,
	\begin{equation} \label{eq:nonlinearmeasurementmethod}
	%\bm{\eta}(Z) \subseteq \bm{\eta}(\mbf{h}) \oplus \nabla^T \bm{\eta}(\mbf{h})(Z - \mbf{h}) \oplus R,
	Y = (\mbf{y} - \bm{\kappa}(\mbf{h}) + \nabla^T_x \bm{\kappa}(\mbf{h})\mbf{h}_x + \nabla^T_v \bm{\kappa}(\mbf{h})\mbf{h}_v) \oplus (- \nabla^T_v \bm{\kappa}(\mbf{h}) V) \oplus (-R),
	\end{equation}
	and
	\begin{align}
	R = \tilde{\mbf{c}} &\oplus [ \tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}} ] B_\infty(\tilde{\mbf{A}}, \tilde{\mbf{b}}) \oplus \gzinclusion (\mbf{L}, (\mbf{c} - \mbf{h}) \oplus 2\mbf{G} B_\infty(\mbf{A},\mbf{b}) ). \nonumber
	\end{align}
\end{theorem}


\proof
Choose $\mbf{z} = (\mbf{x},\mbf{v}) \in Z$ such that $\bm{\kappa}(\mbf{x}, \mbf{v}) = \mbf{y}$, and any $q\in\{1,\ldots,p\}$. By Taylor's theorem applied to $\kappa_q$ with reference point $\mbf{h}$, there must exist $\bm{\Gamma}^{[q]} \in \mbf{H} \kappa_q (Z) \subseteq \mbf{Q}^{[q]}$ such that \citep{Combastel2005}
\begin{align*}
%\eta_q(\mbf{z}) & = \eta_q (\mbf{h}) + \nabla^T \eta_q (\mbf{h})(\mbf{z} - \mbf{h}) + (\mbf{z} - \mbf{h})^T \bm{\Gamma}^{[q]} (\mbf{z} - \mbf{h}). \nonumber
y_q & = \kappa_q (\mbf{h}) + \nabla^T_x \kappa_q (\mbf{h})(\mbf{x} - \mbf{h}_x) + \nabla^T_v \kappa_q (\mbf{h})(\mbf{v} - \mbf{h}_v) + (\mbf{z} - \mbf{h})^T \bm{\Gamma}^{[q]} (\mbf{z} - \mbf{h}).
\end{align*}
Since $\mbf{z}\in Z$, there must exist $\bm{\xi} \in B_\infty(\mbf{A},\mbf{b})$ such that $\mbf{z}=\mbf{c} + \mbf{G}\bm{\xi}$. Thus, defining $\mbf{p} = \mbf{c} - \mbf{h}$ for brevity,
%\begin{align*}
%\eta_q(\mbf{z}) & = \eta_q (\mbf{h}) + \nabla^T \eta_q (\mbf{h})(\mbf{p} + \mbf{G}\bm{\xi}) \\
%& \quad + (\mbf{p} + \mbf{G}\bm{\xi})^T \bm{\Gamma}^{[q]}  (\mbf{p} + \mbf{G}\bm{\xi}).
%\end{align*}
\begin{align*}
y_q = \kappa_q (\mbf{h}) + \nabla^T_x \kappa_q (\mbf{h})(\mbf{x} - \mbf{h}_x) + \nabla^T_v \kappa_q (\mbf{h})(\mbf{v} - \mbf{h}_v) + (\mbf{p} + \mbf{G}\bm{\xi})^T \bm{\Gamma}^{[q]}  (\mbf{p} + \mbf{G}\bm{\xi}).
\end{align*}
Expanding the product $(\mbf{p} + \mbf{G}\bm{\xi})^T \bm{\Gamma}^{[q]}  (\mbf{p} + \mbf{G}\bm{\xi})$ yields $\mbf{p}^T \bm{\Gamma}^{[q]} (\mbf{p} + 2 \mbf{G} \bm{\xi}) + \bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi}$, 
with $\tilde{\bm{\Gamma}}^{[q]} = \mbf{G}^T \bm{\Gamma}^{[q]} \mbf{G} \in \tilde{\mbf{Q}}^{[q]}$.
Since $\tilde{\bm{\Gamma}}^{[q]} \in \tilde{\mbf{Q}}^{[q]}$, it follows that $\tilde{\Gamma}^{[q]}_{ij} = \midpoint{\tilde{Q}^{[q]}_{ij}} + \rad{\tilde{Q}^{[q]}_{ij}} \Lambda^{[q]}_{ij}$ for some $\Lambda^{[q]}_{ij} \in B_\infty^1$. Additionally, $\xi_i \in [-1,1]$ implies that $\xi_i^2 \in [0, 1]$, and hence $\xi_i^2 = \half + \half \zeta_i$ for some $\zeta_i \in [-1,1]$. Considering these two facts,
\begin{align*}
\bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi} & = \half \sum_i \midpoint{\tilde{Q}^{[q]}_{ii}} + \half \sum_i \midpoint{\tilde{Q}^{[q]}_{ii}} \zeta_i \\
& \quad + \sum_{i<j}(\midpoint{\tilde{Q}^{[q]}_{ij}} + \midpoint{\tilde{Q}^{[q]}_{ji}}) \xi_i \xi_j + \sum_{i,j} \rad{\tilde{Q}^{[q]}_{ij}} \xi_i \xi_j \Lambda^{[q]}_{ij},
\end{align*}
where the third summation results from the fact that $\xi_i \xi_j = \xi_j \xi_i$. Thus, by defining the new generator variables% vector
\begin{equation*} %\label{eq:firstordernewgen}
\bar{\bm{\xi}} = \big[ \,\; \cdots \,\; \underbrace{\zeta_i}_{\forall i} \,\; \cdots \,\; \underbrace{\xi_i \xi_j}_{\forall i<j} \,\; \cdots \,\; \underbrace{\xi_i \xi_j \Lambda^{[q]}_{ij}}_{\forall i,j,q} \,\; \cdots \,\; \big]^T,
\end{equation*}
we have that $\bm{\xi}^T \tilde{\bm{\Gamma}}^{[q]} \bm{\xi} = \tilde{c}_q + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}]_{q,:} \bar{\bm{\xi}}$, where
$\bar{\mbf{G}}_{\mbf{v}} = \text{blkdiag}(\mbf{N}^{[1]}, \mbf{N}^{[2]}, \dots, \mbf{N}^{[m]})$, 
\begin{equation*}
\mbf{N}^{[q]} = \big[ \,\; \cdots \,\; \underbrace{\rad{\tilde{Q}^{[q]}_{ij}}}_{\forall i,j} \,\; \cdots \,\; \big] \in \realsetmat{1}{(n_g+m_g)^2}.
\end{equation*} 

Therefore, we have established that
\begin{align*}
y_q = \kappa_q (\mbf{h}) + \nabla^T_x \kappa_q (\mbf{h})(\mbf{x} - \mbf{h}_x) + \nabla^T_v \kappa_q (\mbf{h})(\mbf{v} - \mbf{h}_v) + \mbf{p}^T \bm{\Gamma}^{[q]} (\mbf{p} + 2 \mbf{G} \bm{\xi}) + \tilde{c}_q + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}]_{q,:} \bar{\bm{\xi}}.
\end{align*}
This holds for every $q = 1,2,\dots,p$. Moreover, since $\mbf{L}$ is an interval matrix satisfying $\mbf{L}_{q,:} \supseteq \mbf{p}^T \mbf{Q}^{[q]}$ for all $q = 1,2,\dots,p$, there must exist $\hat{\mbf{L}}\in\mbf{L}$ such that $\hat{\mbf{L}}_{q,:}=\mbf{p}^T \bm{\Gamma}^{[q]}$ for all $q = 1,2,\dots,p$. Therefore,
\begin{equation*}
\mbf{y} = \bm{\kappa} (\mbf{h}) + \nabla^T_x \bm{\kappa} (\mbf{h})(\mbf{x} - \mbf{h}_x) + \nabla^T_v \bm{\kappa} (\mbf{h})(\mbf{v} - \mbf{h}_v) + \hat{\mbf{L}}(\mbf{p} + 2 \mbf{G} \bm{\xi}) + \tilde{\mbf{c}} + [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] \bar{\bm{\xi}},
\end{equation*}
which yields
\begin{equation} \label{Eq: kappa vector expansion}
\nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x}= \mbf{y} - \bm{\kappa} (\mbf{h}) + \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{h}_x + \nabla^T_v \bm{\kappa} (\mbf{h})\mbf{h}_v - \nabla^T_v \bm{\kappa} (\mbf{h})\mbf{v} - \hat{\mbf{L}}(\mbf{p} + 2 \mbf{G} \bm{\xi}) - \tilde{\mbf{c}} - [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] \bar{\bm{\xi}}. 
\end{equation}

The equality constraints $\mbf{A} \bm{\xi} = \mbf{b}$ imply that $\mbf{A} \bm{\xi} \bm{\xi}^T \mbf{A}^T = \mbf{b} \mbf{b}^T$. Thus, considering $\xi_i^2 = \half + \half \zeta_i$, the $r$-th row and $s$-th column of this matrix equality yields
\begin{align*}
\half \sum_i A_{ri} A_{si} \zeta_i + \sum_{i<j} (A_{ri} A_{sj} + A_{rj} A_{si}) \xi_i \xi_j = b_r b_s - \half \sum_i A_{ri} A_{si},
\end{align*}
with $r,s = 1,2,\dots,n_c$.
Such constraints are linear in $\bar{\bm{\xi}}$, and non-repeating for $r \leq s$, therefore $\bar{\mbf{A}} \bar{\bm{\xi}} = \tilde{\mbf{b}}$ holds, where $\bar{\mbf{A}} = [\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \bm{0}_{\tilde{n}_c \times n (n_g+m_g)^2}]$, with $\tilde{n}_c = \frac{n_c+m_c}{2}(1+n_c+m_c)$. Hence $\bm{\xi} \in B_\infty(\mbf{A},\mbf{b}) \implies \bar{\bm{\xi}} \in B_\infty(\bar{\mbf{A}},\tilde{\mbf{b}})$.

%Combining this with \eqref{Eq: eta vector expansion}, we have proven the enclosure
Combining this with \eqref{Eq: kappa vector expansion}, it was proven that
\begin{align*}
%\bm{\eta}(Z) & \subseteq \bm{\eta} (\mbf{h}) \oplus \nabla^T \bm{\eta} (\mbf{h})(Z - \mbf{h}) \\
%&\quad \oplus \mbf{L} (\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b})) \\
%& \quad \oplus \tilde{\mbf{c}} \oplus [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}).
\nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x} \in (\mbf{y} - \bm{\kappa} (\mbf{h}) + \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{h}_x &+ \nabla^T_v \bm{\kappa} (\mbf{h})\mbf{h}_v) \oplus (- \nabla^T_v \bm{\kappa} (\mbf{h})V) \\ & \oplus (- \mbf{L}(\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b}))) \oplus (- \tilde{\mbf{c}} )\oplus (- [\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty(\bar{\mbf{A}},\tilde{\mbf{b}}))).
\end{align*} 
This enclosure is greatly simplified by noting that the columns of $\bar{\mbf{A}}$ corresponding to the variables $[\,\; \cdots \,\; \xi_i \xi_j \Lambda^{[q]}_{ij}\,\; \cdots \,\;]$ are all zero, and hence
\begin{equation*}
[\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}) = \tilde{\mbf{G}} B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}}], \tilde{\mbf{b}}) \oplus \bar{\mbf{G}}_{\mbf{v}} B_\infty^{n(n_g+m_g)^2}.
\end{equation*}
Since $\bar{\mbf{G}}_{\mbf{v}}$ is block diagonal and each $\mbf{N}^{[q]}$ is a row vector, $\bar{\mbf{G}}_{\mbf{v}} B_\infty^{n(n_g+m_g)^2}$ is an interval, and is equivalent to $\tilde{\mbf{G}}_{\mbf{v}} B_\infty^{n}$, with $\tilde{\mbf{G}}_{\mbf{v}}$ defined as in the statement of the theorem. Thus,
\begin{align*}
[\tilde{\mbf{G}} \,\; \bar{\mbf{G}}_{\mbf{v}}] B_\infty (\bar{\mbf{A}}, \tilde{\mbf{b}}) &= \tilde{\mbf{G}} B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}}], \tilde{\mbf{b}}) \oplus \tilde{\mbf{G}}_{\mbf{v}} B_\infty^{n}, \\
&= [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty ([\tilde{\mbf{A}}_{\bm{\zeta}} \,\; \tilde{\mbf{A}}_{\bm{\xi}} \,\; \mbf{0}_{\tilde{n}_c\times n}], \tilde{\mbf{b}}), \\
&= [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty (\tilde{\mbf{A}}, \tilde{\mbf{b}}).
\end{align*}
Therefore,
\begin{align*}
%\bm{\eta}(Z) \subseteq \bm{\eta} (\mbf{h}) &\oplus \nabla^T \bm{\eta} (\mbf{h})(Z - \mbf{h}) \\
%&\oplus \mbf{L} (\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b})) \\
%&\oplus \tilde{\mbf{c}} \oplus [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty (\tilde{\mbf{A}}, \tilde{\mbf{b}}),
\nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x} & \in (\mbf{y} - \bm{\kappa} (\mbf{h}) + \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{h}_x + \nabla^T_v \bm{\kappa} (\mbf{h})\mbf{h}_v) \oplus (- \nabla^T_v \bm{\kappa} (\mbf{h})V) \\ & \quad \quad \quad \quad \oplus (- \mbf{L}(\mbf{p} \oplus 2 \mbf{G} B_\infty(\mbf{A},\mbf{b}))) \oplus (- \tilde{\mbf{c}} )\oplus (- [\tilde{\mbf{G}} \,\; \tilde{\mbf{G}}_{\mbf{v}}] B_\infty(\tilde{\mbf{A}},\tilde{\mbf{b}})))\\
& = (\mbf{y} - \bm{\kappa} (\mbf{h}) + \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{h}_x + \nabla^T_v \bm{\kappa} (\mbf{h})\mbf{h}_v) \oplus (- \nabla^T_v \bm{\kappa} (\mbf{h})V) \\ & \quad \quad \quad \quad \oplus (- R)\\
& = Y.
\end{align*}
Therefore, $\bm{\kappa}(\mbf{x},\mbf{v}) = \mbf{y} : \mbf{x} \in X, \mbf{v} \in V \implies \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x} \in Y$. Then, for every $\mbf{x} \in X : \bm{\kappa}(\mbf{x},\mbf{v}) = \mbf{y}, \mbf{v} \in V$, we conclude that $\nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x} \in Y$. Therefore, $\{\mbf{x} \in X : \bm{\kappa}(\mbf{x},\mbf{v}) = \mbf{y}, \mbf{v} \in V\} \subseteq \{\mbf{x} \in X : \nabla^T_x \bm{\kappa} (\mbf{h})\mbf{x} \in Y\} = X \ginter{\mbf{C}} Y$. \qed

\begin{remark} \rm Similarly to Theorems \ref{the:pred2} and \ref{thm:firstorder}, Theorem \ref{thm:nonlinearmeasurement} allows different choices of $\mbf{h}_x \in X$, $\mbf{h}_v \in V$. It is expected that these different choices affect the conservatism of the resulting bounds, specifically in the computation of the constrained zonotope $Y$. Since these bounds are based on the first-order Taylor extension, we propose in fact \emph{C4}-\emph{C6} as possible choices of $\mbf{h}_x$ and $\mbf{h}_v$, and expect \emph{C6} to be the least conservative one.	
\end{remark}

%The exact characterization of sets $X_k$ containing the evolution of the system states is very difficult in the nonlinear case, if not intractable \citep{Alamo2005a,Kieffer1998,Kuhn1998}. Therefore, in the set-membership framework the objective is to over-approximate such sets by guaranteed outer bounds $\hat{X}_k$ on the possible trajectories of the system states $\mbf{x}_k$. Such outer bounds must be consistent with the previous estimate $\hat{X}_{k-1}$ and known inputs $\mbf{u}_{k-1}$, and also with the current measurement $\mbf{y}_k$, and the bounds on the disturbances and uncertainties $W_{k-1}$, $V_k$. Given an initial set $\mbf{x}_0 \in \hat{X}_0$, a common approach is to proceed through the well-known prediction-update algorithm, which consists in computing real compact sets $\bar{X}_k$ and $\hat{X}_k$ such that
%\begin{align}
%\bar{X}_k & \supseteq \{ \mbf{f}(\mbf{x}, \mbf{u}_{k-1}, \mbf{w}) : \mbf{x} \in \hat{X}_{k-1}, \, \mbf{w} \in W_{k-1} \}, \label{eq:prediction0}\\
%\hat{X}_k & \supseteq \{ \mbf{x} \in \bar{X}_k : \mbf{C} \mbf{x} + \mbf{D}_u \mbf{u}_k + \mbf{D}_v \mbf{v} = \mbf{y}_k, \, \mbf{v} \in V_k \}, \label{eq:update0}
%\end{align}
%in which \eqref{eq:prediction0} is referred to as the \emph{prediction step}, and \eqref{eq:update0} as the \emph{update step}. 
%
%Our goal is to obtain accurate outer bounds $\bar{X}_k$ and $\hat{X}_k$ according to \eqref{eq:prediction0} and \eqref{eq:update0}, respectively. Following these definitions, and considering the initial condition $\mbf{x}_0 \in \hat{X}_0$, the property $\mbf{x}_k \in \hat{X}_k$ is guaranteed by construction for all $k \geq 0$ \citep{Chisci1996,Le2013,Alamo2008}.



\section{Final remarks}

This chapter developed new set-valued state estimation methods based on constrained zonotopes. The first method was applied to a linear case with different sampling times, involving state-feedback control for trajectory tracking of a suspended load using a tilt-rotor UAV. A constrained minimum-variance criterion was proposed for feedback connection with estimated states. Thereafter, three new nonlinear set-valued state estimation methods were developed, specifically the CZIB algorithm, the mean value extension, and the first-order Taylor extension using constrained zonotopes. Measurement data were effectively taken into account by means of exact intersection of constrained zonotopes considering linear measurement. A novel approach to deal with nonlinear measurement using constrained zonotopes was also proposed.%are presented, and some future directions are proposed.

The linear state estimation method was validated through numerical experiments carried out in the ProVANT simulator, a platform based on the Gazebo simulator with a CAD model of the system, which demonstrated the reduced conservativeness of the proposed linear set-valued state estimator, the performance of the optimal selection of estimated states, and the robustness of the designed controller.


The new nonlinear state estimation methods were validated through numerical experiments. The first example demonstrated the reduced conservativeness of the CZIB algorithm in comparison to a zonotope-based method from the literature. The second example demonstrated the accuracy of the proposed extensions for nonlinear set-valued state estimation using constrained zonotopes. A numerical experiment considering a quadrotor UAV was also conducted, considering a realistic scenario in which measurements are provided by sensors located at the UAV. In each experiment the new methods were compared with existing zonotope-based approaches. % based on constrained zonotopes,

The next chapter develops a new method for set-based fault detection and isolation of nonlinear discrete-time systems. Enclosures described by constrained zonotopes are employed in the passive fault detection and active fault isolation processes, based on the nonlinear state estimation methods introduced in this chapter.





==> template/macros.tex <==
\selectlanguage{english}%
\global\long\def\dq#1{\underline{\boldsymbol{#1}}}


\global\long\def\quat#1{\boldsymbol{#1}}


\global\long\def\mymatrix#1{\boldsymbol{#1}}


\global\long\def\myvec#1{\boldsymbol{#1}}


\global\long\def\mapvec#1{\boldsymbol{#1}}


\global\long\def\dualvector#1{\underline{\boldsymbol{#1}}}


\global\long\def\dual{\varepsilon}


\global\long\def\dotproduct#1{\langle#1\rangle}


\global\long\def\norm#1{\left\Vert #1\right\Vert }


\global\long\def\mydual#1{\underline{#1}}


\global\long\def\hamilton#1#2{\overset{#1}{\operatorname{\mymatrix H}}\left(#2\right)}


\global\long\def\hamiquat#1#2{\overset{#1}{\operatorname{\mymatrix H}}_{4}\left(#2\right)}


\global\long\def\hami#1{\overset{#1}{\operatorname{\mymatrix H}}}


\global\long\def\tplus{\dq{{\cal T}}}


\global\long\def\getp#1{\operatorname{\mathcal{P}}\left(#1\right)}


\global\long\def\getd#1{\operatorname{\mathcal{D}}\left(#1\right)}


\global\long\def\swap#1{\text{swap}\{#1\}}


\global\long\def\imi{\hat{\imath}}


\global\long\def\imj{\hat{\jmath}}


\global\long\def\imk{\hat{k}}


\global\long\def\real#1{\operatorname{\mathrm{Re}}\left(#1\right)}


\global\long\def\imag#1{\operatorname{\mathrm{Im}}\left(#1\right)}


\global\long\def\imvec{\boldsymbol{\imath}}


\global\long\def\vector{\operatorname{vec}}


\global\long\def\mathpzc#1{\fontmathpzc{#1}}


\global\long\def\cost#1#2{\underset{\text{#2}}{\operatorname{\text{cost}}}\left(\ensuremath{#1}\right)}


\global\long\def\diag#1{\operatorname{diag}\left(#1\right)}


\global\long\def\frame#1{\mathcal{F}_{#1}}


\global\long\def\ad#1#2{\text{Ad}\left(#1\right)#2}




\global\long\def\dualquaternion#1{\underline{\boldsymbol{#1}}}


\global\long\def\quaternion#1{\boldsymbol{#1}}
\selectlanguage{american}%


